DUB: Discrete Unit Back-translation for Speech Translation

How can speech-to-text translation (ST) perform as well as machine translation (MT)? The key point is to bridge the modality gap between speech and text so that useful MT techniques can be applied to ST. Recently, the approach of representing speech with unsupervised discrete units yields a new way to ease the modality problem. This motivates us to propose Discrete Unit Back-translation (DUB) to answer two questions: (1) Is it better to represent speech with discrete units than with continuous features in direct ST? (2) How much benefit can useful MT techniques bring to ST? With DUB, the back-translation technique can successfully be applied on direct ST and obtains an average boost of 5.5 BLEU on MuST-C En-De/Fr/Es. In the low-resource language scenario, our method achieves comparable performance to existing methods that rely on large-scale external data. Code and models are available at https://github.com/0nutation/DUB.

==> Sections/010_intro_pre.tex <==

\skeleton{
Can speech be sufficiently represented by discrete units? Previous work has used discrete representations to enhance better speech representations, such as w2v, hubert, cobert... 
}

\skeleton{There are other studies using discrete audio units in downstream tasks such as TTS and S2ST in speech generation tasks. For example, xxx defines a new paradigm for speech generation.
}

\skeleton{Translation is a good task for such verification. MT and ST are two sibling tasks, but due to the symbolic gap between speech and text, there is always a gap between ST and MT. Techniques in MT are also difficult to transfer to speech. For example back-translation, xxx. But with speech discretization, can we also use BT in ST?}

% \skeleton{para1: ST problem and challenge (no enough data)}
Speech-to-text translation (ST) aims at using a single model to translate source-language speech directly into target-language texts, which has gained significant attention recently~\cite{sung2019towards,salesky-etal-2019-exploring,chen2020mam,han-etal-2021-learning,fang2022stemm,ye2022cross}.
%This feature gives ST special advantages over conventional cascaded systems in accelerating inference and avoiding transcription mistakes made by ASR models. 
However, as a cross-modal translation task, ST is overloaded for a single model especially when suffering from severe data scarcity. 
Prevailing ST methods focus on pre-training strategies~\cite{zheng2021fused,dong2021consecutive,dong2021listen,tang2022unified,zhang2022speechut} or multi-task learning framework~\cite{anastasopoulos2018tied,indurthi2021task,tang2021improving,ye2021end} using external machine translation (MT) and automatic speech recognition (ASR) data to tackle this problem and have made great improvements.

Recently, researchers have started exploring discretizing continuous speech representation in self-supervised speech representation learning~\cite{van2017neural, baevski2019vq,baevski2020wav2vec,hsu2021hubert,meng2022cobert}. 
Discrete representations have been applied to various speech-processing tasks, such as text-to-speech synthesis~\cite{dunbar2019zero}, spoken language modeling~\cite{lakhotia2021generative,kharitonov2022text}, speech-to-speech translation~\cite{lee2022textless,inaguma2022unity,popuri2022enhanced,huang2022transpeech}, speech emotion conversion~\cite{kreuk2021textless} etc. 
Previous work~\cite{polyak2021speech} shows that self-supervised discrete representation can retain linguistic content and remove speaker identity and prosodic information in speech. 
Moreover, compared with continuous speech representation, discrete representation enables a wide variety of NLP techniques to be applied to speech-processing tasks. Consequently, the model structure of NLP tasks and speech-processing taks can be formally unified.
This is exactly what we practice in our work, where we take speech-to-text translation as an example, unify the model architecture of ST and MT through a discrete unit extractor for speech, and migrate back-translation techniques that are commonly used in MT to ST. In this way, we can resort to monolingual text corpus to tackle data scarity in ST. 


%\skeleton{para2: introducing monolingual text data is an interesting topic. How?} 
\iffalse
However, ASR/MT data is scarce for many low-source languages and about 3000 languages in the world have no written form at all, which means that resorting to ASR/MT data is not the answer to speech translation for all language pairs. In fact, monolingual text corpus is several orders of magnitude larger than ASR/MT data and accessible for all ST language pairs, so it will be a big step forward if we can utilize unpaired text to tackle data scarcity in ST. In the field of machine translation, back-translation is the most prevalent approach to utilize unpaired text data and remains widely used in state-of-the-art NMT systems~\cite{sennrich-etal-2016-improving,edunov-etal-2018-understanding,caswell2019tagged}. To apply back-translation in ST, a pre-trained text-to-speech translation model is required to generate source speech from unpaired target text. However, it's difficult to apply back-translation in ST for several reasons:
\begin{itemize}
  \item[1.]
    Cascaded text-to-speech translation pipeline combines machine translation model and text-to-speech model, which is lengthy and suffer from the issues of error propagation;
  \item[2.]
  Speech-to-text translation and text-to-speech translation are not dual task. Generating continuous speech is more difficult than generating discrete text so it's challenging to train an end-to-end text-to-speech translation model;
  \item[3.]
  Synthetic speech is robotic and monotonic and in a different distribution from real speech, making it easy to overfit the model to synthetic speech.
\end{itemize}
Inspired by recent studies on discrete self-supervised speech representations~\cite{baevski2019vq,baevski2020wav2vec,hsu2021hubert}, we argue that back-translating to discrete representations has the potential to reduce the difficulty of text-to-speech translation and apply back-translation to ST successfully.
\fi
%But BT in ST is not easy, because:  (show figure1 here at the left-upper)
%    - 1. STT and TTS are not dual. 
%    - 2. Cascaded BT-TTS pipeline is lengthy. 
%    - 3. Generated speech is robotic and monotonic, easily for the model to overfit. While generating diverse speech is complicated.
%    - 4. Error propagation may occur during the cascaded BT-TTS pipeline, making the pseudo parallel data mismatching.

%\skeleton{para3: In this work, we propose xx. }
In this paper, we proposed \textbf{D}iscrete \textbf{U}nit \textbf{B}ack-translation~(\method) to apply back-translation to ST. We adopt HuBERT~\cite{hsu2021hubert} to convert speech to discrete unit and regard discrete unit as a kind of pseudo-language. Instead of using a text-to-speech translation system on unpaired text to produce synthetic speech, we build a text-to-unit model which learns to predict the discrete units rather than continuous value, making it a much easier task and reducing speaker dependency. The trained text-to-units model generates the synthetic discrete units from a large amount of unpaired text and we fulfill the forward translation pass by training the unit-to-text Transformer model on mixture of real and synthetic paired data. Experimental results demonstrate that DUB can bring about 5 bleu improvement over baseline and achieves comparable performance with previous methods in MuST-C dataset and and achieve comparable performance with large-scale multilingual speech or text pre-training methods in CoVoST2 low-source scenes.

Our contributions are as follows:
\begin{itemize}
  \item
  This is the first work to unify the ST and MT framework, by adding a discrete unit extractor for speech.
  \item
  Based on the unified structure, we propose Discrete Unit Back-translation (DUB), which makes a large number of easily-obtained target language texts to be efficiently utilized.
  \item
  Since the discretization process is unsupervised, our method does not rely on transcribed text, friendly for unwritten language.
  \item
  We perform experiments on standard MuST-C benchmark, as well as high-resource and low-resource unwritten sceneries on CoVoST-2. 
\end{itemize}


==> Sections/010_intro_pre2.tex <==
Speech-to-text translation (ST) converts the spoken source language into the written target language, which is a closely related task to machine translation (MT).
In recent years, direct ST that does not rely on intermediate transcription has received considerable attention due to its potential applications in unwritten language scenarios and various domains~\cite{sung2019towards,han-etal-2021-learning,papi2021speechformer,fang2022stemm,ye2022cross}. 
One of the major challenges faced by ST is data scarcity, which is similar to the low-resource scenarios encountered in MT. 
Intuitively, techniques developed for low-resource MT~\cite{xia2019generalized,chen2020facebook,liu2020multilingual,tang2020multilingual} should be utilized to improve ST performance.
In fact, these techniques are hard to be transferred to ST due to the modality gap between speech and text, where ST takes continuous speech as input and MT takes discrete tokens as input.


==> Sections/034_pretrains.tex <==
\yr{this part needs to think twice...}
\yr{or we need the figure to show such procedures.}

Through speech discretization, our model unifies the text translation and speech translation frameworks, while other techniques commonly used in MT, such as pre-training, are compatible with our approach.
We explore two pre-training methods for the unit-to-text translation model: cross-modal mBART and unit-ASR \yr{name is weird} pre-training. 

\noindent\textbf{Cross-modal mBART}~ 
mBART\cite{liu2020multilingual} pre-trains a complete sequence-to-sequence model by denoising full texts in multiple languages. 
mBART trains the model to predict original text $\boldsymbol{X}$ given corrupted text $\boldsymbol{g(X)}$, where $\boldsymbol{g}$ is a noising function and $\boldsymbol{X}$ is a mixture of multilingual texts. 
Following mBART, our cross-modal mBART is trained with a Transformer encoder-decoder architecture. We treat the mixture of discrete units $\boldsymbol{D_{units}}$ extracted from unlabeled speech data and unlabeled text $\boldsymbol{D_{text}}$ in the target language as $\boldsymbol{X}$
 and use sentence permutation and word-span masking strategies as $\boldsymbol{g}$.  Formally, we aim to minimize
\begin{equation*}
    \mathcal{L}_\theta=\sum_{\mathcal{D}_i \in \mathcal{D}} \sum_{X \in \mathcal{D}_i} \log P(X \mid g(X) ; \theta)
\end{equation*}
, where $\mathcal{D}=\left\{\mathcal{D}_{unit}, \mathcal{D}_{text}\right\}$, $g(\cdot)$ is the noising function by randomly masking some discrete tokens, and $\boldsymbol{P}$\yr{params are $\theta$} is defined by the cross-modal mBART model. 


 
\noindent\textbf{Unit-ASR}~
According to \cite{wang-etal-2020-fairseq}, a pre-trained ASR encoder is essential for speech translation models. 
Unit-ASR has the same objective function as ASR, where the model needs to predict the transcripts based on the input sequence. 
Particularly, unit-ASR takes discrete units as input. Similarly, we pre-train the discrete unit pre-net, discrete unit encoder and text decoder with parallel units-transcripts pairs $(\boldsymbol{U},\boldsymbol{X})$, converted from speech-transcript pairs $(\boldsymbol{S},\boldsymbol{X})$ by the discrete units extractor. The training objective is negative log-likelihood on units-transcripts pairs as the loss function. 
\begin{equation*}
    \mathcal{L}_{unit-ASR}=-E_{(U,X)} \log P(X|U)
\end{equation*}
Different from previous encoder-only ASR pre-training, we utilize pre-trained unit-ASR complete encoder-decoder architecture for DUB pre-training.



==> Tables/model_size.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{c|c|ccc}
        \toprule
         & Model & Encoder & Decoder &   \\
         & Params & Layers & Layers & Hidden \\
        \midrule
        \textcircled{1} & 73M & 6 & 6 & 512 \\
        \textcircled{2} & 176M & 12 & 6 & 768 \\
        \textcircled{2} & 260M & 12 & 6 & 1024 \\
        \bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/000_abstract.tex <==
How can speech-to-text translation (ST) perform as well as machine translation (MT)?
The key point is to bridge the modality gap between speech and text so that useful MT techniques can be applied to ST.
Recently, the approach of representing speech with unsupervised discrete units yields a new way to ease the modality problem.
This motivates us to propose \textbf{D}iscrete \textbf{U}nit \textbf{B}ack-translation~(\textbf{\method}) to answer two questions:
\begin{inparaenum}[(1)\upshape]
    \item Is it better to represent speech with discrete units than with continuous features in direct ST?
    \item How much benefit can useful MT techniques bring to ST?
\end{inparaenum}
With \method, the back-translation technique can successfully be applied on direct ST and obtains an average boost of 5.5 BLEU on MuST-C En-De/Fr/Es.
In the low-resource language scenario, our method achieves comparable performance to existing methods that rely on large-scale external data.
Code and models are available at 
\url{https://github.com/0nutation/DUB}.
% \url{https://anonymous.4open.science/r/DUB/}.


%This motivates us to propose \textbf{D}iscrete \textbf{U}nit \textbf{B}ack-translation~(\textbf{\method}) for two purposes:
%(1) To explore the potential benefits of using speech discrete units 
%This motivates us to explore the potential benefits of using such approach in end-to-end ST.

%Also, it achieves comparable performance to joint speech-text pre-training models that rely on large-scale external data on ST for low-resource languages with less than 2 hours, indicating its promising potential in dealing with unwritten languages.

% How can the techniques used in text-to-text machine translation~(MT) be transferred to speech-to-text translation~(ST)? 
%The key point is to bridge the modal gap between continuous speech \textit{signals} and discrete text \textit{symbols}. 
%In this paper, we propose \textbf{D}iscrete \textbf{U}nit \textbf{B}ack-translation~(\textbf{\method}), which migrates the back-translation technique from MT to ST by discretizing the speech signals into unit sequences and leveraging the additional easy-to-obtain text in the target language.
%Without relying on transcription and pre-training, \method obtains an average boost of 6.3 BLEU on MuST-C En-De/Fr/Es, and achieves comparable performance to the large-scale speech-text joint pre-training models on CoVoST-2 low-resource ST. 
%Code and models are available at \url{https://anonymous.4open.science/r/DUB/}.



==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/010_intro.tex <==
% As a sibling task of machine translation~(MT), speech-to-text translation~(ST) aims to translate source-language speech into target-language text. 
% Speech-to-text translation (ST) is a closely related task to machine translation (MT) that involves converting spoken source language into written target language.

Speech-to-text translation (ST) converts the spoken source language into the written target language, which is a closely related task to machine translation (MT).
In recent years, direct ST that does not rely on intermediate transcription has received considerable attention due to its potential applications in unwritten language scenarios and various domains~\cite{berard2016listen,sung2019towards,han-etal-2021-learning,papi2021speechformer,fang2022stemm,ye2022cross, cheng2023m}. 
One of the major challenges faced by ST is data scarcity, which is similar to the low-resource scenarios encountered in MT. 
Intuitively, techniques developed for low-resource MT~\cite{imamura2018enhancement,xia2019generalized,chen2020facebook,liu2020multilingual,tang2020multilingual} should be utilized to improve ST performance.
% However, the modality gap between speech and text presents a challenge in transferring these techniques, as ST takes continuous speech as input while MT takes discrete tokens as input.
However, these techniques are hard to be transferred to ST due to the modality gap between speech and text, where ST takes continuous speech as input and MT takes discrete tokens as input.
Generally speaking, if there is a way to efficiently remove the modality gap, a large number of useful NLP techniques can be applied and facilitate the improvement of ST.

%However, the application of specific MT techniques, such as back-translation~\cite{edunov-etal-2018-understanding,imamura2018enhancement}, 
%is hard to be applied on ST due to the modality gap between speech and text.
%This modality gap also limits the transfer of other NLP techniques to ST.
%If there is a way to remove the modality gap, a large number of useful NLP techniques can be applied on ST.
%potential for further advancements in ST performance.
% However, applying specific MT techniques such as back-translation to ST remains challenging due to the symbolic discrepancy between their input, where ST takes continuous speech as input and MT takes discrete tokens as input. This mismatch limits further improvements in ST performance. 
% Naturally, we have this question: How sufficiently can continuous speech be represented by discrete units?
%Can continuous speech be sufficiently represented by discrete units? 


% Discretizing continuous speech is a topic of significant interest in the field of speech processing. Researchers have started exploring using discrete speech representation to enhance better speech representation~\cite{baevski2019vq,baevski2020wav2vec,hsu2021hubert,meng2022cobert}. 
Recently, representing speech with unsupervised discrete units has become popular and successful in the field of speech processing~\cite{baevski2019vq,baevski2020wav2vec,hsu2021hubert,lakhotia2021generative}.
Instead of losing relevant information, discretizing continuous speech has been found to have the advantage of filtering out extraneous signals~\cite{sicherman2023analysing, lakhotia2021generative}, leading to significant improvements in the speech tasks, such as automatic speech recognition~\cite{meng2022cobert}, text-to-speech~\cite{dunbar2019zero}, and speech-to-speech translation~\cite{zhang2021uwspeech,lee2022textless,inaguma2022unity}.
% Additionally, utilizing discrete units for speech representation enables the application of a wide variety of NLP techniques to speech processing tasks.
% Instead of losing relevant information, discretizing continuous speech has been found to have the benefit of filtering out extraneous signals~\cite{sicherman2023analysing} and leads to significant gains in various speech tasks.
% New state-of-the-art results are reported in automatic speech recognition~\cite{meng2022cobert}, text-to-speech~\cite{dunbar2019zero} and speech-to-speech translation~\cite{lee2022textless,inaguma2022unity}.
Based on this observation, we are motivated to explore the answers to the following two questions: 
\begin{inparaenum}[(1)\upshape]
    \item Is it better to represent speech with discrete units and use them as model input than with continuous features for direct ST?
    \item By narrowing the modality gap with discrete speech units, how much benefit can useful MT techniques bring to direct ST?
\end{inparaenum}
% Instead of losing relevant information, discretizing continuous speech seems to have the benefit of filtering out unwanted 

% First, research has suggested that speech discrete representation can help eliminate some unwanted signals~\cite{sicherman2023analysing} and leads to significant gains in various speech tasks~\cite{meng2022cobert,lee2022textless,dunbar2019zero}. Consequently, this leads to the question: Is it more beneficial to use discrete units to represent speech in direct ST?  
% Second, speech discrete representation is distinct from continuous representation in that it is composed of discrete symbols, much like text tokens; the narrowed modality gap enables a range of NLP techniques to be integrated with speech. This brings up the second question: How much benefit can useful MT techniques bring to ST?

%Using discrete units seems to be a good way to narrow the modality gap between 
%Discretizing continuous speech is a topic of significant interest in the field of speech processing. Researchers have started exploring using discrete speech representation to enhance better speech representation~\cite{baevski2019vq,baevski2020wav2vec,hsu2021hubert,meng2022cobert}. 
%There are other studies that utilize discrete units to represent speech and apply them to downstream speech generation tasks such as text-to-speech synthesis~\cite{dunbar2019zero}, spoken language modeling~\cite{lakhotia2021generative}, and speech-to-speech translation~\cite{lee2022textless,inaguma2022unity}. 
% Among them, GSLM~\cite{lakhotia2021generative} defines a new paradigm for speech generation. 
%Meanwhile, compared to continuous speech representation, discrete representation facilitates the utilization of a wide variety of NLP techniques that can be applied to speech-processing tasks. 
%One specific example is the utilization of back-translation, which is commonly employed in MT
% ~\cite{sennrich-etal-2016-improving,edunov-etal-2018-understanding,caswell2019tagged}
%but not as prevalent in ST due to the complex pipeline involved in generating source-language speech from target-language text.
%However, through the process of speech discretization, the use of discrete units allows for the application of back-translation in ST.

In this paper, we propose \textbf{D}iscrete \textbf{U}nit \textbf{B}ack-translation~(\textbf{\method}), which migrates the useful back-translation technique from MT to ST by discretizing the speech signals into unit sequences.
% To convert speech to discrete units, we utilize HuBERT~\cite{hsu2021hubert}, and treat the discrete units as a form of pseudo-language. 
In our proposed method, we first convert speech into discrete units using the clustering indices on HuBERT~\cite{hsu2021hubert} representations. 
% (called \textit{hidden units} in previous literature) 
% and treat the discrete units as a form of pseudo-language.
To complete the translation task, we feed the discrete units into the \textbf{U}nit-\textbf{to}-\textbf{T}ext \textbf{T}ranslation (U2TT) model.
% For the back-translation training strategy, instead of predicting continuous source speech, \method employs a text-to-unit translation model that learns to predict the source discrete units from target text, thus reducing the difficulty of generation and minimizing speaker dependency.
For the back-translation training strategy, \method employs a text-to-unit translation model that learns to predict the source discrete units from the target text.
By leveraging the additional easily accessible text in the target language, we utilize the synthetic parallel data generated by the text-to-unit translation model in conjunction with the original parallel data to update the final unit-to-text model.


% We conducted experiments on the MuST-C~\cite{di2019must} and CoVoST-2~\cite{wang2021covost} ST benchmarks, 
% and show that the model, as well as our DUB training method, outperforms the baseline model in the MuST-C English-to-German/French/Spanish ST directions by an average of 5.5 BLEU.
% And more importantly, we investigate the great value of discretizing speech and using the unit-to-text model to perform downstream tasks.
% \begin{inparaenum}[\itshape a)\upshape]
%     \item We show that the unit retains the semantic information for translation and can be used as model input.
%     \item Various phenomena in the analysis that are consistent with MT, indicate the potential of such a framework for incorporating more MT techniques, such as large-scale pre-training.
%     \item Our approach is particularly beneficial for resource-poor or unwritten languages in the world because unit extraction does not require any textual supervision and only speech-translation pairs are used for training.
% \end{inparaenum}

% Our results demonstrate that \method can obtain an average boost of 6.3 BLEU on the MuST-C benchmark and achieve comparable performance to large-scale speech-text pre-training models on CoVoST-2 low-resource language pairs. 
% Furthermore, it is feasible to build a unified framework for ST and MT through speech discretization.


Our contributions include the following.
\begin{itemize}[itemsep=1pt, leftmargin=10pt, parsep=0pt, topsep=1pt]
    \item We design a novel unit-text translation (U2TT) framework for direct ST by discretizing the speech feature in an unsupervised manner.
    Our analysis shows that in such a framework, the unit retains the semantic information for translation and can be used as model input.

    \item 
    Based on the U2TT framework, we propose \method, which successfully applies the back-translation technique to direct ST.
    Experimental results show that DUB can further yield an average 5.5 BLEU gain over the U2TT model on the MuST-C English-to-German, French, and Spanish translation directions.

    
    \item Our approach is particularly beneficial for low-resource or unwritten languages in the world because unit extraction does not require any textual supervision and only speech-translation pairs are used for training.
\end{itemize}

%   We unify the ST and MT frameworks by adding a discrete unit extractor for speech.
%   % We propose Discrete Unit Back-translation (DUB), which migrates back-translation technique from MT to ST and utilizes numerous easily-obtained target language texts to boost ST performance.
%      We propose Discrete Unit Back-translation~(DUB), which is an effective method to integrate unpaired text into ST and obtains an average boost of 5.3 BLEU on MuST-C benchmark and achieves comparable performance to large-scale pre-training models on CoVoST-2 low-resource language pairs.
     
%   \item
%   % We verify the feasibility of building a unified framework for ST and MT through speech discretizaton.
%     We verify the feasibility of building a unified framework for ST and MT through speech discretizaton.
  % \item
  % Without demanding for transcribed text, \method is friendly for unwritten language.
  % \item
  % %We perform experiments on standard MuST-C benchmark, as well as high-resource and low-resource unwritten scenarios on CoVoST-2. 
  % \method obtains an average boost of 5.3 BLEU on MuST-C benchmark and achieves comparable performance to large-scale pre-training models on CoVoST-2 low-resource language pairs. 
  % % \yr{detailed figures}
% \end{itemize}

==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/010_intro_pre.tex <==

\skeleton{
Can speech be sufficiently represented by discrete units? Previous work has used discrete representations to enhance better speech representations, such as w2v, hubert, cobert... 
}

\skeleton{There are other studies using discrete audio units in downstream tasks such as TTS and S2ST in speech generation tasks. For example, xxx defines a new paradigm for speech generation.
}

\skeleton{Translation is a good task for such verification. MT and ST are two sibling tasks, but due to the symbolic gap between speech and text, there is always a gap between ST and MT. Techniques in MT are also difficult to transfer to speech. For example back-translation, xxx. But with speech discretization, can we also use BT in ST?}

% \skeleton{para1: ST problem and challenge (no enough data)}
Speech-to-text translation (ST) aims at using a single model to translate source-language speech directly into target-language texts, which has gained significant attention recently~\cite{sung2019towards,salesky-etal-2019-exploring,chen2020mam,han-etal-2021-learning,fang2022stemm,ye2022cross}.
%This feature gives ST special advantages over conventional cascaded systems in accelerating inference and avoiding transcription mistakes made by ASR models. 
However, as a cross-modal translation task, ST is overloaded for a single model especially when suffering from severe data scarcity. 
Prevailing ST methods focus on pre-training strategies~\cite{zheng2021fused,dong2021consecutive,dong2021listen,tang2022unified,zhang2022speechut} or multi-task learning framework~\cite{anastasopoulos2018tied,indurthi2021task,tang2021improving,ye2021end} using external machine translation (MT) and automatic speech recognition (ASR) data to tackle this problem and have made great improvements.

Recently, researchers have started exploring discretizing continuous speech representation in self-supervised speech representation learning~\cite{van2017neural, baevski2019vq,baevski2020wav2vec,hsu2021hubert,meng2022cobert}. 
Discrete representations have been applied to various speech-processing tasks, such as text-to-speech synthesis~\cite{dunbar2019zero}, spoken language modeling~\cite{lakhotia2021generative,kharitonov2022text}, speech-to-speech translation~\cite{lee2022textless,inaguma2022unity,popuri2022enhanced,huang2022transpeech}, speech emotion conversion~\cite{kreuk2021textless} etc. 
Previous work~\cite{polyak2021speech} shows that self-supervised discrete representation can retain linguistic content and remove speaker identity and prosodic information in speech. 
Moreover, compared with continuous speech representation, discrete representation enables a wide variety of NLP techniques to be applied to speech-processing tasks. Consequently, the model structure of NLP tasks and speech-processing taks can be formally unified.
This is exactly what we practice in our work, where we take speech-to-text translation as an example, unify the model architecture of ST and MT through a discrete unit extractor for speech, and migrate back-translation techniques that are commonly used in MT to ST. In this way, we can resort to monolingual text corpus to tackle data scarity in ST. 


%\skeleton{para2: introducing monolingual text data is an interesting topic. How?} 
\iffalse
However, ASR/MT data is scarce for many low-source languages and about 3000 languages in the world have no written form at all, which means that resorting to ASR/MT data is not the answer to speech translation for all language pairs. In fact, monolingual text corpus is several orders of magnitude larger than ASR/MT data and accessible for all ST language pairs, so it will be a big step forward if we can utilize unpaired text to tackle data scarcity in ST. In the field of machine translation, back-translation is the most prevalent approach to utilize unpaired text data and remains widely used in state-of-the-art NMT systems~\cite{sennrich-etal-2016-improving,edunov-etal-2018-understanding,caswell2019tagged}. To apply back-translation in ST, a pre-trained text-to-speech translation model is required to generate source speech from unpaired target text. However, it's difficult to apply back-translation in ST for several reasons:
\begin{itemize}
  \item[1.]
    Cascaded text-to-speech translation pipeline combines machine translation model and text-to-speech model, which is lengthy and suffer from the issues of error propagation;
  \item[2.]
  Speech-to-text translation and text-to-speech translation are not dual task. Generating continuous speech is more difficult than generating discrete text so it's challenging to train an end-to-end text-to-speech translation model;
  \item[3.]
  Synthetic speech is robotic and monotonic and in a different distribution from real speech, making it easy to overfit the model to synthetic speech.
\end{itemize}
Inspired by recent studies on discrete self-supervised speech representations~\cite{baevski2019vq,baevski2020wav2vec,hsu2021hubert}, we argue that back-translating to discrete representations has the potential to reduce the difficulty of text-to-speech translation and apply back-translation to ST successfully.
\fi
%But BT in ST is not easy, because:  (show figure1 here at the left-upper)
%    - 1. STT and TTS are not dual. 
%    - 2. Cascaded BT-TTS pipeline is lengthy. 
%    - 3. Generated speech is robotic and monotonic, easily for the model to overfit. While generating diverse speech is complicated.
%    - 4. Error propagation may occur during the cascaded BT-TTS pipeline, making the pseudo parallel data mismatching.

%\skeleton{para3: In this work, we propose xx. }
In this paper, we proposed \textbf{D}iscrete \textbf{U}nit \textbf{B}ack-translation~(\method) to apply back-translation to ST. We adopt HuBERT~\cite{hsu2021hubert} to convert speech to discrete unit and regard discrete unit as a kind of pseudo-language. Instead of using a text-to-speech translation system on unpaired text to produce synthetic speech, we build a text-to-unit model which learns to predict the discrete units rather than continuous value, making it a much easier task and reducing speaker dependency. The trained text-to-units model generates the synthetic discrete units from a large amount of unpaired text and we fulfill the forward translation pass by training the unit-to-text Transformer model on mixture of real and synthetic paired data. Experimental results demonstrate that DUB can bring about 5 bleu improvement over baseline and achieves comparable performance with previous methods in MuST-C dataset and and achieve comparable performance with large-scale multilingual speech or text pre-training methods in CoVoST2 low-source scenes.

Our contributions are as follows:
\begin{itemize}
  \item
  This is the first work to unify the ST and MT framework, by adding a discrete unit extractor for speech.
  \item
  Based on the unified structure, we propose Discrete Unit Back-translation (DUB), which makes a large number of easily-obtained target language texts to be efficiently utilized.
  \item
  Since the discretization process is unsupervised, our method does not rely on transcribed text, friendly for unwritten language.
  \item
  We perform experiments on standard MuST-C benchmark, as well as high-resource and low-resource unwritten sceneries on CoVoST-2. 
\end{itemize}


==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/010_intro_pre2.tex <==
Speech-to-text translation (ST) converts the spoken source language into the written target language, which is a closely related task to machine translation (MT).
In recent years, direct ST that does not rely on intermediate transcription has received considerable attention due to its potential applications in unwritten language scenarios and various domains~\cite{sung2019towards,han-etal-2021-learning,papi2021speechformer,fang2022stemm,ye2022cross}. 
One of the major challenges faced by ST is data scarcity, which is similar to the low-resource scenarios encountered in MT. 
Intuitively, techniques developed for low-resource MT~\cite{xia2019generalized,chen2020facebook,liu2020multilingual,tang2020multilingual} should be utilized to improve ST performance.
In fact, these techniques are hard to be transferred to ST due to the modality gap between speech and text, where ST takes continuous speech as input and MT takes discrete tokens as input.


==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/020_related.tex <==

\noindent\textbf{Speech translation}~
Without using textual transcriptions during inference or training, translating audio directly into the target language is very meaningful for languages that do not have a written form. \citet{berard2016listen} first proposed an end-to-end encoder-decoder architecture for such direct speech-to-text translation. Later, novel models~\cite{di2019adapting,dong2021consecutive,dong2021listen,zheng2021fused} and training techniques, such as multi-task learning~\cite{indurthi2021task,tang2021improving,ye2021end}, knowledge distillation~\cite{liu2019end, dong2021listen}, and pretraining methods~\cite{zheng2021fused, zhang2022speechut}, were developed to improve end-to-end performance. However, these training methods often rely on the use of source text or knowledge from the pre-trained models. 
% \citet{zhang2022revisiting} revisited training end-to-end ST from scratch. 
Without using transcripts or pretraining, \citet{zhang2022revisiting} proposed the parameterized distance penalty to better model speech locality in the self-attention structure and provided results on ST benchmarks covering 23 languages.

\noindent\textbf{Back-translation}~
Back-translation (BT) is a widely used method for improving machine translation systems by training a target-to-source model and creating synthetic parallel data from monolingual target text. This approach has been shown to be effective in both statistical~\cite{bertoldi2009domain,bojar2011improving} and neural machine translation models~\cite{sennrich-etal-2016-improving, edunov-etal-2018-understanding,hoang2018iterative}, and is frequently used to improve translation performance in WMT competitions~\cite{farhad2021findings,wenzek2021findings,adelani2022findings}.
A similar data augmentation idea through synthesizing speech from utterances can be applied to automatic speech recognition (ASR)~\cite{tjandra2017listening, hayashi2018back, ueno2021data}.
However, applying BT in ST is not trivial. \citet{zhang2022ustc} augmented the triplet data by TTS generation from transcription, but the experiment showed that such scaling yields minimal improvement to the final ST model.

\noindent\textbf{Discrete speech representation}~
Discrete speech representations are often studied in the work on self-supervised speech representation learning~\cite{van2017neural,baevski2019vq,baevski2020wav2vec,hsu2021hubert,meng2022cobert}. For example, \citet{van2017neural} proposed Vector Quantised-Variational AutoEncoder (VQ-VAE) to map continuous signals, like speech or image, into a discrete sequence space.
% , and VQ-VAE has yielded promising results for tasks such as subword unit discovery from speech, text-to-speech synthesis~\cite{dunbar2019zero}, and speech-to-speech translation for unwritten languages~\cite{zhang2021uwspeech}.
\citet{hsu2021hubert} proposed HuBERT, which learns self-supervised speech representation by extracting speech features and clustering them offline, and iteratively training the clustering indexes of features at masked locations.
Although the clustered discrete representations are only a by-product of HuBERT, they are used to build the generative spoken language
model~\cite{lakhotia2021generative,kharitonov2022text},
enhance speech representation~\cite{chung2021w2v,meng2022cobert,chen2022wavlm,wu2022wav2seq,zhang2022speechut}, 
and model direct speech-to-speech translation~\cite{lee2022textless,inaguma2022unity}.
% ~\cite{lee2022textless,inaguma2022unity,popuri2022enhanced,huang2022transpeech}.
% One of the benefits of audio discretization is that it allows a wide variety of NLP techniques to be applied to speech data. 
% This is exactly what we practice in our work, where we take speech-to-text translation as an example, unify the model architecture of ST and MT through a discrete unit extractor for speech, and migrate back-translation techniques that are commonly used in MT to ST. 
In the prior literature, probably the most similar task to ours is the textless speech-to-speech translation~\cite{lee2022textless}, but the difference is that they discretized the target-side speech and convert speech-to-speech generation into speech-to-discrete-unit generation, while we discretize the speech at the source side.
\citet{zhang2022speechut} leveraged the discrete unit as an interface to align speech and text, and proposed a unified-modal encoder-decoder pre-training model, SpeechUT.
SpeechUT aims to improve speech representation via the units, while we use the units to construct a unified framework for ST and MT, and to explore transferable training methods from NLP to speech.


==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/030_method.tex <==

\subsection{Problem Formulation}
\label{sec:031_problem}
\input{Sections/031_problem.tex}


\subsection{Model Structure}
\label{sec:032_model_structure}
\input{Sections/032_model_structure.tex}


\subsection{Discrete Unit Back-Translation (\method)}
\label{sec:033_dub}
\input{Sections/033_dub.tex}


\subsection{Generation methods for back-translated units}
\label{sec:034_gen_methods}
\input{Sections/034_generation_methods.tex}

==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/031_problem.tex <==

Unlike cascade systems or existing end-to-end ST work that utilizes speech-transcription-translation triplet $(\mathbf{s},\mathbf{x},\mathbf{y})$, we aim to build and train the model that translates speech directly into text in another language without using the transcription $\mathbf{x}$. 
The training dataset is denoted as $\mathcal{\dsy} =\{(\mathbf{s}, \mathbf{y})\}$.
Also, we introduce the monolingual corpus of the target language $\mathcal{\dy^{\prime}} = \{\mathbf{y^{\prime}}\}$,  enhance the model via the discrete unit back-translation~(\method) method (described in Section~\ref{sec:033_dub}).

% Speech translation datasets usually consist of speech-text-translation triples D={(s,x,y)}\mathcal{D}=\{(\mathbf{s}, \mathbf{x}, \mathbf{y})\}.
% DUB utilizes translation y\mathbf{y} and speech s\mathbf{s} without access to transcript x\mathbf{x}. 
% As a benefit of back translation, DUB is able to leverage large-scale monolingual corpora in the target language ˆY={ˆy}\mathcal{\hat{Y}}=\mathbf{\{\hat{y}\}}, where ˆy\mathbf{\hat{y}} are the target text sentences.

==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/032_model_structure.tex <==

As illustrated in Figure~\ref{fig:u2tt_dub}(a), our model consists of three main components: \textit{discrete unit extractor}, \textit{unit-to-text translation model}, and \textit{text-to-unit translation model}. 
% The discrete unit extractor encodes the speech input into discrete units. 
% The forward-translation~(FT) model θu→y\theta_{u \rightarrow y} performs the units-to-text translation task. It consists of a discrete unit embedding layer and a forward-translation Transformer. 
% The back translation (BT) θy→u\theta_{y \rightarrow u} model has the same structure as the FT model to perform the text-to-unit translation, which is added to incorporate the \method training.
% The back-translation~(BT) model θy→u\theta_{y \rightarrow u}, fulfills text-to-unit translation task. It consists of a text embedding layer and a back-translation Transformer. 

\noindent\textbf{Discrete Unit Extractor}~
The discrete unit extractor converts continuous speech signals into a sequence of discrete units, which we use the Hidden-unit BERT~(HuBERT)~\cite{hsu2021hubert}.
HuBERT is a self-supervised model learned by predicting discrete labels of masked audio segments from k-means clustering on the model's intermediate representations. 
It consists of a stack of 1-D convolutional layers and a Transformer encoder to encode the speech into continuous intermediate representations, and a k-means model to convert the representations into a sequence of cluster indices.
We then remove the adjacent duplicate indices to obtain the discrete units sequence, denoted as $\vecu=(\vecu_1, \vecu_2, \ldots, \vecu_T)$, $\vecu_i \in \{0,1, \ldots, K-1\}$, $\forall 1 \leq i \leq T$, where $K$ is the number of clusters.
% and TT is the number of frames. 
Note that the discrete unit extractor used \textbf{offline} during the pre-processing stage before translation, can be considered as a \textbf{feature extractor}.

\noindent\textbf{Unit-to-Text Translation (U2TT) Model}~
The U2TT model $\theta_{u \rightarrow y}$ performs the forward translation. It consists of a discrete unit embedding layer and a Transformer. 
The discrete unit embedding layer converts discrete units $\vecu$ into the embedding $\ee=(\ee_1, \ee_2, \ldots, \ee_T)$. 
In order to retain more contextual and textual information from HuBERT, we adopt the intermediate representations of HuBERT's k-means cluster centroids as prior knowledge to initialize the unit embedding. 
This initialization operation is referred to as \textit{pre-trained embedding} in the later analysis~(Section~\ref{sec:unit_infoloss}).
The Transformer follows the vanilla Transformer architecture~\cite{vaswani2017attention}, consisting of a Transformer encoder and a Transformer decoder. The encoder takes unit embedding $\ee$ plus sinusoidal positional embedding as input and outputs semantic representation. The decoder generates the translation sequence $\vecy=(\vecy_1, \vecy_2, \ldots, \vecy_{|\vecy|})$ autoregressively based on the semantic representation.

\noindent\textbf{Text-to-Unit Translation (T2UT) Model}~
The T2UT model $\theta_{y \rightarrow u}$ has the same structure as the U2TT model, but with a randomly initialized text embedding layer. It is added to perform the text-to-unit translation and to incorporate the \method training.

% Back-translation~(BT) model converts text sequence into discrete unit sequence, comprised of a random initialized text embedding layer and a standard Transformer model.

% \noindent\textbf{Text Embedding Layer}~
% The text embedding layer converts subword sequence into continuous embedding. The embedding lookup table is initialized randomly.

% \noindent\textbf{Back-Translation Transformer}~
% Back-translation Transformer has the same architecture as forward-translation Transformer.
% It takes subword embedding plus sinusoidal positional embedding as input and generates the discrete unit sequence autoregressively.

%\noindent\textbf{Discrete Unit Encoder}~
%The unit encoder is built by a stack of Transformer blocks~\cite{vaswani2017attention}, consisting of a self-attention layer, a feed-forward layer, normalization layers, and residual connections. It takes unit embedding \boldsymbol{Z}\boldsymbol{Z} plus sinusoidal positional embedding as input and outputs contextual representation \boldsymbol{C}=\left(c_1,c_2,\ldots,c_T\right)\boldsymbol{C}=\left(c_1,c_2,\ldots,c_T\right). 

%\noindent\textbf{Text Decoder}~
%The text decoder is a standard Transformer decoder~\cite{vaswani2017attention} which contains a text embedding layer, stacked Transformer layers, and an output projection layer. It is used to generate the target text sequence \boldsymbol{Y}=\left(y_1,y_2,\ldots,y_Y\right)\boldsymbol{Y}=\left(y_1,y_2,\ldots,y_Y\right) autoregressively based on the discrete unit encoder output \boldsymbol{C}\boldsymbol{C}. 
%\yr{No need to separate encoder-decoder, no need to use different names.}





==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/033_dub.tex <==
% An overview of our proposed \textbf{D}iscrete \textbf{U}nit \textbf{B}ack-translation (DUB) is shown in Figure

\noindent\textbf{Training Steps}~
Given ST parallel dataset $\mathcal{\dsy} =\{(\mathbf{s}, \vecy)\}$, extra target-language corpus $\mathcal{\dy^{\prime}} = \{\vecy^{\prime}\}$, and the discrete unit extractor $E$. 
As shown in Figure\ref{fig:u2tt_dub}(b), the \method training steps are as follows.

\begin{itemize}[itemsep=1pt, leftmargin=12pt, parsep=0pt, topsep=1pt]
  \item[\textbf{1.}]
  Extract unit for each speech input~$\vecu=E(\mathbf{s})$, and get unit-translation pairs~$\mathcal{\duy}=\{(\vecu, \vecy)\}$;
  
  \item[\textbf{2.}]
  Train the T2UT model based on $\mathcal{\duy}$ with cross-entropy loss as in Eq.~(\ref{eq:2});
  
  \item[\textbf{3.}]
  For each text $\vecy^{\prime} \in \mathcal{\dy^{\prime}}$, generate corresponding synthetic units $\hat{\vecu}^{\prime}$ through the BT model~(generation methods will be discussed in Section~\ref{sec:034_gen_methods}).
  Then, add special \texttt{<BT>} indicator at the begining of $\hat{\vecu}^{\prime}$~\cite{caswell2019tagged}. 
  The synthetic units-translation set is denoted as $\mathcal{\duy^{\prime}} =\{(\hat{\vecu}^{\prime}, \vecy^{\prime})\}$;
  
  \item[\textbf{4.}]
  Upsample the original training data by a rate of $r$ and train U2TT model based on $\mathcal{\duy}\union \mathcal{\duy^{\prime}}$ and loss in Eq.~(\ref{eq:1}).
    % = \lvert \duy \rvert / \lvert \duy\union \duy^{\prime} \rvert$;
  % \item[5.]
  % Continue training from model \theta_{u\rightarrow y}^{\ast}\theta_{u\rightarrow y}^{\ast} on \duy\duy and get final system.
\end{itemize}


\noindent\textbf{Training Objective}~
% In DUB, the unit-to-text and text-to-unit translation are both straight-forward. The supervision signal comes from parallel unit-translation pairs. 
The training objectives for U2TT and T2UT models are the negative log-likelihood losses based on the unit-translation pairs:
\begin{align}
     \mathcal{L}_{\text{U2TT}} = -\expect_{(u,y) \in D} \log P\left(\vecy \mid \vecu,\theta_{u\to y}\right)
     \label{eq:1} \\
     \mathcal{L}_{\text{T2UT}} = -\expect_{(u,y) \in D_{u,y}} \log P\left(\vecu \mid \vecy,\theta_{y\to u}\right)
     \label{eq:2}
\end{align}
, where 
$D$ refers to $\mathcal{\duy} \union \mathcal{\duy^{\prime}}$ for \method training, and when $D=\mathcal{\duy}$, Eq.~(\ref{eq:1}) is the loss function for training U2TT from scratch.



==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/034_generation_methods.tex <==
We explore the following generation methods for producing synthetic units: beam search, sampling, and top-k sampling.  We also apply a speech normalization method to remove speaker information when generating units.

\textbf{Beam search} tries to identify the maximum a posteriori~(MAP) output and generate the sentence with the largest estimated probability given an input. 
\textbf{Sampling} means sampling from the distribution randomly at each step, which generates diverse outputs. 
\textbf{Top-k sampling} is a middle ground between beam search and sampling. At each time step, we select the \emph{k} most likely tokens from the output distribution, re-normalize and then sample from this restricted set.

The discrete unit extractor produces various unit sequences for speech with the same content when delivered by multiple speakers~\cite{lee2022textless}.  These variations pose a challenge for training the BT model. In order to address this issue, we adopt a \textbf{Speech Normalization} module from~\cite{lee2022textless}, which removes speaker information from the discrete units and produces norm units. 
% Since the discrete unit extractor produces various unit sequences for the same speech when delivered by multiple speakers, we directly use the speech normalization module in~\cite{lee2022textless}
% \footnote{download at \url{https://dl.fbaipublicfiles.com/fairseq/speech_to_speech/speech_normalizer/en/en_10h.tar.gz}}
Specifically, it is an off-the-shelf HuBERT-CTC model trained on VoxPopuli~\cite{wang2021voxpopuli} that normalizes variant speech input to a single speaker to eliminate such influence (denoted as \textit{Speech Norm}). We implement back-translation with norm units and use the resulting BT model to generate pseudo norm units.


==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/034_pretrains.tex <==
\yr{this part needs to think twice...}
\yr{or we need the figure to show such procedures.}

Through speech discretization, our model unifies the text translation and speech translation frameworks, while other techniques commonly used in MT, such as pre-training, are compatible with our approach.
We explore two pre-training methods for the unit-to-text translation model: cross-modal mBART and unit-ASR \yr{name is weird} pre-training. 

\noindent\textbf{Cross-modal mBART}~ 
mBART\cite{liu2020multilingual} pre-trains a complete sequence-to-sequence model by denoising full texts in multiple languages. 
mBART trains the model to predict original text $\boldsymbol{X}$ given corrupted text $\boldsymbol{g(X)}$, where $\boldsymbol{g}$ is a noising function and $\boldsymbol{X}$ is a mixture of multilingual texts. 
Following mBART, our cross-modal mBART is trained with a Transformer encoder-decoder architecture. We treat the mixture of discrete units $\boldsymbol{D_{units}}$ extracted from unlabeled speech data and unlabeled text $\boldsymbol{D_{text}}$ in the target language as $\boldsymbol{X}$
 and use sentence permutation and word-span masking strategies as $\boldsymbol{g}$.  Formally, we aim to minimize
\begin{equation*}
    \mathcal{L}_\theta=\sum_{\mathcal{D}_i \in \mathcal{D}} \sum_{X \in \mathcal{D}_i} \log P(X \mid g(X) ; \theta)
\end{equation*}
, where $\mathcal{D}=\left\{\mathcal{D}_{unit}, \mathcal{D}_{text}\right\}$, $g(\cdot)$ is the noising function by randomly masking some discrete tokens, and $\boldsymbol{P}$\yr{params are $\theta$} is defined by the cross-modal mBART model. 


 
\noindent\textbf{Unit-ASR}~
According to \cite{wang-etal-2020-fairseq}, a pre-trained ASR encoder is essential for speech translation models. 
Unit-ASR has the same objective function as ASR, where the model needs to predict the transcripts based on the input sequence. 
Particularly, unit-ASR takes discrete units as input. Similarly, we pre-train the discrete unit pre-net, discrete unit encoder and text decoder with parallel units-transcripts pairs $(\boldsymbol{U},\boldsymbol{X})$, converted from speech-transcript pairs $(\boldsymbol{S},\boldsymbol{X})$ by the discrete units extractor. The training objective is negative log-likelihood on units-transcripts pairs as the loss function. 
\begin{equation*}
    \mathcal{L}_{unit-ASR}=-E_{(U,X)} \log P(X|U)
\end{equation*}
Different from previous encoder-only ASR pre-training, we utilize pre-trained unit-ASR complete encoder-decoder architecture for DUB pre-training.



==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/040_exps.tex <==


\subsection{Datasets}
\label{sec:041_datasets}
\input{Sections/041_datasets.tex}


\subsection{Experimental setups}
\input{Sections/042_setups.tex}

\subsection{Baseline models}
\label{sec:043_baselines}
\input{Sections/043_baselines.tex}


\input{Tables/mustc.tex}

\input{Tables/covost_high_resource.tex}
\input{Tables/covost_low_resource.tex}

\subsection{Main results on Speech-to-text Translation}
\input{Sections/044_main_results.tex}





==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/041_datasets.tex <==

\noindent\textbf{MuST-C}~
MuST-C\footnote{All released under CC BY NC ND 4.0 International\label{fn:data}}~\cite{di2019must}, one of the most widely-used ST benchmarks, contains translations from English to 8 languages collected from TED talks.
We train and validate our approach in three ST directions: English-German~(En-De), English-French~(En-Fr), and English-Spanish~(En-Es).


\noindent\textbf{CoVoST-2 X-En}~
CoVoST-2~\cite{wang2021covost} is a multilingual ST corpus derived from the Common Voice project, which offers translations from English to 15 languages and from 21 languages to English.
% One notable feature of our method is that it does not require transcription, making it particularly suited for speech translation from written language. Since resources for unwritten languages are often scarce, 
We conducted experiments on X-En, including high-resource languages~($\geq$ 10 hours of speech) such as French~(Fr) and German~(De), and low-resource languages~($\leq$ 2 hours of speech), like Arabic~(Ar), Swedish~(Sv), Japanese~(Ja), etc.
Without the need for transcription, the evaluation focuses on the capability of our method to generalize to the low-resource unwritten multi-languages. 
% Details about CoVoST-2 X-En are shown in Table.


\noindent\textbf{Monolingual text corpus}~
Monolingual target-language text corpora are introduced for back-translation. 
For MuST-C we include 48M German, 79M French and 64M Spanish sentences sampled from TED~\cite{duh18multitarget}, WMT~\cite{bojar-EtAl:2016:WMT1} and CCMartix~\cite{schwenk2019ccmatrix} datasets for En-De/Fr/Es respectively.
% Details about monolingual data are shown in Table.
% For MuST-C En-De experiments, we concatenate parallel English-German corpus provided by WMT and randomly sample 48M German sentences as monolingual data. 
% Similar operations are applied to obtain 79M French and 64M Spanish sentences for En-Fr and En-Es experiments respectively.
% We repeat the same process to extract 79M French sentences for English-French (En-Fr) and 64M Spanish sentences for English-Spanish (En-Es) experiments. 
For CoVoST-2 X-En experiments, we introduce 1M extra English sentences sampled from the transcriptions of Common Voice Corpus 11.0~\cite{ardila-etal-2020-common}.

All statistics of the datasets are in Appendix~\ref{sec:app:data statistics}.
% For CoVoST-2 X-En experiments, we provide 10M English sentences as monolingual data, which is composed of 1M English sentences from Common Voice Corpus 11.0 English transcriptions and 9M English sentences randomly sampled from WMT parallel English-German corpus.

==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/042_setups.tex <==
\noindent\textbf{Pre-processing}~
The model accepts 16-bit 16KHz mono-channel raw waveform speech and then discretizes them into units.
We denote the discrete units clusters by the numbers (\textit{e.g.} $\#1$, $\#2$), and combining with the target-language sentences, we learn the joint vocabulary via SentencePiece~\cite{kudo-richardson-2018-sentencepiece}. We set the joint vocabulary size to 8000 for both MuST-C and CoVoST-2. 
% More details are in Appendix.

\noindent\textbf{Model Configuration}~
For MuST-C experiments, we use the HuBERT-base\footnote{\url{https://dl.fbaipublicfiles.com/hubert/hubert\_base\_ls960.pt}} (pre-trained on Librispeech without fine-tuning) with a 500-cluster k-means quantizer based on the 9th layer representation as the \textit{discrete unit extractor}.
For CoVoST-2, we employ the mHuBERT\footnote{\url{https://dl.fbaipublicfiles.com/hubert/mhubert_base_vp_en_es_fr_it3.pt}} with a 1000-cluster k-means quantizer based on the 11th layer representations pre-trained on the VoxPopuli~\cite{wang2021voxpopuli} speech in English, Spanish, and French.
The U2TT and T2UT models have the same model architecture, consisting of a 12-layer Transformer encoder and a 6-layer Transformer decoder, with hidden size $d=768$, $16$ attention heads, and $4096$ FFN hidden states. 
Additionally, we implement the \textsc{Base} and \textsc{Large} versions of the model, with hidden sizes of 768 and 1024, respectively. Both versions are performed in the main experiments, while in the analysis, we primarily investigate the \textsc{Base} model.
More information on model size and scalability experiments can be found in Appendix~\ref{sec:app:ana_model_data_size}.

%For CoVoST-2 Xx-En experiments, we train all 21 X-to-English language pairs in a multi-task learning setup. \yr{this is not multi-task. We train a multi-lingual Xx-En model covering 21 translation directions.}

% \noindent\textbf{Training Details}~
% For MuST-C experiments, we train FT and BT models of each translation direction under bilingual settings. 
% For CoVoST-2 Xx-En experiments, we train a multi-lingual Xx-En model covering 21 translation directions. Appendix B contains more details about training settings.

\noindent\textbf{Evaluation}~
We evaluate the models using case-sensitive sacreBLEU\footnote{\url{https://github.com/mjpost/sacrebleu}, \textbf{BLEU Signature}:
nrefs:1 | bs:1000 | seed:12345 | case:mixed | eff:no | tok:13a | smooth:exp | version:2.0.0}~\cite{post2018call} on the MuST-C \texttt{tst-COM} sets and CoVoST-2 test sets.


See Appendix~\ref{sec:app:experimental_deatils} for more details on vocabulary learning, training, and test.



==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/043_baselines.tex <==
We compare our method with the baselines as listed in Table~\ref{tab:mustc} $\sim$ \ref{tab:covost_low}~(Appendix~\ref{sec:app:baseline_models} for details). In particular, we explain the following baselines that do not involve transcriptions during training.

\noindent\textbf{Revisit ST}~\cite{zhang2022revisiting}
is a direct speech-to-translation model with parameterized distance penalty (PDP) and CTC regularization. Its framework and training objectives are sorely different from ours.

\noindent\textbf{Unit-to-text Translation~(U2TT)}~
has the structure as described in Section~\ref{sec:032_model_structure} and is trained using only speech-translation supervision from the ST dataset from scratch, without applying \method. As a baseline, comparison with this model helps to see the influence of~\method.

\noindent\textbf{Transformer-ST}~
stands for training the Speech-Transformer~\cite{dong2018speech} from scratch, but without ASR pre-training as in the previous work~\cite{wang-etal-2020-fairseq, inaguma2020espnet, zhao2021neurst}. The training details are in Appendix~\ref{sec:app:baseline_models}.


% For a fair comparison, we set a hidden size of 768, which makes the model size larger than baselines like Fairseq ST~\cite{wang-etal-2020-fairseq} while keeping roughly the same parameter size as ours.

% stands for training speech-Transformer model from scratch, unlike 
% We implement a Transformer-based speech translation baseline using speech-translation pairs \{(\mathbf{s}, \mathbf{y})\}\{(\mathbf{s}, \mathbf{y})\} without access to any other data at training. The model takes fbank80 features as input and consists of two 2D convolutions layers and a standard Transformer model. 
% Note that Transformer-ST is trained with the same parameters as DUB.


% \textit{<discrete unit,translation>} pairs in training set without help of any other data.






%Compare with: \\
%\noindent\textbf{}~
%  1. Baseline Speech transformer model. w/ or w/o ASR pretrain\\
%  2. Cascaded Back-translation-TTS model. ? 10M?\\
%1. SOTA TTS\\
%2. Unit-vocoder\\
%3. unit2de (only mustc) with Load pretrained  monolingual target-language bart decoder (10M de)\\
%  \\
%    To show BT or pretrain decoder, which is better?
    

==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/044_main_results.tex <==
\noindent\textbf{MuST-C}~
As shown in Table~\ref{tab:mustc}, compared to the methods that do not involve the transcribed text, our method, U2TT~(\textsc{Large}) with \method, gets the best ST results by introducing extra target-language text, and \method obtains an average boost of 5.5 BLEU compared with U2TT in the three En-X directions.
Encouragingly, we find that our method achieves comparable performance to previous models that utilize transcriptions through multi-task learning or pre-training.
As for the baseline, U2TT outperforms the Transformer-ST, where we believe that the discrete units still retain the semantic information of the audio feature (\textit{e.g.} log Mel-filter bank, \textit{abbr.} Fbank) for translation. 
As for the gap between our method and the SoTA system, we argue that SpeechUT~\cite{zhang2022speechut} performed various mask-predict pre-training tasks using extra 1.4k hours of speech and parallel MT data from WMT, which is not included in our approach.

\noindent\textbf{CoVoST-2}~
% We evaluate the proposed DUB on Xx-En 21 language pairs. We divide 21 language pairs into high-resource and low-resource groups.
Our method performs similarly to MuST-C on the high-resource En-X~(Table~\ref{tab:covost_high}).
Without considering auxiliary data or pre-training methods, adding only 1M additional English text, \method improves by an average of 2.1 BLEU over 7 language pairs compared to U2TT, and by an average of 3.4 BLEU over the cascaded ST system.
For the low-resource setting, our method can bring improvement on almost every language pair and achieve better performance than the large-scale multilingual speech or text pre-training models, like XLS-R+mBART-50 model~\cite{babu2021xls}, with much fewer parameters. 
The discrete unit extractor is unsupervised, so our method does not require transcriptions, which is particularly advantageous for unwritten ST. 
This experiment mimics such low-resource nature of unwritten languages in practice. The results also show that the U2TT model and the DUB training have the potential to translate low-resource unwritten languages.
% Note that on both high and low-resource language pairs, even without BT, U2TT can outperform existing work that does not rely on large-scale multilingual pretraining, which means the discrete units can still retain the semantic information of the original speech for translation.

% There is still a gap between \method and state-of-the-art~(SoTA) systems, but it should be noted that they utilize more data and various pre-training tasks, which are indeed helpful to learn better speech representations and improve ST performance. For example, 
% the SoTA MuST-C system SpeechUT~\cite{zhang2022speechut} designed various mask-predict pre-training tasks and trained using extra 1.4k hours of speech and parallel MT data from WMT.
% The SoTA CoVoST2 system mSLAM\cite{bapna2022mslam} is pre-trained on unlabeled speech in 51 languages, unlabeled text in 101 languages and 32-language ASR data with 2 billion parameters.
% , much larger than 1M monolingual English text used in \method.
%\yr{We need to mention SOTA, and tell the reviewer they used much more data}



==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/050_dub_analysis.tex <==
\subsection{Is DUB better than other methods that leverage extra raw data? }
\label{sec:utilize_raw_text}
\input{Sections/051_utilize_raw_text.tex}


% \subsection{Diverse pseudo-units are needed}
\subsection{The better the pseudo-unit, the more effective the DUB method?}
\label{sec:pseudo_unit_quality}
\input{Sections/052_pseudo_unit_quality.tex}

% This section seeks to answer the question of whether DUB is a more efficient method than other non-parallel text based enhancement strategies for improving ST, and further examines if the rules of BT in MT can be applied to DUB.


==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/051_utilize_raw_text.tex <==
\input{Tables/utilize_raw_text.tex}

The key benefit of the \method is to make use of a lot of monolingual text.
Here, alternative techniques such as pseudo-labeling and pre-training (implemented as Cascaded BT and Bi-modal BART) 
are also evaluated on the MuST En-De translation, by introducing an equivalent corpus of 10 million German sentences.
\begin{itemize}[itemsep=1pt, leftmargin=10pt, parsep=0pt, topsep=1pt]
    \item 
    \textbf{Cascaded BT}~ 
    aims to build a target-to-source MT-TTS pipeline to construct pseudo-speech translation augmented data for the training.
    Specifically, we use transcription-translation pairs of MuST-C to train a back-translation MT model and use the released FastSpeech2\footnote{\url{https://github.com/ming024/FastSpeech2}}~\cite{ren2020fastspeech} and a HiFi-GAN~\cite{kong2020hifi} vocoder for TTS generation. 
    % Cascaded BT system is used to convert 10M unpaired target-language text to synthetic source-language speech, which can be used in combination with authentic parallel data to augment performance of Transformer-ST.
    \item 
    \textbf{Bi-modal BART}~
    has the same structure as U2TT, and is pre-trained by denoising large-scale corrupted discrete units and monolingual text, following the recipe of mBART~\cite{liu2020multilingual}.
    We combine the 10M additional text with 7M discrete units extracted from 10k hours of speech in GigaSpeech~\cite{chen2021gigaspeech} to pre-train the model and fine-tune it based on MuST-C unit-translation pairs. 
    See Appendix~\ref{sec:app:experimental_deatils} for training details.
\end{itemize}

As shown in Table~\ref{tab:utilize_raw_text} introducing equivalent raw text, \textbf{DUB is superior to the above two approaches and has a greater potential to exploit monolingual raw text}. 
We find that the gain from \textit{cascaded BT}-synthesized speech is limited because the synthetic speech is robotic and monotonic, making it easy to overfit the model to the synthetic pairs. 
Although the bi-modal BART pre-training can bring about 2 BLEU improvements, it is still inferior to DUB. 
We attribute this to the gap between the denoising pre-training task and the downstream generation tasks, while DUB does not have such a gap.
Meanwhile, we observe that combination of bi-modal BART and DUB can bring further performance improvements, which indicates that they are complementary to each other.
% At the pre-training stage, the bi-modal BART takes noisy units or text as input and conducts a denoising task whereas at finetuning stage the model takes complete units as input and is required to generate corresponding text. 


==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/052_pseudo_unit_quality.tex <==

In Section~\ref{sec:033_dub}, we presented four generation methods to create synthetic pseudo-units based on the BT model, namely beam search, sampling, top-k sampling, and speech normalization. 
In the experiments, we set a beam size of 5 for the beam search, k=10 for top-k sampling, and use an off-the-shelf speech normalizer\footnote{\url{https://dl.fbaipublicfiles.com/fairseq/speech_to_speech/speech_normalizer/en/en_10h.tar.gz}} from \citet{lee2022textless} for Speech Norm. 

Does the forward model gain more from synthesized pairs when the synthesized units are of higher quality?
We calculate the Unit Error Rate (UER) on the MuST-C validation set to assess the synthesis quality.   
A lower UER indicates that the generated units are closer to the directly extracted units, \textit{i.e.} of higher quality. 
We systematically vary the back-translated data from 1M to 10M, and present the BLEU scores and UERs of the generation methods in Table~\ref{tab:bt_uer} and Figure~\ref{fig:bt_strategy}. 
The \textit{Speech Norm} module produces the highest quality synthesized units, while the sampling-based methods have lower quality. Interestingly, the sampling method with the lowest synthesis quality has the most significant improvement over the forward model.

We conjecture that \textbf{the richness and irregularity of the synthesized data can better improve the forward ST model}, while regular pseudo-units, \textit{e.g.} generated by MAP-based beam search, are more predictable and not conducive to performance improvement. 
This is consistent with previous findings of BT techniques in machine translation~\cite{edunov-etal-2018-understanding}.
In addition, \textbf{\textit{Speech Norm}, which normalizes speech to a single speaker, is not necessary for our \method method}. 
Although such an operation makes the ST model easier to learn and the UER smaller, it compromises the diversity of the synthetic data, which is also not helpful for performance improvement. The model generalization ability weakens when these single-speaker synthesis units increase. 

\input{Tables/bt_uer.tex}

\begin{figure}[htb]
    % \setlength{\abovecaptionskip}{-0.cm}
    % \setlength{\belowcaptionskip}{-0.6cm}
    \centering
    \includegraphics[width=0.87\linewidth]{Figures/dub_bt_strategy_bleus.pdf}
    \caption{MuST-C En-De \texttt{tst-COM} BLEU scores for the increasing amounts of BT data (1M, 5M, and 10M), obtained using different generation methods. Note that the unit extractor of \textit{Speech Norm} is mHuBERT, so without extra text, the BLEU score is 20.9, which is slightly higher than HuBERT, but the gap is quite small.
    % \yr{figures may change later.}
    }
    \label{fig:bt_strategy}
\end{figure}




==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/054_model_data_size.tex <==



% \textbf{5.1 BLEU vs amount of monolingual data}\\
% plot 
% \textbf{5.2 model size vs. BLEU}\\
% - When data size is small .....\\
% - When we use a large amount of data, we need a larger model. ....\\

How does model size affect the results of our method? How much improvement does the raw text in the target language bring to our method? To this end, we take MuST-C English-German translation as an example. We set the model size to 73M, 176M and 260M parameters respectively (the specific hyperparameter settings are shown in Table~\ref{tab:model_size}), and introduce extra 1M, 10M, and 48M German sentences.

Figure~\ref{fig:data_model_size} shows the BLEU scores of different sizes of models, with different amounts of monolingual back-translation data added.
In general, regardless of the model size, introducing \textbf{more text brings better performance}. When we introduce a large amount of back-translated data, \textbf{the larger model gets significantly better performance}. We find that when no or less back-translated data is introduced, the performance of the large model is instead not optimal. This is because the large model is prone to overfitting when the original training data is small, but as the monolingual data is gradually introduced, the advantage of the large model becomes obvious, without replying to the transcription, introducing 48M back-translated pairs, the model with 260M parameters can boost up to 6.1 BLEU on En-De.


\begin{table}[htb]
    \small
    \centering
    \begin{tabular}{lc|ccc}
        \toprule
         & \textbf{Model} & \textbf{Encoder} & \textbf{Decoder} & \textbf{Hidden} \\
         & \textbf{Params} & \textbf{Layers} & \textbf{Layers} & \textbf{Dim}\\
        \midrule
        \textbf{\circled{1}}\textsc{Small} & \textbf{73M} & 6 & 6 & 512 \\\hline
        \textbf{\circled{2}}\textsc{Base} & \textbf{176M} & 12 & 6 & 768 \\\hline
        \textbf{\circled{3}}\textsc{Large} & \textbf{260M} & 12 & 6 & 1024 \\
        \bottomrule
    \end{tabular}
    \caption{Hyper-parameter settings for the models in Figure~\ref{fig:data_model_size}.}
    \label{tab:model_size}
\end{table}

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/dub_data_model_size_bleus_2.pdf}
    \caption{MuST-C En-De \texttt{tst-COM} BLEU scores for different amounts of target-language text data are introduced, under different model sizes.}
    \label{fig:data_model_size}
\end{figure}



==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/060_unit_analysis.tex <==
% To explore why DUB can boost improvement, we assess the properties of units in both FT and BT processes. 
% If discrete units are suitable input features for ST, then it is feasible to unify the frameworks of ST and MT through discrete units. Furthermore, if BT process can generate credible discrete units, then it is viable to enhance the FT process through back-translated unit-text pairs.
Why does DUB work? To answer this question, we examine the properties of the discretized speech unit. Specifically, (1) do the units make sense to replace the original speech input in the forward translation process? (2) Do the units generated by back translation also contain semantic information and can they even restore the speech?

\subsection{Are discrete units suitable features for ST input?}
\label{sec:unit_infoloss}
\input{Sections/061_infoloss.tex}

\subsection{Can we recover faithful speech from pseudo-units?}
\label{sec:text-to-speech translation}
\input{Sections/062_TTS_trans.tex}




==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/061_infoloss.tex <==


We show how much semantic information is retained for different input forms by comparing the results of the downstream ST task~(shown in Table~\ref{tab:discrete_infoloss}).
Training from scratch, we find that the U2TT model translates better than Transformer-ST~(19.9 \textit{vs.}18.0), 
indicating that \textbf{compared to the speech feature, like Fbank, the discrete unit is a better choice for input and has no information loss in terms of the semantic information required for translation.}
We assume that this is strongly correlated with the HuBERT-based discrete unit extractor, since HuBERT is designed to learn a combined acoustic and language model over the continuous speech input, which preserves much textual information for the speech.
But rigorously, compared to the continuous representation of HuBERT, the discretization procedure does suffer from semantic information loss. Comparing Line~\RNum{2} and \RNum{3}, there is a gap of 2.9 BLEU between U2TT and HuBERT-Transformer (where frozen HuBERT Layer-9 continuous representation is taken as input to perform ST), in terms of ST metrics. 
Fortunately, the gap can be compensated by 
\begin{inparaenum}[\itshape a)\upshape]
    \item initializing the unit embedding as its corresponding K-means cluster centroid on continuous HuBERT representations as described in Section~\ref{sec:032_model_structure}~(denoted as pre-trained embedding, Line~\RNum{4}), which can slightly close the gap by 0.5 BLEU;
    and
    \item simply introducing only 1M additional text and applying \method, which can achieve 2.7 BLEU improvement (Line~\RNum{5} \textit{vs.} \RNum{4}).
\end{inparaenum}


\input{Tables/discretize_infoloss.tex}

% We contend that the decline in performance can be attributed to the discretization process.

==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/062_TTS_trans.tex <==

Do the back-translated units capture the semantics of the target language text? 
Since it is difficult to directly evaluate the correctness of the pseudo-units generated by the back-translation model, we concatenate a unit-based HiFi-GAN vocoder\footnote{\url{https://dl.fbaipublicfiles.com/fairseq/speech_to_speech/vocoder/code_hifigan/mhubert_vp_en_es_fr_it3_400k_layer11_km1000_lj/g_00500000}} with our back-translation model to recover speech from the generated pseudo-units, thus completing the text-to-speech~(TTS) translation task.
TTS generation quality is measured by ASR-BLEURT, where we transcribe the speech output using a high-quality open-source ASR model\footnote{\url{https://huggingface.co/facebook/wav2vec2-large-960h-lv60-self}} and calculate BLEURT\footnote{\url{https://github.com/google-research/bleurt}} with reference transcription.% compare it with the reference transcription to compute SacreBLEU~\cite{post2018call}. 
As shown in Table~\ref{tab:tts_translation}, the ASR-BLEURT of beam search and sampling is 0.6 and 0.47 respectively, indicating that \textbf{the unit sequence back-translated from a given target language text can convey its general semantic meaning, which is the guarantee for the success of \method.}
We conduct the listening test by checking 30 randomly sampled BT-recovered speeches for semantic consistency with ground-truth. 22 of 30 sentences matched ground-truth speech, while the remaining 8 had minor issues, with only 1 being of low quality and the other 7 missing or repeating 1-2 details.
We also provide some generated audio samples in Appendix~\ref{sec:app:cases_tts_translation} to help illustrate the degree of speech restoration.

\input{Tables/tts_translation.tex}

% In this way, we can perform text-to-speech translation by translating text in one language into speech in another language and analyze if back-translated units can capture the proper semantics.


==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/070_conclusion.tex <==
In this paper, we propose \textbf{D}iscrete \textbf{U}nit \textbf{B}ack-translation (DUB), as well as the \textbf{U}nit-\textbf{to}-\textbf{T}ext \textbf{T}ranslation (U2TT) model for direct speech translation.
Our approach successfully migrates the back-translation technique from MT to ST by discretizing the speech signals into unit sequences and making use of extra widely accessible text in the target language. 
Without using transcription, \method can achieve an average increase of 5.5 BLEU on MuSTC En-De/Fr/Es over the raw U2TT framework, and achieves comparable performance to the large-scale speech-text joint pre-training models on CoVoST-2 low-resource ST.
The analysis experiments also show the potential of such discrete audio units as inputs and outputs for text or speech generation tasks.




==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/080_broaderImpact.tex <==
Our proposed model structure with a discrete unit extractor for speech and the unit-to-text translation model, which does not need any transcriptions during training, is particularly relevant for speech translation for more than 3,000 languages and dialects in the world that cannot be transcribed.
Since these unwritten languages are typically low-resource, we emphasize that boosting ST performance via text-to-unit back-translation data augmentation, \textit{i.e.} \method, is very promising.
Meanwhile, as a by-product of \method, TTS translation has significant implications for assisting visually impaired or dyslexic people in understanding the world as well as preserving low-resource unwritten spoken languages.

However, as exploratory work, we focus on investigating the potential of using BT to enhance ST performance, while popular large-scale pre-training methods are not employed in this paper. 
This makes our method slightly inferior to these methods in terms of performance, perhaps.
But promisingly, in terms of structure, the model is more general across various modalities and also has more potential to integrate with the methods in NLP area (might be the topic of future research). 
Also, the models are still far from real industrial applications. For example, the data used for training is much smaller than the scale in reality, while the real speech is noisier and more complex than the open-source dataset, which may require front-end processing.
Moreover, the success of our method is partly attributable to the HuBERT representation, which contains certain textual information for the speech, and via experiments, we also find that the quality of discrete units influences the translation performance. Nevertheless, learning meaningful discrete units is not the primary goal of HuBERT pre-training, and how to learn discrete units or representations for speech with more \textit{contextual} semantic information can be explored in the future. 
% Furthermore, it is also valuable to investigate the integration of discrete units with transcriptions through techniques such as CTC loss and multi-task learning.


==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/085_acknowledgments.tex <==
We thank Fuliang Weng for the careful guidance and revisions to the paper and thank all the anonymous reviewers for their insightful and valuable comments.

==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/091_experimental_details.tex <==
\noindent\textbf{Vocabulary}~
We apply the SentencePiece\footnote{\url{https://github.com/google/sentencepiece}}~\cite{kudo-richardson-2018-sentencepiece} to tokenize the text and discrete units into subwords.  
We add all the discrete units as special symbols to the joint vocabulary. 
The joint subword tokenizer is learned on all the translation sentences and discrete unit sequences in the ST training set.
The vocabulary size is 8000 for both MuST-C and CoVoST-2 experiments. Specifically, 
for MuST-C experiments, since the number of K-means clusters is 500,  the vocabulary is composed of 500 special unit symbols and 7500 text subwords. 
For CoVoST2 X-En experiments, the vocabulary consists of 1000 special unit symbols representing 1000 clusters of mHuBERT,
and 7000 text subwords.

\noindent\textbf{Training details}~
We use Adam optimizer with $\beta_1=0.9, \beta_2=0.98$, and 4k warm-up updates to optimize the parameters in our model. We train the model with a batch size of 5k tokens. The learning rate is 7e-4 and we apply an inverse square root schedule. 
The value of label smoothing is set to 0.1. 
The up-sampling rate $r$ in DUB is set to 32, given the huge volume differences between the BT data and the original data.
For MuST-C experiments, we train U2TT and T2UT models of each translation direction under bilingual settings. 
For CoVoST-2 X-En experiments, we train a multi-lingual X-En model covering 21 translation directions, distinguished by the language tags of the units in different languages.
We implement our models based on
Fairseq\footnote{\url{https://github.com/facebookresearch/fairseq}}~\cite{ott2019fairseq} codebase.
All models are trained on 8 Nvidia Tesla-V100 GPUs and take about 400k steps to converge.
During inference, We save the checkpoint with the best BLEU on the validation set and average the last 10 checkpoints. 
We use beam search with a beam size of 5 for each translation direction.

\noindent\textbf{Training details for Bi-modal BART}~
The training of bi-modal BART follows the recipe of mBART~\cite{liu2020multilingual}. We implemented a mask rate of 0.3, with the replacement of the masked tokens by random tokens at a probability of 0.1. Additionally, the mask length was determined through sampling from a Poisson distribution, with a lambda parameter of 3.5.










==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/092_cases_tts_translation.tex <==


In Table \ref{tab:cases_tts_translation}, we show two cases of German-English text-to-speech translation on MuST-C En-DE \textsc{tst-COM} set.
In CASE 1, our text-to-speech translation system generates speech with the same content and a similar spectrogram as reference speech.
In CASE 2, the synthetic speech deviated slightly from the reference speech, but the translation is correct --- ``release'' has the same meaning as ``shoveling out'' and ``all the time '' just means ``all along''.
The samples of generated audio are included in \url{https://anonymous.4open.science/r/DUB/ttss_samples}.

\clearpage
\begin{table*}[]
    \small
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|p{13.cm}}
        \toprule
        & \textbf{German:} Einzige Land der Welt. \\
         
        & \textbf{Ref:} the only country in the world.\\
        &  
        \begin{minipage}[t]{\textwidth}
            \vspace{0pt}
            {\includegraphics[width=0.9\textwidth]{Figures/Ref_the_only_country_in_the_world.pdf}}
        \end{minipage} \\
        
        \textbf{CASE 1} & \textbf{Hyp:} the only country in the world.\\
        &
         \begin{minipage}[t]{\textwidth}
            \vspace{0pt}
            {\includegraphics[width=0.9\textwidth]{Figures/Hyp_the_only_country_in_the_world.pdf}}
        \end{minipage} \\
        
        
        \midrule
         % & \makecell{\textbf{German:} Und sicher, hätten wir diese diese Hydranten die ganze Zeit freischaufeln können, und viele Menschen tun das.} \\
         & \textbf{German:} Und sicher, hätten wir diese diese Hydranten die ganze Zeit freischaufeln können, und viele Menschen tun das. \\
         
          & \textbf{Ref:} And certainly, we could have been shoveling out these fire hydrants all along, and many people do.\\
        &
        \begin{minipage}[t]{\textwidth}
            \vspace{0pt}
            {\includegraphics[width=0.9\textwidth]{Figures/Ref_we_could_have_been_shoveling_out_those_fire_hydrants.pdf}}
        \end{minipage} \\
        
        \textbf{CASE 2} & \textbf{Hyp:} And certainly we could have released those hydrants all the time and many people do that.\\
        &
         \begin{minipage}[t]{\textwidth}
            \vspace{0pt}
            {\includegraphics[width=0.9\textwidth]{Figures/Hyp_we_could_have_been_shoveling_out_those_fire_hydrants.pdf}}
        \end{minipage} \\
        
        \bottomrule
    \end{tabular}
    
    }
    \caption{Cases of De-En text-to-speech translation on MuST-C En-De \texttt{tst-COM} set. 
    % The title of spectrogram is the corresponding transcription.
    }
    
    \label{tab:cases_tts_translation}
\end{table*}

==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/093_baseline_models.tex <==
% \noindent\textbf{U2TT}~
% We implement the BASE and LARGE version, the same as \method BASE and LARGE respectively.

\noindent\textbf{Existing ST Systems}~
We list the ST systems we compared with on different datasets:
\begin{itemize}[itemsep=1pt, leftmargin=10pt, parsep=0pt, topsep=1pt]
    \item 
    \textbf{MuST-C}~
    In Table~\ref{tab:mustc}, we compare our method with the following: Fairseq ST~\cite{wang-etal-2020-fairseq}, NeurST~\cite{zhao2021neurst}, Espnet ST~\cite{inaguma2020espnet}, E2E-ST-JT~\cite{du2022regularizing}, Speechformer~\cite{papi2021speechformer}, Cascaded ST~\cite{inaguma2020espnet}, MTL~\cite{tang2021improving}, Self-training~\cite{pino2020selfa}, SpeechT5~\cite{ao2022speecht5},  SpeechUT~\cite{zhang2022speechut} and Revisit ST~\cite{zhang2022revisiting}.
    
    \item
    \textbf{CoVoST X-En high resource}~
    In Table~\ref{tab:covost_high}, we compare our method with several baselines from \cite{wang2021covost}, including Transformer-ST, Transformer-ST + ASR pre-train and Cascaded ST, and Revisit ST~\cite{zhang2022revisiting}.
    
    \item
    \textbf{CoVoST X-En low resource}~
    In Table~\ref{tab:covost_low}, we compare our method with several existing ST methods, including Transformer-ST, Transformer-ST + ASR pre-train from~\cite{wang2021covost} and  large-scale multilingual speech or text pre-training methods: XLS-R~\cite{wu2022wav2seq}, Wav2seq~\cite{wu2022wav2seq}, XLS-R+mBART-50~\cite{babu2021xls}, LNA-E,D~\cite{li2021multilingual}.
    Note that XLS-R is pre-trained on 436K hours of speech across 128 languages.
    % and mSLAM~\cite{bapna2022mslam}.
\end{itemize}

\noindent\textbf{Transformer-ST for MuST-C}~
For a fair comparison, we keep the parameters roughly the same size as \method, setting two covolutional layers, a 12-layer Transformer encoder and a 6-layer Transformer decoder, with hidden size $d=768$, $16$ attention heads, and $4096$ FFN hidden states, which makes the model size larger than baselines like Fairseq ST~\cite{wang-etal-2020-fairseq}, NeurST~\cite{zhao2021neurst}, and Espnet ST~\cite{inaguma2020espnet}.

==> [ACL2023]DUB_ discrete unit back-translation for ST/Sections/094_comparision_with_cascaded_system.tex <==
It could be argued that our model employs a cascaded architecture, comprising a unit extractor and a unit-to-text translation model.
The traditional cascade ST system (ASR+MT) can also be enhanced through applying back-translation to improve its MT model. 

In Table \ref{tab:comaprision_with_cascaded}, we compare the performance of DUB with the BT-enhanced cascaded ST system both utilizing 10M unpaired text.
By comparison, we can find that the BLEU score of the U2TT model is inferior to that of the cascaded system when utilizing 10 million unpaired text samples. This discrepancy can likely be attributed to the higher baseline performance of the cascaded system. Additionally, DUB demonstrates a superior relative improvement in BLEU score compared to the cascaded system. Moreover, the discrete unit extractor is obtained through unsupervised training on unlabeled speech, which requires no transcriptions compared with the ASR system trained on speech-transcription pairs.


\begin{table}[]
    \centering
    % \small
    \begin{tabular}{l|c|ccc}
        \toprule
        \textbf{Method} & \textbf{Extra Text} & \textbf{BLEU} & \textbf{$\Delta$BLEU}\\
        \midrule
        U2TT & - & 20.4 & -\\
        \quad w/ DUB & \checkmark & 25.0 & 4.6\\
        \midrule
        Cascaded ST & - & 23.1 & - \\
        \quad w/ MT-BT & \checkmark & 26.0 & 2.9 \\
        \bottomrule
        
    \end{tabular}
    \caption{MuST-C En-De \texttt{tst-COM} BLEU for U2TT and cascaded system. MT-BT refers to enhancing MT model of cascaded ST through back-translation. Cascaded ST is trained by ourselves on MuST-C En-De \texttt{train} set. The same extra text corpus with 10 million German sentences is used for both methods.}
    \label{tab:comaprision_with_cascaded}
\end{table}

==> [ACL2023]DUB_ discrete unit back-translation for ST/Tables/bt_uer.tex <==
\begin{table}[htb]
    % \setlength{\abovecaptionskip}{-0.cm}
    \setlength{\belowcaptionskip}{-0.2cm}
    % \small
    \centering
    \begin{tabular}{lrr}
        \toprule
         & \textbf{UER(\%)} & \textbf{$\Delta$BLEU}\\
        \midrule
        Speech Norm & 73.0 & 0.7 \\
        Beam Search & 83.0 & 1.7 \\
        Top-10 Sampling & 89.0 & 3.6\\
        Sampling & 92.0 & 4.6 \\
        \bottomrule
    \end{tabular}
    \caption{The quality of generated pseudo-units using different generation methods and their BLEU increases from 10M extra texts,  evaluated by \textbf{Unit Error Rate (UER)} on MuST-C En-De \texttt{Dev}, the smaller the better. 
    % ^\diamondsuit^\diamondsuit: we directly apply the speech normalization model in \citet{lee2022textless} to unify the discrete units of multiple speakers of a speech to a single speaker by an ad-hoc CTC model.
    }
    \label{tab:bt_uer}
\end{table}

==> [ACL2023]DUB_ discrete unit back-translation for ST/Tables/covost_high_resource.tex <==
\begin{table*}[]
    % \setlength{\abovecaptionskip}{-0.cm}
    % \setlength{\belowcaptionskip}{-0.4cm}
    \small
    \centering
    \begin{tabular}{l|cc|ccccccc|c}
        \toprule
        & \multicolumn{2}{c|}{\textbf{Aux. Data}} & \\
        \textbf{Methods} & \textbf{ASR} & \textbf{Text} & \textbf{Fr} & \textbf{De} & \textbf{Es} & \textbf{Ca} & \textbf{It} & \textbf{Ru} & \textbf{Zh} & \textbf{Avg.} \\
        \midrule 
        Transformer-ST$^{\dagger}$ & - & - & 
        4.3 & 8.4 & 12.0 & 14.4 & 0.2 & 1.2 & 1.4 & 8.8 \\
        Transformer-ST + ASR pre-train$^{\dagger}$ & \checkmark & - &
        26.3 & 17.1 & 23.0 & 18.8 & 11.3 & 14.8 & 5.8 & 16.7 \\
        
        Cascaded ST$^{\dagger}$ & \checkmark & - & 
        27.6 & \textbf{21.0} & 27.4 & 21.3 & 13.5 & 16.8 & \textbf{7.0} & 19.2\\
        
        Revisit ST~\cite{zhang2022revisiting} & - & - & 
        26.9 & 14.1 & 15.7 & 17.2 & 2.4 & 3.6 & 2.0 & 11.7 \\
        \midrule
        U2TT~(\textsc{Large}) & - & - &
        27.4 & 16.7 & 28.1 & 23.1 & 20.0 & 21.9 & 5.9 & 20.5 \\
        \quad w/ \method & - & \checkmark1M &
        \textbf{29.5} & 19.5 & \textbf{30.9} & \textbf{25.2} & \textbf{23.9} & \textbf{23.2} & 6.1 & \textbf{22.6} \\
        % \method & & 10M & 31.0 & 22.1 & 32.0 & 27.2 & 25.2 & 26.3 & 6.2 & \textbf{24.3} \\
        \bottomrule
    \end{tabular}
    \caption{Test BLEU scores on CoVoST-2 X-En language pairs with more than 10 hours of speech.
    Auxiliary data refers to all data at training excluding \textit{<speech,translation>} pairs.
    $^{\dagger}$: Results from \cite{wang2021covost}. Random sampling is the decoding strategy for DUB.
    % \yr{Here, we do not consider the work that takes advantage of joint speech-text pre-training from even larger-scale monolingual text, raw audio or ASR data.}
    }
    \label{tab:covost_high}
\end{table*}

==> [ACL2023]DUB_ discrete unit back-translation for ST/Tables/covost_low_resource.tex <==
% \begin{table*}[]
%     \small
%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{l|cc|cccccccccccc|c}
%         \toprule
%         & \multicolumn{2}{c}{\textbf{Aux. Data}}& \textbf{Et} & \textbf{Mn} & \textbf{Nl} & \textbf{Tr} & \textbf{Ar} & \textbf{Sv} & \textbf{Lv} & \textbf{Sl} & \textbf{Ta} & \textbf{Ja} & \textbf{Id} & \textbf{Cy} & \textbf{Avg.} \\
%         \textbf{Methods} & \textbf{ASR} & \textbf{Text} & 
%         3h & 3h & 7h & 4h & 2h & 2h & 2h & 2h & 2h & 1h & 1h & 2h & - \\
%         \midrule
%         Transformer-ST†^{\dagger} &  - & - &
%         0.1 & 0.1 & 0.3 & 0.7 & 0.3 & 0.2 & 0.1 & 0.3 & 0.3 & 0.3 & 0.4 & 0.3 & 0.3 \\
%         Transformer-ST + ASR pre-train†^{\dagger} & \checkmark & - &
%         0.1 & 0.2 & 3.0 & 3.6 & 4.3 & 2.7 & 2.5 & 3.0 & 0.3 & 1.5 & 2.5 & 2.7 & 2.2 \\
%         \midrule
%         \multicolumn{12}{l}{
%         \textit{Larger models based on large-scale multilingual speech, text or joint pre-training, involving more data}} \\
%         % HuBERT-large & 0.6 & 0.4 & 3.6 & 3.4 & 5 & 4.4 & 2.8 & 2.6 & 0.4 & 1.7 & 2.3	& 3.2 & 2.5 \\
%         XLS-R (0.4B)♢^{\diamondsuit} & \checkmark & - & 
%         0.6 & 0.3 & 3.5 & 3.7 & 8.1 & 5.3 & 3.1 & 5.3 & 0.0 & 2.0	& 3.3 & 3.4 & 3.2\\
%         XLS-R + mBART-50 (0.7B)♢^{\diamondsuit} & \checkmark & \checkmark & 
%         3.5 & 0.4 & 22.0 & 4.6 & 3.0 & 10.3 & 6.0 & 6.6 & 0.2 & 0.6 & 1.4 & 2.5 & 5.1 \\
%         Wav2seq (0.4B)~\cite{wu2022wav2seq} & \checkmark & - &
%         2.4 & 0.3 & 12.2 & 4.5 & 10.5 & 8.8 & 4.8 & 5.9 & 0.0 & 1.9 & 5.0 & 5.7 & 5.2 \\
%         XMEF-X + mBART-50 (0.7B)♢^{\diamondsuit} & \checkmark & \checkmark & 
%         2.5 & 1.2 &24.0 & 9.4& 6.4 & 4.0 &5.0 & 5.6& 0.9 & 1.0& 2.8 & 8.1 & 5.9 \\
%         % mSLAM~(2B)~\cite{bapna2022mslam}∗^{\ast} & \checkmark & \checkmark & 
%         % 22.6 & 0.8 & 37.6 & 24.2 & 19.3 & 38.5 & 26.8 & 32.3 & 0.6 & 3.3 & 8.8 & 6.7 & 18.5 \\
%         \midrule
%         U2TT & - & - &
%         1.5 & 0.5 & 6.9 & 3.4 & 7.0 & 8.0 & 6.3 & 6.8 & 0.3 & 1.6 & 6.6 & 2.7 & 4.3 \\
%         \quad w/ \method & - & \checkmark 1M & 
%         1.8 & 0.4 & 10.0 & 5.2 & 6.9 & 8.7 & 6.9 & 7.6 & 0.5 & 2.0 & 6.6 & 5.5 & 5.2 \\
%         %\method (+10M mono) \yr{?} & 1.8 & 0.4 & 10.0 & 6.6 & 7.2 & 7.9 & 7.0 & 6.6 & 0.3 & 1.8 & 7.3 & 5.3 & 5.2 \\
%         % \textit{SoTA: Use larger model and }} \\
%         % mSLAM~(2B)~\cite{bapna2022mslam}^{\dagger}^{\dagger} & 
%         % 22.6 & 0.8 & 37.6 & 24.2 & 19.3 & 38.5 & 26.8 & 32.3 & 0.6 & 3.3 & 8.8 & 6.7 & 18.5 \\
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Test BLEU scores on CoVoST 2 low-resource Xx-to-En language pairs. Auxiliary data refers to all data at training excluding \textit{<speech,translation>} pairs. †^{\dagger}: Results from \cite{wang2021covost}.
%     ♢^\diamondsuit: Results from \cite{babu2021xls}. ∗^\ast is the state-of-the-art system, pre-trained on unlabeled speech in 51 languages, unlabeled text in 101 languages, and 32-language ASR data with 2 billion parameters.}
%     \label{tab:covost_low}
% \end{table*}

\begin{table*}[]
    % \setlength{\abovecaptionskip}{-0.cm}
    \setlength{\belowcaptionskip}{-0.4cm}
    \small
    \centering
    % \resizebox{\textwidth}{!}{
    \begin{tabular}{l|cc|cccccccc|c}
        \toprule
        & \multicolumn{2}{c}{\textbf{Aux. Data}}& \textbf{Ar} & \textbf{Sv} & \textbf{Lv} & \textbf{Sl} & \textbf{Ta} & \textbf{Ja} & \textbf{Id} & \textbf{Cy} & \textbf{Avg.} \\
        \textbf{Methods} & \textbf{ASR} & \textbf{Text} & 
        2h & 2h & 2h & 2h & 2h & 1h & 1h & 2h & - \\
        \midrule
        Transformer-ST$^{\dagger}$ &  - & - &
        0.3 & 0.2 & 0.1 & 0.3 & 0.3 & 0.3 & 0.4 & 0.3 & 0.3 \\
        Transformer-ST A2E$^{\dagger}$ &  - & - &
        0.6 & 0.6 & 0.4 & 1.2 & 0.1 & 0.2 & 0.3 & 2.6 & 0.8 \\
        Transformer-ST + ASR pre-train$^{\dagger}$ & \checkmark & - &
        4.3 & 2.7 & 2.5 & 3.0 & 0.3 & 1.5 & 2.5 & 2.7 & 2.4 \\
        \midrule
        \multicolumn{12}{l}{
        \textit{Larger models based on large-scale multilingual speech, text or joint pre-training, involving more data}} \\
        XLS-R (0.4B)$^{\ast}$ & \checkmark & - & 
        8.1 & 5.3 & 3.1 & 5.3 & 0.0 & 2.0	& 3.3 & 3.4 & 3.8 \\
        Wav2seq (0.4B)$^{\ast}$ & \checkmark & - &
        \textbf{10.5} & 8.8 & 4.8 & 5.9 & 0.0 & 1.9 & 5.0 & \textbf{5.7} & 5.3 \\
        XLS-R + mBART-50 (0.7B)$^{\diamondsuit}$ & \checkmark & \checkmark & 
        3.0 & \textbf{10.3} & 6.0 & 6.6 & 0.2 & 0.6 & 1.4 & 2.5 & 3.8 \\
        LNA-E,D (0.7B)$^{\spadesuit}$ & \checkmark & \checkmark & 
        3.7 & 5.9 & 4.6 & 4.6 & \textbf{0.7} & 1.7 & 2.9 & 2.8 & 3.4 \\
        % mSLAM~(2B)~\cite{bapna2022mslam}∗^{\ast} & \checkmark & \checkmark & 
        % 22.6 & 0.8 & 37.6 & 24.2 & 19.3 & 38.5 & 26.8 & 32.3 & 0.6 & 3.3 & 8.8 & 6.7 & 18.5 \\
        \midrule
        U2TT~(\textsc{Large}) & - & - &
        7.0 & 8.0 & 6.3 & 6.8 & 0.3 & 1.6 & 6.6 & 2.7 & 4.9 \\
        \quad w/ \method & - & \checkmark 1M & 
        7.1 & 8.9 & \textbf{6.9} & \textbf{7.9} & 0.5 & \textbf{2.1} & \textbf{7.0} & \textbf{5.7} & \textbf{5.8} \\
        \bottomrule
    \end{tabular}
    % }
    \caption{Test BLEU scores on CoVoST-2 low-resource X-En language pairs with less than 2 hours of speech. $^{\dagger}$: results from~\cite{wang2021covost}.
    $^{\ast}$:
    results from~\cite{wu2022wav2seq}
    $^\diamondsuit$: results from~\cite{babu2021xls}. $^\spadesuit$: results from~\cite{li2021multilingual}. The numbers in parentheses are their parameter sizes.
    Random sampling is the decoding strategy for DUB.
    % ∗^\ast is the state-of-the-art system, pre-trained on unlabeled speech in 51 languages, unlabeled text in 101 languages, and 32-language ASR data with 2 billion parameters.
    }
    \label{tab:covost_low}
\end{table*}



==> [ACL2023]DUB_ discrete unit back-translation for ST/Tables/discretize_infoloss.tex <==
\begin{table}[]
    % \setlength{\abovecaptionskip}{-0.cm}
    \setlength{\belowcaptionskip}{-0.5cm}
    % \small
    \centering
    \begin{tabular}{cl|l}
        \toprule
        \textbf{No.} & \textbf{Methods} &   \textbf{BLEU} \\
        \midrule
        % Cascaded ST \yr{need?} & 23.x \\
        \RNum{1} & Transformer-ST & 18.0 \\
        \RNum{2} & HuBERT + Transformer  & 22.8 \\
        \midrule
        % \circled{3} \method & 48M & 25.8 \\
        \RNum{3} & U2TT & 19.9 \\
        % \circled{5} \quad - kmeans init. & 1M & 22.0 \\
        \RNum{4} & $\hookrightarrow$ w/ pre-trained embedding & 20.4$^{\ast}$ \\
        \RNum{5} & \qquad $\hookrightarrow$ w/ \method-1M & 23.1 \\
        
        % \method  w/o BT & ×\times & 19.9 \\
        % \quad + Kmeans init. & ×\times & 20.4  \\
        % \midrule
        % \method & 1M &  22.7 (?) \\
        % \quad + Kmeans init. & 1M & 23.1 \\
        % \method & 5M \\
        \bottomrule
    \end{tabular}
    \caption{BLEU scores on MuST-C En-De \texttt{tst-COM} set. 
    % HuBERT + Transformer means that frozen HuBERT Layer-9 continuous representation is taken as input to perform ST. pre-trained embedding refers to initializing the unit embedding as its corresponding K-means cluster centriod on continuous HuBERT representations. 
    DUB-1M means to introduce 1M unpaired text via the DUB method.
    $^\ast$:~the improvement over U2TT is statistically significant~($p<0.05$)}
    \label{tab:discrete_infoloss}
\end{table}

==> [ACL2023]DUB_ discrete unit back-translation for ST/Tables/model_size.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{c|c|ccc}
        \toprule
         & Model & Encoder & Decoder &   \\
         & Params & Layers & Layers & Hidden \\
        \midrule
        \textcircled{1} & 73M & 6 & 6 & 512 \\
        \textcircled{2} & 176M & 12 & 6 & 768 \\
        \textcircled{2} & 260M & 12 & 6 & 1024 \\
        \bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

==> [ACL2023]DUB_ discrete unit back-translation for ST/Tables/mustc.tex <==
\begin{table}[t]
    % \setlength{\abovecaptionskip}{-0.cm}
    \setlength{\belowcaptionskip}{-0.5cm}
    \centering
    % \small
    \resizebox{1.05\linewidth}{!}{
    \begin{tabular}{l|ccc|c}
        \toprule
        \textbf{Method} & \textbf{De} & \textbf{Fr} & \textbf{Es} & \textbf{Avg}. \\
        \midrule
        \multicolumn{5}{l}{\textit{Methods that utilize transcriptions}} \\
        Fairseq ST~\cite{wang-etal-2020-fairseq} &  22.7 &  32.9 &  27.2 & 27.6 \\
        NeurST~\cite{zhao2021neurst} & 22.8 & 33.3 & 27.4 & 27.8 \\
        Espnet ST~\cite{inaguma2020espnet} & 22.9 & 32.8 & 28.0 & 27.9\\
        E2E-ST-JT~\cite{du2022regularizing} & 23.1 & 32.8 & 27.5 & 27.8 \\
        Speechformer~\cite{papi2021speechformer} & 23.6 & - & 28.5 & - \\

        Cascaded~\cite{inaguma2020espnet} & 23.6 & 33.8 & 28.7 & 28.7\\
        MTL~\cite{tang2021improving} & 23.9 & 33.1 & 28.6 & 28.5 \\
        Self-training~\cite{pino2020selfa} & 25.2 & 34.5 & - & - \\
        SpeechT5~\cite{ao2022speecht5} & 25.2 & \textbf{35.3} & - & - \\
        % XSTNet-Base~\cite{ye2021end} & 25.5 & 36.0 & 29.6  \\
        % SpeechUT~\cite{zhang2022speechut}^{\ast}^{\ast} & 30.1 & 33.6 & 41.4 \\ 
        % FAT-ST~\cite{zheng2021fused} & 25.5 & - & 30.8 \\
        % ConST~\cite{ye2022cross} & 25.7 & 36.8 & 30.4 \\
        % STEMM~\cite{fang2022stemm} & 28.7 &  37.4 &  31.0 \\
        % STPT~\cite{tang2022unified} & 29.2 &  39.7 & 33.1 \\
        \midrule
        \multicolumn{5}{l}{\textit{Methods that do not involve transcriptions}} \\
        Revisit ST~\cite{zhang2022revisiting} & 23.0 & 33.5 & 28.0 & 28.2\\
        Transformer-ST &  18.0 & 28.5 & 24.1 & 23.5 \\
        % \quad + BART-decoder \\
        % HuBERT(freeze)-Transformer & 22.8\\
        %Cascade-BT ST & \\
        U2TT~(\textsc{Base}) & 20.4 & 30.3 & 25.3 & 25.3 \\
            \quad\quad w/ \method & 25.8 & 34.7 & 30.2 & 30.2 \\
        U2TT~(\textsc{Large}) & 20.5 & 30.1 & 24.7 & 25.1\\
        %\quad + cross-modal mBART pre-train & 22.4 & 31.4 & 26.3 \\
        %\method (\textsc{Base}) & 25.8 \\
        \quad\quad w/ \method & \textbf{26.2} &  \textbf{35.3} & \textbf{30.4} & \textbf{30.6} \\
        \midrule
        \multicolumn{5}{l}{\textit{SoTA: use much more speech and various pre-training tasks}} \\
        SpeechUT~\cite{zhang2022speechut}$^{\ast}$ & 30.1 & 41.4 & 33.6 & 35.0 \\ 
        \bottomrule
        
    \end{tabular}
    }
    \caption{BLEU Scores on MuST-C En-X \texttt{tst-COM} set. $\ast$ is the state-of-the-art system, which designed various mask-predict pre-training tasks and trained using extra 1.4k hours of speech and parallel MT data from WMT. Random sampling is the decoding strategy for DUB.}
    \label{tab:mustc}
\end{table}

==> [ACL2023]DUB_ discrete unit back-translation for ST/Tables/tts_translation.tex <==
\begin{table}[htb]
    % \setlength{\abovecaptionskip}{-0.cm}
    \setlength{\belowcaptionskip}{-0.5cm}
    \centering
    % \small
    \begin{tabular}{l|ccc}
        \toprule
        \textbf{Generation Method} & \textbf{ASR-BLEURT} \\
        \midrule
        % beam search & 17.6 \\
        beam search & 0.60 \\
        sampling & 0.47 \\
        \bottomrule
        
    \end{tabular}
    \caption{MuST-C En-De \texttt{tst-COM} ASR-BLEURT for text-to-speech translation}
    \label{tab:tts_translation}
\end{table}

==> [ACL2023]DUB_ discrete unit back-translation for ST/Tables/utilize_raw_text.tex <==
\begin{table}[]
    % \setlength{\abovecaptionskip}{-0.cm}
    \setlength{\belowcaptionskip}{-0.5cm}
    \centering
    \small
    \resizebox{\linewidth}{!}{
    \begin{tabular}
    {l|cc|ccc}
        \toprule & \multicolumn{2}{c|}
        {\textbf{Aux. Data}} & \\
        \textbf{Method} & 
        \textbf{Speech} & 
        \textbf{Text} & 
        \textbf{BLEU} \\
        \midrule
        Transformer-ST & - & - & 18.0 \\
        \quad w/ Cascaded BT & - & 10M & 20.3 \\
        \midrule 
        U2TT & - & - & 20.4 \\
        \quad w/ Bimodal BART & 10k\textbf{h} & 10M & 22.4 \\
        \quad w/ \method & - & 10M & 25.0 \\
        \quad w/ Bimodal BART + \method & 10k\textbf{h} & 10M & 25.4 \\
        \bottomrule
        
    \end{tabular}
    }
    \caption{MuST-C En-De \texttt{tst-COM} BLEU scores for different methods that utilize 10M monolingual text data in ST. 
    Transformer-ST and U2TT are described in Section~\ref{sec:043_baselines}.
    % Cascaded-BT performs back-translation using a cascaded system composed of a target-to-source MT model and a TTS model to generate synthetic parallel data to augment Transformer-ST. Bi-modal BART applies mBART-style pre-training on discrete unit and text. And it is loaded as the pre-train model for U2TT. DUB-10M means utilizing 10M unpaired text through DUB.
    }
    \label{tab:utilize_raw_text}
\end{table}

==> [ACL2023]DUB_ discrete unit back-translation for ST/def.tex <==
% !TEX root = main.tex
\newcommand{\pad}{\ensuremath{\langle\text{pad}\rangle}\xspace}
\newcommand{\sentpair}{(\vecs, \vect)\xspace}
\newcommand{\seq}{(\vecx, \vecy)\xspace}
\newcommand{\vecP}{\ensuremath{\mathbf{P}}\xspace}

\newcommand{\delay}{\langle \varepsilon \rangle\xspace}
\newcommand{\pixyofst}{\pi^\star_{\vecx, \vecy} ((\vecs, \vect))\xspace}
\newcommand{\pixy}{\pi^\star_{\vecx, \vecy}\xspace}
\newcommand{\pixyabofst}{\pi^\star_{\vecx, \vecy, \alpha, \beta} ((\vecs, \vect))\xspace}
\newcommand{\pixyab}{\pi^\star_{\vecx, \vecy, \alpha, \beta}\xspace}
\newcommand{\piofs}{\pi^\star_{\vecx, \vecy, \alpha, \beta}(s)\xspace}
\newcommand{\piofsi}{\pi^\star_{\vecx, \vecy, \alpha, \beta}(s_i)\xspace}

\newcommand{\tuple}[1]{\ensuremath{\langle {#1} \rangle}}
%\newcommand{\argmax}[2]{\ensuremath{\mbox{argmax}_{#1}\ {#2}}}

\newcommand{\featuresum}[1]{\ensuremath{\sum_i \lambda_i f_i({#1})}}

\newcommand{\fvec}[1]{\ensuremath{\vec{f} ({#1})}}

\newcommand{\fiof}[1]{\ensuremath{f_i ({#1})}}

\newcommand{\fofi}[0]{\ensuremath{f_i}}

\newcommand{\featureprod}[1]
{\ensuremath{\vec{\lambda} \cdot \fvec{#1} } }

\newcommand{\efprod}[1]{\ensuremath{e^{\featureprod{#1}}}}
\newcommand{\efsum} [1]{\ensuremath{e^{\featuresum {#1}}}}

\newcommand{\lami}{\ensuremath{\lambda_i}}

\newcommand{\empExp}[1]{\ensuremath{\mbox{\~{E}} [{#1}]}}
\newcommand{\expect}{\ensuremath{\mathbb{E}}}

\newcommand{\ks}{\ensuremath{k}}
\newcommand{\Ks}{\ensuremath{K}}
\newcommand{\kbest}{\ks-best\xspace}
\newcommand{\topk}{top-\ks\xspace}
\newcommand{\kBest}{\Ks-Best\xspace}

\newcommand{\notes}[1]{}%{\it {\small {#1}}}}

\newcommand{\acite}[1]{({--#1})}

\newcommand{\define}[1]{{\bf Definition.} {\em {#1}}}
\newcommand{\zerobar}{\ensuremath{\overline{0}}\xspace}
\newcommand{\onebar}{\ensuremath{\overline{1}}\xspace}

\newcommand{\Items}{\ensuremath{\mathcal{I}}\xspace}

\newcommand{\oplusk}{\ensuremath{\oplus_{\tiny k}}}
\newcommand{\otimesk}{\ensuremath{\otimes_{\tiny k}}}

\newcommand{\zerok}{\ensuremath{\overline{0}^k}\xspace}
\newcommand{\onek}{\ensuremath{\overline{1}^k}\xspace}

\newcommand{\scalar}{\ensuremath{\odot_k}}

\newcommand{\kdim}{\ks-dimensional\ }


\newcommand{\nextfunc}{\operatornamewithlimits{\mathrm{next}}}



% \newlistof{defin}{def}{List of Definitions}

% \newcommand{\defin}[1]{%
% \refstepcounter{defin}
% \par\noindent\textbf{Definition \thedefin. #1}
% \addcontentsline{ans}{defin}{\protect\numberline{\thedefin}#1}\par}

% for amsthm
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}

%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{definition}[theorem]{Definition}

\newcommand{\gc}{\ensuremath{|G|}\xspace}
\newcommand{\ntsize}{\ensuremath{|N|}\xspace}
\newcommand{\nt}{\ensuremath{N}\xspace}
\newcommand{\rulepernt}{\ensuremath{R}\xspace}

\newcommand{\Ttimesk}{\ensuremath{T_{\otimesk}}\xspace}
\newcommand{\Tplusk}{\ensuremath{T_{\oplusk}}\xspace}
\newcommand{\maxk}{\ensuremath{\mbox{\bf max}_k}\xspace}

\newcommand{\tenexp}[1]{\ensuremath{10^{{-#1}}}\xspace}

\newcommand{\naive}{na\"{\i}ve\xspace}

\newcommand{\perc}[1]{\ensuremath{{#1}\%}\xspace}

\newcommand{\veca}{\ensuremath{\mathbf{a}}\xspace}
\newcommand{\vecb}{\ensuremath{\mathbf{b}}}
\newcommand{\vecp}{\ensuremath{\mathbf{p}}}
\newcommand{\klogk}{\ensuremath{k\log k}}
\newcommand{\vecz}{\ensuremath{\mathbf{z}}}
\newcommand{\vech}{\ensuremath{\mathbf{h}}}
\newcommand{\vecW}{\ensuremath{\mathbf{W}}}
\newcommand{\vecs}{\ensuremath{\mathbf{s}}\xspace}
% \newcommand{\vecs}{\mathbf{s}\xspace}
\newcommand{\vect}{\ensuremath{\mathbf{t}}\xspace}
\newcommand{\veco}{\ensuremath{\mathbf{o}}\xspace}
\newcommand{\better}{\ensuremath{\preceq}}


\newcommand{\opt}{\ensuremath{\mbox{{\bf min}}_\better}}
\newcommand{\mergek}{\ensuremath{\mbox{{\bf merge}}_{\better k}}\xspace}
\newcommand{\multk}{\ensuremath{\mbox{{\bf mult}}_{\better k}}\xspace}

\newcommand{\kw}{\ensuremath{\mathbf{w}}}

\newcommand{\kwi}{\ensuremath{w_i}}
\newcommand{\wejv}[3]{\ensuremath{w^{#1}_{{#2}}({#3})}}

\newcommand{\vecj}{\ensuremath{\mathbf{j}}}
\newcommand{\vecD}{\ensuremath{\mathbf{D}}}
\newcommand{\vecu}{\ensuremath{\mathbf{u}}\xspace}
\newcommand{\vecU}{\ensuremath{\mathbf{U}}}
\newcommand{\vecjhat}{\ensuremath{\hat{\mathbf{j}}}}
\newcommand{\vecone}{\ensuremath{\mathbf{1}}}
\newcommand{\dbp}[2]{\ensuremath{\langle{#1}, {#2}\rangle}}

\newcommand{\reviewtimetoday}[3]{
    \AtBeginDocument{
    \special{
    !userdict begin
    /pagenum 0 def
    /bop-hook
    {
        /pagenum pagenum 1 add def
        pagenum #3 le
        {
        gsave
        430 750 translate
        0 rotate
        0.4 setgray
        /Times-Roman findfont
        10 scalefont setfont
        0 0   moveto
        (#1) show
        0 -10 moveto
        (#2) show
        grestore
        } if
    } def
    }  }}

% for submission
\iffalse
\renewcommand{\marginpar}[1]{}
\fi

%\newcommand{\comment}[1]{\marginpar{\raggedright{\em{\small #1}}}}

\newcommand{\ith}[1]{\ensuremath{i^{{th}}}}
\def\alglazy{Algorithm 3}

\newcommand{\JnM}{Jim\'enez and Marzal\xspace}

%\newcommand{\ind}[1]{\ensuremath{^{(#1)}}}
\newcommand{\srule}[1]{\ensuremath{\mathrm{#1}}}
\newcommand{\goesto}{\ensuremath{\rightarrow}\xspace}
\newcommand{\chn}[1]{\mbox{{\it {#1}}}}

\newcommand{\ngram}{\ensuremath{\text{$n$-gram}}\xspace}
\newcommand{\ngrams}{\ensuremath{\text{$n$-grams}}\xspace}

\newcommand{\ngramitem}[5]{
\ensuremath{
\left(
\begin{smallmatrix}
\mbox{\small {#4}} &\cdots & \mbox{\small {#5}} \\
&
%\!\!_{#2}
\mbox{#1}
%_{#3}
 &
\\ {#2} & & {#3}
\end{smallmatrix}
 \right)
}}

\newcommand{\specialngramitem}[7]{
\begin{math}
\left(
\begin{smallmatrix}
\mbox{\small {#2}}\ \cdots\ \mbox{\small{#3}}
& \cdots &
\mbox{\small {#4}}\ \cdots\ \mbox{\small {#5}} \\
& \mbox{{#1}} & \\
{#6} & & {#7}
\end{smallmatrix}
 \right)
\end{math}
}

\newcommand{\chartitem}[3]{
\ensuremath{(\mbox{#1},{#2},{#3})}
}

\newcommand{\vtnt}[1]{\ensuremath{V_{\mbox{\tiny #1}}}}
%%% \bigram{a}{b} means (a,b) is a bigram pair. P (b | a)!
\newcommand{\bigram}[2]{\ensuremath{\Pr(\mbox{\small #2} \mid \mbox{\small #1})}}

\newcount\permx
\newcount\permy
\def\permdot#1#2{
\permx=#1 \advance\permx by-1
\permy=#2 \advance\permy by-1
\psframe[fillcolor=black, fillstyle=solid]
(\permx,\permy)(#1, #2)
}

%%% note: realcalc.sty has a fatal bug : 23-0.5=23.5.
%%% so i have to do this... +1-0.5 thing
\newcommand{\minushalf}[1]{
    \Radd{\aaa}{#1}{-1}
    \Radd{\aaa}{\aaa}{0.5}
    \Rtrunc{\aaa}{1}{\aaa}
    \aaa
}


\newcommand{\permnt}[3]{
\rput({#1},{#2}){\huge\color{white} {#3}}
}


\newcommand\union{\cup}
\newcommand\intersect{\cap}

\newcommand\vecd[2]{\ensuremath{d_{#2}{(#1)}}}
\newcommand\veczero{\ensuremath{\mathbf{0}}}
\newcommand\vecq{\ensuremath{\mathbf{q}}}
\newcommand\vecn{\ensuremath{\mathbf{n}}}
%\newcommand\vecone{\ensuremath{\mathbf{1}}}
% \newcommand{\argmax}{\operatornamewithlimits{\mathbf{argmax}}}
\newcommand{\argtop}{\operatornamewithlimits{\mathbf{argtop}}}
\newcommand{\toptop}{\operatornamewithlimits{\mathbf{top}}}
% \newcommand{\argmin}{\operatornamewithlimits{\mathbf{argmin}}}

\newcommand{\deltahat}{\ensuremath{\hat{\delta}}\xspace}

\newcommand{\xrs}{{\bf xRs}\xspace}
\newcommand{\xrsln}{\mbox{1-{\bf xRLNs}}\xspace}
\newcommand{\RLN}{{\bf RLN}\xspace}

\newcommand{\x}[1]{\ensuremath{x_{#1}}\xspace}
\newcommand{\foot}[1]{\ensuremath{^{\tiny({#1})}_{\downarrow}}}


\newcommand{\chnprd}{{\tiny \ensuremath{_{\circ}}}}

%\newcommand{\ckyitem}[3]{\ensuremath{(_{#2}{\mbox{#1}}_{#3})}\xspace}
%\newcommand{\ckyitem}[3]{\ensuremath{({\mbox{#1}}_{#2, #3})}\xspace}
\newcommand{\ckyitem}[3]{\ensuremath{{\mbox{#1}}_{{{#2},\,{#3}}}}\xspace}
\newcommand{\treeitem}[2]{\ensuremath{{\mbox{#1}}_{#2}}\xspace}
\newcommand{\nodent}[3]{\ensuremath{\treeitem{#1}{#2}:{#3}}}

\newcommand{\coverage}[1]{\ensuremath{(\mbox{{#1}})}\xspace}
\newcommand{\lmcov}[2]{\ensuremath{(\mbox{#1}, ^{\mbox{\scriptsize #2}}\!)}\xspace}
\newcommand{\phritem}[3]{\ensuremath{\coverage{#1}:({#2}, \mbox{\footnotesize ``#3''})}\xspace}
\newcommand{\lmphritem}[4]{\ensuremath{\lmcov{#1}{#2}:({#3}, \mbox{\footnotesize ``#4''})}\xspace}
\newcommand{\phrpair}[2]{\ensuremath{\langle \mbox{\chn{#1}, {#2}}\rangle}\xspace}

\newcommand{\lmitem}[3]{\ensuremath{({{#1}}^{#2 \star #3})}\xspace}
%\newcommand{\lmckyitem}[5]{\resizebox{!}{.15in}{\ensuremath{(\mbox{\small #1}_{\mbox{\tiny\ {#2},{#3}}}^{\tiny\ \mbox{#4}\ \star\ \mbox{#5}})}}\xspace}
\newcommand{\lmckyitem}[5]{\ensuremath{(\mbox{#1}_{\mbox{\scriptsize\ ({#2},{#3})}}^{\scriptsize\ \mbox{#4}\ \star\ \mbox{#5}})}\xspace}

\def\wlm{+LM\mathord+\textrm{LM}\xspace}
\def\wolm{−LM\mathord-\textrm{LM}\xspace}

\newcommand{\sym}[1]{\textrm{#1}\xspace}
\newcommand{\VP}{\sym{VP}}
\newcommand{\PP}{\sym{PP}}

\newcommand{\startsym}{\mbox{\scriptsize \texttt{<s>}}\xspace}
\newcommand{\stopsym}{\mbox{\scriptsize \texttt{</s>}}\xspace}
\newcommand{\TOP}{\sym{TOP}}
%\newcommand{\plm}[2]{\ensuremath{P_{lm}(\mbox{\small #2}\mid\mbox{\small #1})}}
\newcommand{\plm}[2]{\ensuremath{P_{lm}(\mbox{#2}\mid\mbox{#1})}}

%\newcommand{\order}[1]{\ensuremath{\mathcal{O}(#1)}}
\newcommand{\order}{\ensuremath{\mathcal{O}}}

\newcommand{\wocombo}{\ensuremath{h}\xspace}
\newcommand{\mincombo}{\ensuremath{h_{\mathit{combo}}}\xspace}

% \renewcommand{\min}{\ensuremath{\mbox{\bf min}}\xspace}
\newcommand{\hyp}[1]{\mbox{\tiny ``{#1}''}}
\newcommand{\hl}{\ensuremath{k}\xspace}


\newcommand{\cand}{\ensuremath{\mathit{cand}}\xspace}
\newcommand{\buf}{\ensuremath{\mathit{buf}}\xspace}
\newcommand{\bound}{\ensuremath{\mathit{bound}}\xspace}

\newcommand{\lazyjbest}{\ensuremath{\textproc{LazyJthBest}}\xspace}

\newcommand{\backwardstar}{\ensuremath{\mathit{IN}}\xspace}

\newtheorem{proposition}[theorem]{Proposition}

\newcommand{\ff}{\ensuremath{\mathbf{f}}\xspace}
\newcommand{\ee}{\ensuremath{\mathbf{e}}\xspace}
\newcommand{\al}{\ensuremath{\mathbf{a}}\xspace}

\newcommand{\pt}{\ensuremath{p_{\mbox{t}}}}
\newcommand{\pd}{\ensuremath{p_{\mbox{d}}}}


\newcommand{\current}{\color{blue}{\fbox{{\bf C}}}\xspace}
\newcommand{\future}{\color{red}{\fbox{{\bf F}}}\xspace}

\newcommand{\boxnum}[1]{{\setlength{\fboxsep}{1pt}\raisebox{1pt}{\hspace{1pt}\fbox{\tiny #1}\hspace{1pt}}}}
\newcommand{\ind}[1]{\ensuremath{_{\kern-0.5pt\boxnum{#1}}}}
\newcommand{\BS}{\ensuremath{\mathit{IN}}\xspace}
\newcommand{\NTX}{\text{X}}
\newcommand{\NTS}{\text{S}}

\def\FS{\mathit{FS}\xspace}
\def\BS{\mathit{BS}\xspace}
\def\bfR{\mathbf{R}\xspace}

\newcommand{\head}{\ensuremath{\mathit{head}}\xspace}
\newcommand{\tails}{\ensuremath{\mathit{tails}}\xspace}

\newcommand{\Deriv}{\ensuremath{\mathscr{D}}\xspace}
\newcommand{\hhat}{\ensuremath{\hat{h}}\xspace}

\newcommand{\opluseq}{\ensuremath{\ \oplus=}\xspace}

\newcommand{\lianheguo}{\chn{Li\'anh\'egu\'o}\xspace}
\newcommand{\jiandu}{\chn{ji\=and\=u}\xspace}


\newcommand{\chnBushi}{\chn{B\`ush\'i}\xspace}
\newcommand{\chnyu}{\chn{y\v{u}}\xspace}
\newcommand{\chnle}{\chn{le}\xspace}
\newcommand{\chnShalong}{\chn{Sh\=al\'ong}\xspace}
\newcommand{\chnBaoweier}{\chn{B\`aow\=eier}\xspace}
\newcommand{\chnjuxing}{\chn{j\v{u}x\'ing}\xspace}
\newcommand{\chnhuitan}{\chn{hu\`it\'an}\xspace}

\newcommand{\mybullet}{\ensuremath{\bullet\hspace{-0.05mm}}}
\newcommand{\myunderscore}{\ensuremath{\mbox{\Large\_}}}

\newcommand{\nocov}{$_0$\myunderscore\myunderscore\myunderscore\myunderscore\myunderscore\myunderscore}
\newcommand{\onecov}{\mybullet$_1$\myunderscore\myunderscore\myunderscore\myunderscore\myunderscore}
\newcommand{\halfcov}{\mybullet\myunderscore\myunderscore\mybullet\mybullet\mybullet$_{6}$}
\newcommand{\fullcov}{\mybullet\mybullet\mybullet$_{3}$\mybullet\mybullet\mybullet}

%% \newcommand{\nocov}{\ensuremath{_0\myunderscore\myunderscore\myunderscore\myunderscore\myunderscore\myunderscore}\xspace}
%% \newcommand{\onecov}{\ensuremath{\mybullet_1\myunderscore\myunderscore\myunderscore\myunderscore\myunderscore}\xspace}
%% \newcommand{\halfcov}{\ensuremath{\mybullet\myunderscore\myunderscore\mybullet\mybullet\mybullet_6}\xspace}
%% \newcommand{\fullcov}{\ensuremath{\mybullet\mybullet\mybullet_3\mybullet\mybullet\mybullet}\xspace}
\newcommand{\fullncov}{\mybullet\mybullet\ldots\mybullet}


\long\def\signature#1{%
% \begin{flushleft}
\begin{center}
% \begin{minipage}{6in}
\parindent=0pt
\shortstack{\vrule width 3in height 0.4pt\\ #1}
% \end{minipage}
\end{center}
% \end{flushleft}
}

% forest rerank acl 2008
\newcommand{\feat}[1]{{\bf {#1}}}
\newcommand{\Gen}[1]{\ensuremath{\mathit{cand}({#1})}\xspace}
\newcommand{\yhat}{\ensuremath{\hat{y}}\xspace}
\newcommand{\ystar}{\ensuremath{y^*}\xspace}
\newcommand{\yplus}{\ensuremath{y^+}\xspace}
\newcommand{\cost}{\ensuremath{\mathit{c}}\xspace}
\newcommand{\oracle}{\ensuremath{\mathit{oracle}}\xspace}
\newcommand{\ora}{\ensuremath{\mathit{ora}}\xspace}
\newcommand{\cnj}{charniak+johnson:2005}
\newcommand{\coll}{collins:2000}
\newcommand{\dom}{\ensuremath{\mathit{dom}}\xspace}
\newcommand{\gold}{\ensuremath{\mathit{gold}}\xspace}

\newcommand{\myoval}[1]{\ovalnode[linestyle=none,fillstyle=solid,fillcolor=lightgray]{foo}{#1}}
\newcommand{\mybox}[1]{\psframebox[linestyle=none,linewidth=0pt,fillstyle=solid,fillcolor=lightgray]{#1}}

%\newcommand{\vecx}{\ensuremath{\bm{x}}\xspace}
\newcommand{\vecx}{\mathbf{x}\xspace}
%\newcommand{\vecy}{\ensuremath{\bm{y}}\xspace}
\newcommand{\vecy}{\mathbf{y}\xspace}
\newcommand{\vece}{\ensuremath{\bm{e}}\xspace}
\newcommand{\vecw}{\ensuremath{\mathbf{w}}\xspace}
\newcommand{\vecc}{\ensuremath{\mathbf{c}}\xspace}
\newcommand{\vecR}{\ensuremath{\mathbb{R}}\xspace}

\newcommand{\vecv}{\ensuremath{\mathbf{v}}\xspace}
\newcommand{\vecf}{\ensuremath{\mathbf{f}}\xspace}
\newcommand{\vecfl}{\ensuremath{\mathbf{f}_L}\xspace}
%\newcommand{\veczero}{\ensuremath{\mathbf{j}}}

\newcommand{\heap}{\ensuremath{\mathit{heap}}\xspace}

\newcommand{\feature}[1]{$\langle$ {#1} $\rangle$\xspace}

\newcommand{\defineq}{\ensuremath{\; \triangleq\; }\xspace}
\newcommand{\extradgt}{\color{white}{0}\xspace}

\newcommand{\funit}{\ensuremath{\mathring{f}}\xspace}
\newcommand{\vecfunit}{\ensuremath{\mathring{\vecf}}\xspace}
\newcommand{\Done}[1]{\ensuremath{D_1(#1)}}

% kbest paper 2005
\let\algsize\normalsize
\newcommand{\algline}[2]{%
\begin{center}
\algsize$\text{#1:}\hspace{1em}#2$
\end{center}}

\def\Dhat{\hat{D}}
\def\vecDhat{\mathbf{\hat{D}}}

%%%%%%%%%%%%%%% pinyins

\newcommand{\Baoweier}{\chn{B\`aow\=eier}\xspace}
\newcommand{\Bushi}{\chn{B\`ush\'i}\xspace}
\newcommand{\bushi}{\Bushi}
\newcommand{\Shalong}{\chn{Sh\=al\'ong}\xspace}
\newcommand{\yu}{\chn{y\v{u}}\xspace}
\newcommand{\hai}{\chn{h\'ai}\xspace}
\newcommand{\jiang}{\chn{ji\=ang}\xspace}
\newcommand{\huiwu}{\chn{hu\`iw\`u}\xspace}
\newcommand{\jinyibu}{\chn{j\`iny\={\i}b\`u}\xspace}
\newcommand{\juxing}{\chn{j\v{u}x\'ing}\xspace}
\newcommand{\huitan}{\chn{hu\`it\'an}\xspace}
\newcommand{\dangtian}{\chn{d\=angti\=an}\xspace}
\newcommand{\jiu}{\chn{ji\`u}\xspace}
\newcommand{\zhongdong}{\chn{zh\=ongd\=ong}\xspace}
\newcommand{\weiji}{\chn{w\=eij\=\i}\xspace}
\newcommand{\fuze}{\chn{f\`uz\'e}\xspace}

\newcommand{\zongtong}{\chn{z\v{o}ngt\v{o}ng}\xspace}
\newcommand{\zai}{\chn{z\`ai}\xspace}
\newcommand{\mosike}{\chn{M\`os\-{i}k\={e}}\xspace}
\newcommand{\pujing}{\chn{P\v{u}j\={\i}ng}\xspace}
\newcommand{\eluosi}{\chn{\'Elu\'os\=\i}\xspace}
\newcommand{\meiguo}{\chn{M\v{e}igu\'o}\xspace}
%\dangju & \dui & \shate & \jiezhe & \shizong & \yi & \an &\gandao &  \danyou \\
\newcommand{\dangju}{\chn{d\=angj\'u}\xspace}
\newcommand{\dui}{\chn{du\`\i}\xspace}
\newcommand{\shate}{\chn{Sh\=at\`e}\xspace}
\newcommand{\jiezhe}{\chn{j\`{\i}zh\v{e}}\xspace}
\newcommand{\shizong}{\chn{sh\={\i}z\=ong}\xspace}
\newcommand{\danyou}{\chn{d\=any\=ou}\xspace}
\newcommand{\gandao}{\chn{g\v{a}nd\`ao}\xspace}
\newcommand{\an}{\chn{\`an}\xspace}
\newcommand{\yi}{\chn{y\=\i}\xspace}
\newcommand{\buman}{\chn{b\`um\v{a}n}\xspace}

\newcommand{\Prob}{\ensuremath{\mathrm{P}}\xspace}

\newcommand{\lhs}{\ensuremath{\mathit{lhs}}\xspace}
\newcommand{\rhs}{\ensuremath{\mathit{rhs}}\xspace}

\newcommand{\NULL}{\ensuremath{\mathit{null}}\xspace}

\newcommand{\gap}{\ensuremath{\sqcup}\xspace}
\newcommand{\spanof}{\ensuremath{\mathit{span}}\xspace}
\newcommand{\yield}{\ensuremath{\mathit{yield}}\xspace}
\newcommand{\fs}{\ensuremath{\mathit{admset}}\xspace}

\newcommand{\closed}{\ensuremath{\mathit{closed}}\xspace}
\newcommand{\open}{\ensuremath{\mathit{open}}\xspace}
\newcommand{\hs}{\frag} %\ensuremath{\mathit{frag}}\xspace}
\newcommand{\vs}{\ensuremath{\mathit{vs}}\xspace}
\newcommand{\frag}{\ensuremath{\mathit{frag}}\xspace}
\renewcommand{\root}{\ensuremath{\mathit{root}}\xspace}
\newcommand{\leaves}{\yield} %\ensuremath{\mathit{leaves}}\xspace}
\newcommand{\exps}{\ensuremath{\mathit{front}}\xspace} % frontier
\newcommand{\newexps}{\ensuremath{\mathit{\exps'}}\xspace}


\newcommand{\PLM}{\ensuremath{\Prob_{\mathrm{lm}}}\xspace}
\newcommand{\PT}{\ensuremath{\Prob}\xspace}
\newcommand{\PLex}{\ensuremath{\Prob_{\mathrm{lex}}}\xspace}

\newcommand{\GHKM}[3]{\ensuremath{{\mbox{#1}}_{{#2}}^{{#3}}}\xspace}
%\newcommand{\newGHKM}[2]{\ensuremath{{\mbox{#1}}\\{\mbox{\scriptsize #2}}}\xspace}
\newcommand{\tspan}[1]{\scriptsize {#1}\xspace}
\newcommand{\wnode}[1]{\rnode[t]{#1}{#1}\xspace}  %% target words

\newcommand{\vtitem}[2]{\ensuremath{({\vtnt{#1}}_{#2})}\xspace}
%\newcommand{\gap}{\ensuremath{\sqcup}}
%\newcommand{\treeitem}[2]{\ensuremath{({\mbox{#1}}_{#2})}\xspace}

\newcommand{\ruleset}{\ensuremath{\mathcal{R}}\xspace}

% pattern-match
\newcommand{\match}{\ensuremath{\mathit{match}}\xspace}
\newcommand{\vars}{\ensuremath{\mathit{vars}}\xspace}
\newcommand{\mlist}{\ensuremath{\mathit{mlist}}\xspace}
%\newcommand{\Prob}{\ensuremath{\mathrm{P}}\xspace}
\newcommand{\eP}{\ensuremath{e_{\mathit{p}}}\xspace}
%\newcommand{\PLM}{\ensuremath{\Prob_{\mathrm{lm}}}\xspace}
% \newcommand{\PT}{\ensuremath{\Prob}\xspace}
% \newcommand{\PLex}{\ensuremath{\Prob_{\mathrm{lex}}}\xspace}

%NOW MOVED HERE
\newcommand{\npshift}{\hspace{1.6cm}}
\newcommand{\styleb}{linestyle=dashed}

\newcommand{\et}{\ensuremath{e^{\mathrm{t}}}}
\newcommand{\Ht}{\ensuremath{H^{\mathrm{t}}}}
%\newcommand{\ep}{\ensuremath{e^{\mathrm{p}}}}
\newcommand{\ep}{\ensuremath{e}\xspace}  % just for EMNLP
\newcommand{\Hp}{\ensuremath{H^{\mathrm{p}}}}
\newcommand{\Vp}{\ensuremath{V^{\mathrm{p}}}}

%\newcommand\newcite{\citet}
\def\namecite{\newcite}
%\def\namecite{\cite}

\def\Fone{F$_1$\xspace}
\def\Foneperc{F$_1\%$}
\newcommand{\goto}{\ensuremath{\triangleright}\xspace}

\newcommand{\TODO}[1]{\textbf{TODO:} \textit{#1}\xspace}

\newcommand{\smallnt}[1]{\ensuremath{_{\mbox{\tiny PP}}}\xspace}

\newcommand{\shift}{\ensuremath{\mathsf{sh}}\xspace}
\newcommand{\reduce}{\ensuremath{\mathsf{re}}\xspace}
\newcommand{\lreduce}{\ensuremath{\mathsf{re_{\small \curvearrowleft}}}\xspace}
\newcommand{\rreduce}{\ensuremath{\mathsf{re_{\small \curvearrowright}}}\xspace}


\newcommand{\sep}{\ensuremath{ \circ }\xspace}

\newcommand{\sttop}{\ensuremath{s_0}\xspace}
\newcommand{\stnext}{\ensuremath{s_1}\xspace}
\newcommand{\stthird}{\ensuremath{s_2}\xspace}
\newcommand{\qhead}{\ensuremath{q_0}\xspace}
\newcommand{\qnext}{\ensuremath{q_1}\xspace}
\newcommand{\qthird}{\ensuremath{q_2}\xspace}
\newcommand{\Tag}[1]{\ensuremath{{#1}.\mathsf{t}}\xspace}
\newcommand{\Wrd}[1]{\ensuremath{{#1}.\mathsf{w}}\xspace}
\newcommand{\LC}[1]{\ensuremath{{#1}.\mathsf{lc}}\xspace}
\newcommand{\RC}[1]{\ensuremath{{#1}.\mathsf{rc}}\xspace}

% Algorithm 3 -> Pseudocode 3
\newcommand{\pseudocode}{Algorithm}
\floatname{algorithm}{\pseudocode}

\newcommand{\cont}[2]{\ensuremath{\mathit{c}({#1}, {#2})}\xspace}
\newcommand{\contR}[2]{\ensuremath{\mathit{c}_{\mbox{\tiny \sc R}}({#1}, {#2})}\xspace}
\newcommand{\contsttops}{\ensuremath{\cont{\stnext}{\sttop}}\xspace}
\newcommand{\contsttopqhead}{\ensuremath{\contR{\sttop}{\qhead}}\xspace}

\newcommand{\sspan}{\ensuremath{\mathit{sp}}\xspace}
\renewcommand{\tspan}{\ensuremath{\mathit{tp}}\xspace}
\newcommand{\aspan}{\ensuremath{\mathit{ap}}\xspace}

% vanilla non-dp shift-reduce item: (l, S, Q)
\newcommand{\olditem}[3]{\ensuremath{{#1}: \tuple{{#2}, \ {#3}}}\xspace}
\newcommand{\newitem}[4]{\ensuremath{{#1}: \tuple{{#2}, \ {#3}, \ {#4}}}\xspace}

\newcommand{\arcs}{\ensuremath{\mathbf{a}}\xspace}
\newcommand{\arcleft}[2]{\ensuremath{{#1}^\curvearrowleft{#2}}\xspace}
\newcommand{\arcright}[2]{\ensuremath{{#1}^\curvearrowright{#2}}\xspace}

% kernel feature function
\newcommand{\vecfker}{\ensuremath{\widetilde{\mathbf{f}}}\xspace}
\newcommand{\fker}[1]{\ensuremath{\vecfker({#1})}\xspace}
\newcommand{\earleyitem}[3]{\ensuremath{\tuple{{#1}, {#2}, \ {#3}}}\xspace}
\newcommand{\nodpearleyitem}[2]{\ensuremath{\tuple{{#1}, \ {#2}}}\xspace}

\iffalse
\newcommand{\eisneritem}[4]{\newitem{#1}{#2}{#3}{\!\!\!\raisebox{0.04in}{\Tree[.{\ensuremath{#4}} !\Troof{\ensuremath{{#2}...{#3}}} ]}}\xspace}
\newcommand{\specialeisneritem}[4]{\newitem{#1}{#2}{#3}{#4}\xspace}
\else
\newcommand{\eisneritem}[4]{\tuple{{#1}, {\!\!\!\raisebox{0.04in}{\Tree[.{\ensuremath{#4}} !\Troof{\ensuremath{{#2}...{#3}}} ]}}\!\!\!}\xspace}
\newcommand{\specialeisneritem}[4]{\ensuremath{{#1}: \tuple{{#4}}}\xspace}
\newcommand{\gpeisneritem}[5]{\ensuremath{{#1}:\tuple{{#4}, {\!\!\!\raisebox{0.04in}{\Tree[.{\ensuremath{#5}} !\Troof{\ensuremath{{#2}...{#3}}} ]}}\!\!\!}}\xspace}
\fi

\newcommand{\decode}{\ensuremath{\mathit{decode}}\xspace}
\newcommand{\GEN}{\ensuremath{\mathcal{Y}}\xspace}
\newcommand{\GENbar}{\ensuremath{\overline{\GEN}}\xspace}

\newcommand{\spb}[1]{\ensuremath{^{{#1}}}\xspace}
\newcommand{\spbkp}{\ensuremath{\spb{k+1}}\xspace}
\newcommand{\vecwk}{\ensuremath{\vecw\spb{k}}\xspace}
\newcommand{\vecwkp}{\ensuremath{\vecw\spb{k+1}}\xspace}
\newcommand{\vecwt}{\ensuremath{\vecw\spb{t}}\xspace}
\newcommand{\vecwtp}{\ensuremath{\vecw\spb{t+1}}\xspace}
\newcommand{\tth}{\ensuremath{t^{\mathrm{th}}}\xspace}


\newcommand{\err}{\ensuremath{\mathit{err}}\xspace}
\newcommand{\bPhi}{\ensuremath{\mathbf{\Phi}}\xspace}
\newcommand{\dPhi}{\ensuremath{\Delta\bPhi}\xspace}
\newcommand{\labels}{\ensuremath{\mathit{labels}}\xspace}
\newcommand{\onestep}{\ensuremath{\mathit{onestep}}\xspace}
\newcommand{\seqx}{\ensuremath{\overline{x}}\xspace}
\newcommand{\seqy}{\ensuremath{\overline{y}}\xspace}
\newcommand{\seqz}{\ensuremath{\overline{z}}\xspace}

\providecommand{\norm}[1]{\lVert#1\rVert}
\providecommand{\card}[1]{\lvert#1\rvert}  % cardinality |x|
\newcommand{\normtwo}[1]{\norm{#1}^2}

\newcommand{\seqzt}{\ensuremath{\overline{z}^{(t)}}\xspace}
\newcommand{\seqxt}{\ensuremath{\overline{x}^{(t)}}\xspace}
\newcommand{\seqyt}{\ensuremath{\overline{y}^{(t)}}\xspace}

\newcommand{\defeq}{\ensuremath{\stackrel{\Delta}{=}}\xspace}
\newcommand{\InlineIf}[2]{{\bf if} {#1} {\bf then} {#2}}
\newcommand{\dsep}{\ensuremath{\mathcal{D}(\vecu,\delta)}\xspace}
\newcommand{\dgsep}{\ensuremath{\mathcal{D}_g(\vecu,\delta)}\xspace}

\newcommand{\hinge}{\ensuremath{h_{\delta}}\xspace}

\newcommand{\Beam}{\ensuremath{\mathcal{B}}\xspace}

% equivalence class under ~: [[x]]_~
\newcommand{\eqvcls}[1]{\ensuremath{\llbracket {#1} \rrbracket_{\equiv}}\xspace}

\newcommand{\Cs}{\ensuremath{C_{\mathrm{s}}}}
\newcommand{\Cg}{\ensuremath{C_{\mathrm{g}}}}
\newcommand{\Cb}{\ensuremath{C_{\mathrm{b}}}}

%\newcommand{\state}{\ensuremath{\mathit{state}}\xspace}
\newcommand{\action}{\ensuremath{\mathit{action}}\xspace}


\newcommand{\fkerdp}[1]{\ensuremath{\vecfker_{{\mathrm{DP}}}({#1})}\xspace}
\newcommand{\fkernodp}[1]{\ensuremath{\vecfker_{\mathrm{noDP}}({#1})}\xspace}

\newcommand{\score}{\ensuremath{\mathit{S}}\xspace}
\newcommand{\scoring}[2]{\ensuremath{\score_{#1}({#2})}\xspace}
\newcommand{\scoresh}[1]{\ensuremath{\scoring{\shift}{#1}}\xspace}
\newcommand{\scoreleft}[1]{\ensuremath{\scoring{\lreduce}{#1}}\xspace}
\newcommand{\scoreright}[1]{\ensuremath{\scoring{\rreduce}{#1}}\xspace}

\newcommand{\leftptrs}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\rightptrs}{\ensuremath{\mathcal{R}}\xspace}

\newcommand{\chart}{\ensuremath{\mathit{C}}\xspace}
\newcommand{\pq}{\ensuremath{\mathit{Q}}\xspace}

\newcommand{\bleu}{{\sc Bleu}\xspace}
\newcommand{\bleuplusone}{\ensuremath{\mathrm{Bleu}^{+1}}\xspace}
\newcommand{\mert}{{\sc Mert}\xspace}
\newcommand{\ce}{{\sc Ch-En}\xspace}
\newcommand{\se}{{\sc Sp-En}\xspace}
\newcommand{\pro}{{\sc Pro}\xspace}
\newcommand{\mira}{{\sc Mira}\xspace}
\newcommand{\hols}{{\sc Hols}\xspace}
\newcommand{\ramp}{{\sc Ramp}\xspace}
\newcommand{\hiero}{{\sc Hiero}\xspace}
\newcommand{\cdec}{{\tt cdec}\xspace}

\newcommand{\MaxForce}{{\sc MaxForce}\xspace}

\newcommand{\myinfer}[3]{\ensuremath{\infer[\mbox{\footnotesize ${#1}$}]{#2}{#3}}\xspace}
\newcommand{\pre}{\ensuremath{\mathit{pre}}\xspace}
\newcommand{\good}{\ensuremath{\mathit{good}}\xspace}
\newcommand{\bad}{\ensuremath{\mathit{bad}}\xspace}
\newcommand{\ygood}{\ensuremath{\mbox{$y$-good}}\xspace}
\newcommand{\ybad}{\ensuremath{\mbox{$y$-bad}}\xspace}

\newcommand{\cn}{\ensuremath{{\sf cn}}\xspace}
\newcommand{\en}{\ensuremath{{\sf en}}\xspace}

\newcommand{\kNN}{\ensuremath{\mbox{$k$-NN}}\xspace}

\newcommand{\Yahoo}{{\sc Yahoo}\xspace}
\newcommand{\TREC}{{\sc TREC}\xspace}
\newcommand{\DMV}{{\sc DMV}\xspace}
\newcommand{\Insurance}{{\sc Insurance}\xspace}


\def\lr{\mbox{\begin{picture}(7,10)
\put(1,0){\line(1,0){5}}
\put(1,0){\line(1,2){5}}
\put(6,0){\line(0,1){10}}
\end{picture}
}}

% \def\ll{\mbox{\begin{picture}(7,10)
% \put(1,0){\line(1,0){5}}
% \put(6,0){\line(-1,2){5}}
% \put(1,0){\line(0,1){10}}
% \end{picture}
% }}

\def\llbig{\mbox{\begin{picture}(25,10)
\put(1,0){\line(1,0){30}}
\put(31,0){\line(-3,1){30}}
\put(1,0){\line(0,1){10}}
\end{picture}
}}

\def\lrbig{\mbox{\begin{picture}(25,10)
\put(1,0){\line(1,0){30}}
\put(1,0){\line(3,1){30}}
\put(31,0){\line(0,1){10}}
\end{picture}
}}
% \newcommand{\doubleitem}[2]{\ensuremath{\stackrel{\!\!\!\!\!{#1}}{\ll} \stackrel{\ {#2}}{\lr}}\xspace}

\newcommand{\doubleitemleft}[2]{\ensuremath{\stackrel{\hspace{-0.9cm}{#1}}{\llbig} \quad \stackrel{\ {#2}}{\lr}}\xspace}


\newcommand{\doubleitemright}[2]{\ensuremath{\stackrel{\!\!\!\!\!{#1}}{\ll} \; \stackrel{\hspace{1.1cm} {#2}}{\lrbig}}\xspace}

\newcommand{\pytorch}{PyTorch\xspace}
\newcommand{\rnnsearch}{RNNsearch\xspace}

\newcommand{\best}{\ensuremath{\mathit{best}}\xspace}
\newcommand{\bestuptoi}{\ensuremath{\mathit{best}_{\leq i}}\xspace}
\newcommand{\completed}{\ensuremath{\mathit{comp}}\xspace}
\newcommand{\eos}{\mbox{\scriptsize \texttt{<eos>}}\xspace}
\newcommand{\bp}{\ensuremath{\mathit{bp}}\xspace}
\newcommand{\BLEU}{\ensuremath{\mathrm{BLEU}}\xspace}
\newcommand{\PWR}{\ensuremath{\mathrm{PWR}}\xspace}
\newcommand{\AdaR}{\ensuremath{\mathrm{AdaR}}\xspace}
\newcommand{\gnmt}{\ensuremath{\mathrm{GNMT}}\xspace}
\newcommand{\lengthnorm}{\ensuremath{\mathrm{length\_norm}}\xspace}
\newcommand{\word}{\ensuremath{\mathrm{word}}\xspace}
\newcommand{\len}{\ensuremath{\mathit{len}}\xspace}
\newcommand{\gratio}{\ensuremath{\mathit{gr}}\xspace}
\newcommand{\lratio}{\ensuremath{\mathit{lr}}\xspace}
\newcommand{\pred}{\ensuremath{\mathit{pred}}\xspace}

\newcommand{\spinyin}[1]{{\small\em {#1}}}
\newcommand{\bajisitan}{B\=aj\={\i}s\={\i}t\v{a}n}
\newcommand{\yindu}{Y\`{\i}nd\`u}

\newcommand{\deen}{{{de}↔\leftrightarrow{en}}\xspace}
\newcommand{\zhen}{{{zh}↔\leftrightarrow{en}}\xspace}
\newcommand{\detoen}{{{de}\goesto\goesto{en}}\xspace}
\newcommand{\entode}{{{en}\goesto\goesto{de}}\xspace}
\newcommand{\zhtoen}{{{zh}\goesto\goesto{en}}\xspace}
\newcommand{\entozh}{{{en}\goesto\goesto{zh}}\xspace}

\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\gwaitk}{\ensuremath{{g_\text{wait-kk}}}\xspace}
\newcommand{\gcatchup}{\ensuremath{{g_\text{wait-kk, cc}}}\xspace}

\newcommand{\CW}{\ensuremath{\mathrm{CW}}\xspace}
\newcommand{\AP}{\ensuremath{\mathrm{AP}}\xspace}
\newcommand{\AL}{\ensuremath{\mathrm{AL}}\xspace}
\newcommand{\RAL}{\ensuremath{\mathrm{RAL}}\xspace}

\newcommand{\dsxy}{D_{\vecs,\vecx,\vecy}\xspace}
\newcommand{\dsy}{D_{\vecs,\vecy}\xspace}
\newcommand{\dsx}{D_{\vecs,\vecx}\xspace}
\newcommand{\dxy}{D_{\vecx,\vecy}\xspace}
\newcommand{\duy}{D_{\vecu,\vecy}\xspace}

\newcommand{\ds}{D_{\vecs}\xspace}
\newcommand{\dx}{D_{\vecx}\xspace}
\newcommand{\dy}{D_{\vecy}\xspace}

==> [ACL2023]DUB_ discrete unit back-translation for ST/rebib_custom.tex <==
@inproceedings{lee2022textless,
 address = {Seattle, United States},
 author = {Lee, Ann  and
Gong, Hongyu  and
Duquenne, Paul-Ambroise  and
Schwenk, Holger  and
Chen, Peng-Jen  and
Wang, Changhan  and
Popuri, Sravya  and
Adi, Yossi  and
Pino, Juan  and
Gu, Jiatao  and
Hsu, Wei-Ning},
 booktitle = {Proceedings of the 2022 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies},
 doi = {10.18653/v1/2022.naacl-main.63},
 pages = {860--872},
 publisher = {Association for Computational Linguistics},
 title = {Textless Speech-to-Speech Translation on Real Data},
 url = {https://aclanthology.org/2022.naacl-main.63},
 year = {2022}
}

@article{lakhotia2021generative,
 address = {Cambridge, MA},
 author = {Lakhotia, Kushal  and
Kharitonov, Eugene  and
Hsu, Wei-Ning  and
Adi, Yossi  and
Polyak, Adam  and
Bolte, Benjamin  and
Nguyen, Tu-Anh  and
Copet, Jade  and
Baevski, Alexei  and
Mohamed, Abdelrahman  and
Dupoux, Emmanuel},
 doi = {10.1162/tacl_a_00430},
 journal = {Transactions of the Association for Computational Linguistics},
 pages = {1336--1354},
 publisher = {MIT Press},
 title = {On Generative Spoken Language Modeling from Raw Audio},
 url = {https://aclanthology.org/2021.tacl-1.79},
 volume = {9},
 year = {2021}
}

@article{inaguma2022unity,
 author = {Inaguma, Hirofumi and Popuri, Sravya and Kulikov, Ilia and Chen, Peng-Jen and Wang, Changhan and Chung, Yu-An and Tang, Yun and Lee, Ann and Watanabe, Shinji and Pino, Juan},
 journal = {ArXiv preprint},
 title = {UnitY: Two-pass Direct Speech-to-speech Translation with Discrete Units},
 url = {https://arxiv.org/abs/2212.08055},
 volume = {abs/2212.08055},
 year = {2022}
}

@article{popuri2022enhanced,
 author = {Popuri, Sravya and Chen, Peng-Jen and Wang, Changhan and Pino, Juan and Adi, Yossi and Gu, Jiatao and Hsu, Wei-Ning and Lee, Ann},
 journal = {ArXiv preprint},
 title = {Enhanced Direct Speech-to-Speech Translation Using Self-supervised Pre-training and Data Augmentation},
 url = {https://arxiv.org/abs/2204.02967},
 volume = {abs/2204.02967},
 year = {2022}
}

@article{huang2022transpeech,
 author = {Huang, Rongjie and Zhao, Zhou and Liu, Jinglin and Liu, Huadai and Ren, Yi and Zhang, Lichao and He, Jinzheng},
 journal = {ArXiv preprint},
 title = {TranSpeech: Speech-to-Speech Translation With Bilateral Perturbation},
 url = {https://arxiv.org/abs/2205.12523},
 volume = {abs/2205.12523},
 year = {2022}
}

@inproceedings{kharitonov2022text,
 address = {Dublin, Ireland},
 author = {Kharitonov, Eugene  and
Lee, Ann  and
Polyak, Adam  and
Adi, Yossi  and
Copet, Jade  and
Lakhotia, Kushal  and
Nguyen, Tu Anh  and
Riviere, Morgane  and
Mohamed, Abdelrahman  and
Dupoux, Emmanuel  and
Hsu, Wei-Ning},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2022.acl-long.593},
 pages = {8666--8681},
 publisher = {Association for Computational Linguistics},
 title = {Text-Free Prosody-Aware Generative Spoken Language Modeling},
 url = {https://aclanthology.org/2022.acl-long.593},
 year = {2022}
}

@article{chen2022wavlm,
 author = {Chen, Sanyuan and Wang, Chengyi and Chen, Zhengyang and Wu, Yu and Liu, Shujie and Chen, Zhuo and Li, Jinyu and Kanda, Naoyuki and Yoshioka, Takuya and Xiao, Xiong and others},
 journal = {IEEE Journal of Selected Topics in Signal Processing},
 number = {6},
 pages = {1505--1518},
 publisher = {IEEE},
 title = {Wavlm: Large-scale self-supervised pre-training for full stack speech processing},
 volume = {16},
 year = {2022}
}

@inproceedings{chung2021w2v,
 author = {Chung, Yu-An and Zhang, Yu and Han, Wei and Chiu, Chung-Cheng and Qin, James and Pang, Ruoming and Wu, Yonghui},
 booktitle = {2021 IEEE Automatic Speech Recognition and Understanding Workshop (ASRU)},
 organization = {IEEE},
 pages = {244--250},
 title = {W2v-bert: Combining contrastive learning and masked language modeling for self-supervised speech pre-training},
 year = {2021}
}

@article{zhang2022speechlm,
 author = {Zhang, Ziqiang and Chen, Sanyuan and Zhou, Long and Wu, Yu and Ren, Shuo and Liu, Shujie and Yao, Zhuoyuan and Gong, Xun and Dai, Lirong and Li, Jinyu and others},
 journal = {ArXiv preprint},
 title = {Speechlm: Enhanced speech pre-training with unpaired textual data},
 url = {https://arxiv.org/abs/2209.15329},
 volume = {abs/2209.15329},
 year = {2022}
}

@inproceedings{berard2016listen,
 author = {B{\'e}rard, Alexandre and Pietquin, Olivier and Besacier, Laurent and Servan, Christophe},
 booktitle = {NIPS Workshop on end-to-end learning for speech and audio processing},
 title = {Listen and Translate: A Proof of Concept for End-to-End Speech-to-Text Translation},
 year = {2016}
}

@inproceedings{di2019adapting,
 author = {Mattia Antonino Di Gangi and
Matteo Negri and
Marco Turchi},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/interspeech/GangiNT19.bib},
 booktitle = {Proc. of INTERSPEECH},
 doi = {10.21437/Interspeech.2019-3045},
 editor = {Gernot Kubin and
Zdravko Kacic},
 pages = {1133--1137},
 publisher = {{ISCA}},
 timestamp = {Fri, 29 Jan 2021 00:00:00 +0100},
 title = {Adapting Transformer to End-to-End Spoken Language Translation},
 url = {https://doi.org/10.21437/Interspeech.2019-3045},
 year = {2019}
}

@inproceedings{gaido2021ctc,
 address = {Online},
 author = {Gaido, Marco  and
Cettolo, Mauro  and
Negri, Matteo  and
Turchi, Marco},
 booktitle = {Proceedings of the 16th Conference of the European Chapter of the Association for Computational Linguistics: Main Volume},
 doi = {10.18653/v1/2021.eacl-main.57},
 pages = {690--696},
 publisher = {Association for Computational Linguistics},
 title = {{CTC}-based Compression for Direct Speech Translation},
 url = {https://aclanthology.org/2021.eacl-main.57},
 year = {2021}
}

@inproceedings{dong2021listen,
 author = {Dong, Qianqian and Ye, Rong and Wang, Mingxuan and Zhou, Hao and Xu, Shuang and Xu, Bo and Li, Lei},
 booktitle = {Proc. of AAAI},
 pages = {12749--12759},
 title = {Listen, understand and translate: Triple supervision decouples end-to-end speech-to-text translation},
 year = {2021}
}

@inproceedings{dong2021consecutive,
 author = {Dong, Qianqian and Wang, Mingxuan and Zhou, Hao and Xu, Shuang and Xu, Bo and Li, Lei},
 booktitle = {Proc. of AAAI},
 pages = {12738--12748},
 title = {Consecutive decoding for speech-to-text translation},
 year = {2021}
}

@inproceedings{xu2021stacked,
 address = {Online},
 author = {Xu, Chen  and
Hu, Bojie  and
Li, Yanyang  and
Zhang, Yuhao  and
Huang, Shen  and
Ju, Qi  and
Xiao, Tong  and
Zhu, Jingbo},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2021.acl-long.204},
 pages = {2619--2630},
 publisher = {Association for Computational Linguistics},
 title = {Stacked Acoustic-and-Textual Encoding: Integrating the Pre-trained Models into Speech Translation Encoders},
 url = {https://aclanthology.org/2021.acl-long.204},
 year = {2021}
}

@inproceedings{zhang2020adaptive,
 address = {Online},
 author = {Zhang, Biao  and
Titov, Ivan  and
Haddow, Barry  and
Sennrich, Rico},
 booktitle = {Findings of the Association for Computational Linguistics: EMNLP 2020},
 doi = {10.18653/v1/2020.findings-emnlp.230},
 pages = {2533--2544},
 publisher = {Association for Computational Linguistics},
 title = {Adaptive Feature Selection for End-to-End Speech Translation},
 url = {https://aclanthology.org/2020.findings-emnlp.230},
 year = {2020}
}

@inproceedings{wang2021voxpopuli,
 address = {Online},
 author = {Wang, Changhan  and
Riviere, Morgane  and
Lee, Ann  and
Wu, Anne  and
Talnikar, Chaitanya  and
Haziza, Daniel  and
Williamson, Mary  and
Pino, Juan  and
Dupoux, Emmanuel},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2021.acl-long.80},
 pages = {993--1003},
 publisher = {Association for Computational Linguistics},
 title = {{V}ox{P}opuli: A Large-Scale Multilingual Speech Corpus for Representation Learning, Semi-Supervised Learning and Interpretation},
 url = {https://aclanthology.org/2021.acl-long.80},
 year = {2021}
}

@inproceedings{di2019must,
 address = {Minneapolis, Minnesota},
 author = {Di Gangi, Mattia A.  and
Cattoni, Roldano  and
Bentivogli, Luisa  and
Negri, Matteo  and
Turchi, Marco},
 booktitle = {Proc. of NAACL-HLT},
 doi = {10.18653/v1/N19-1202},
 pages = {2012--2017},
 publisher = {Association for Computational Linguistics},
 title = {{M}u{ST}-{C}: a {M}ultilingual {S}peech {T}ranslation {C}orpus},
 url = {https://aclanthology.org/N19-1202},
 year = {2019}
}

@inproceedings{wang2021covost,
 author = {Changhan Wang and
Anne Wu and
Jiatao Gu and
Juan Pino},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/interspeech/WangWGP21.bib},
 booktitle = {Proc. of INTERSPEECH},
 doi = {10.21437/Interspeech.2021-2027},
 editor = {Hynek Hermansky and
Honza Cernock{\'{y}} and
Luk{\'{a}}s Burget and
Lori Lamel and
Odette Scharenborg and
Petr Motl{\'{\i}}cek},
 pages = {2247--2251},
 publisher = {{ISCA}},
 timestamp = {Mon, 14 Mar 2022 00:00:00 +0100},
 title = {CoVoST 2 and Massively Multilingual Speech Translation},
 url = {https://doi.org/10.21437/Interspeech.2021-2027},
 year = {2021}
}

@inproceedings{zhao2021neurst,
 address = {Online},
 author = {Zhao, Chengqi  and
Wang, Mingxuan  and
Dong, Qianqian  and
Ye, Rong  and
Li, Lei},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2021.acl-demo.7},
 pages = {55--62},
 publisher = {Association for Computational Linguistics},
 title = {{N}eur{ST}: Neural Speech Translation Toolkit},
 url = {https://aclanthology.org/2021.acl-demo.7},
 year = {2021}
}

@inproceedings{du2022regularizing,
 author = {Du, Yichao and Zhang, Zhirui and Wang, Weizhi and Chen, Boxing and Xie, Jun and Xu, Tong},
 booktitle = {Proc. of AAAI},
 pages = {10590--10598},
 title = {Regularizing end-to-end speech translation with triangular decomposition agreement},
 year = {2022}
}

@inproceedings{pino2020selfa,
 author = {Juan Miguel Pino and
Qiantong Xu and
Xutai Ma and
Mohammad Javad Dousti and
Yun Tang},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/interspeech/PinoXMDT20.bib},
 booktitle = {Proc. of INTERSPEECH},
 doi = {10.21437/Interspeech.2020-2938},
 editor = {Helen Meng and
Bo Xu and
Thomas Fang Zheng},
 pages = {1476--1480},
 publisher = {{ISCA}},
 timestamp = {Thu, 12 Aug 2021 01:00:00 +0200},
 title = {Self-Training for End-to-End Speech Translation},
 url = {https://doi.org/10.21437/Interspeech.2020-2938},
 year = {2020}
}

@inproceedings{inaguma2020espnet,
 address = {Online},
 author = {Inaguma, Hirofumi  and
Kiyono, Shun  and
Duh, Kevin  and
Karita, Shigeki  and
Yalta, Nelson  and
Hayashi, Tomoki  and
Watanabe, Shinji},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2020.acl-demos.34},
 pages = {302--311},
 publisher = {Association for Computational Linguistics},
 title = {{ESP}net-{ST}: All-in-One Speech Translation Toolkit},
 url = {https://aclanthology.org/2020.acl-demos.34},
 year = {2020}
}

@inproceedings{papi2021speechformer,
 address = {Online and Punta Cana, Dominican Republic},
 author = {Papi, Sara  and
Gaido, Marco  and
Negri, Matteo  and
Turchi, Marco},
 booktitle = {Proc. of EMNLP},
 doi = {10.18653/v1/2021.emnlp-main.127},
 pages = {1698--1706},
 publisher = {Association for Computational Linguistics},
 title = {Speechformer: Reducing Information Loss in Direct Speech Translation},
 url = {https://aclanthology.org/2021.emnlp-main.127},
 year = {2021}
}

@inproceedings{ye2021end,
 author = {Rong Ye and
Mingxuan Wang and
Lei Li},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/interspeech/YeW021.bib},
 booktitle = {Proc. of INTERSPEECH},
 doi = {10.21437/Interspeech.2021-1065},
 editor = {Hynek Hermansky and
Honza Cernock{\'{y}} and
Luk{\'{a}}s Burget and
Lori Lamel and
Odette Scharenborg and
Petr Motl{\'{\i}}cek},
 pages = {2267--2271},
 publisher = {{ISCA}},
 timestamp = {Mon, 14 Mar 2022 00:00:00 +0100},
 title = {End-to-End Speech Translation via Cross-Modal Progressive Training},
 url = {https://doi.org/10.21437/Interspeech.2021-1065},
 year = {2021}
}

@inproceedings{ye2022cross,
 address = {Seattle, United States},
 author = {Ye, Rong  and
Wang, Mingxuan  and
Li, Lei},
 booktitle = {Proceedings of the 2022 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies},
 doi = {10.18653/v1/2022.naacl-main.376},
 pages = {5099--5113},
 publisher = {Association for Computational Linguistics},
 title = {Cross-modal Contrastive Learning for Speech Translation},
 url = {https://aclanthology.org/2022.naacl-main.376},
 year = {2022}
}

@inproceedings{tang2021improving,
 address = {Online},
 author = {Tang, Yun  and
Pino, Juan  and
Li, Xian  and
Wang, Changhan  and
Genzel, Dmitriy},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2021.acl-long.328},
 pages = {4252--4261},
 publisher = {Association for Computational Linguistics},
 title = {Improving Speech Translation by Understanding and Learning from the Auxiliary Text Translation Task},
 url = {https://aclanthology.org/2021.acl-long.328},
 year = {2021}
}

@inproceedings{zhang2022revisiting,
 author = {Zhang, Biao and Haddow, Barry and Sennrich, Rico},
 booktitle = {Proc. of ICML},
 title = {Revisiting End-to-End Speech-to-Text Translation From Scratch},
 year = {2022}
}

@inproceedings{tang2022unified,
 address = {Dublin, Ireland},
 author = {Tang, Yun  and
Gong, Hongyu  and
Dong, Ning  and
Wang, Changhan  and
Hsu, Wei-Ning  and
Gu, Jiatao  and
Baevski, Alexei  and
Li, Xian  and
Mohamed, Abdelrahman  and
Auli, Michael  and
Pino, Juan},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2022.acl-long.105},
 pages = {1488--1499},
 publisher = {Association for Computational Linguistics},
 title = {Unified Speech-Text Pre-training for Speech Translation and Recognition},
 url = {https://aclanthology.org/2022.acl-long.105},
 year = {2022}
}

@inproceedings{fang2022stemm,
 address = {Dublin, Ireland},
 author = {Fang, Qingkai  and
Ye, Rong  and
Li, Lei  and
Feng, Yang  and
Wang, Mingxuan},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2022.acl-long.486},
 pages = {7050--7062},
 publisher = {Association for Computational Linguistics},
 title = {{STEMM}: Self-learning with Speech-text Manifold Mixup for Speech Translation},
 url = {https://aclanthology.org/2022.acl-long.486},
 year = {2022}
}

@inproceedings{zheng2021fused,
 author = {Renjie Zheng and
Junkun Chen and
Mingbo Ma and
Liang Huang},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/ZhengCM021.bib},
 booktitle = {Proc. of ICML},
 editor = {Marina Meila and
Tong Zhang},
 pages = {12736--12746},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Wed, 25 Aug 2021 01:00:00 +0200},
 title = {Fused Acoustic and Text Encoding for Multimodal Bilingual Pretraining
and Speech Translation},
 url = {http://proceedings.mlr.press/v139/zheng21a.html},
 volume = {139},
 year = {2021}
}

@article{karakanta2018neural,
 author = {Karakanta, Alina and Dehdari, Jon and van Genabith, Josef},
 journal = {Machine Translation},
 number = {1},
 pages = {167--189},
 publisher = {Springer},
 title = {Neural machine translation for low-resource languages without parallel corpora},
 volume = {32},
 year = {2018}
}

@inproceedings{anastasopoulos2018tied,
 address = {New Orleans, Louisiana},
 author = {Anastasopoulos, Antonios  and
Chiang, David},
 booktitle = {Proc. of NAACL-HLT},
 doi = {10.18653/v1/N18-1008},
 pages = {82--91},
 publisher = {Association for Computational Linguistics},
 title = {Tied Multitask Learning for Neural Speech Translation},
 url = {https://aclanthology.org/N18-1008},
 year = {2018}
}

@inproceedings{indurthi2021task,
 author = {Indurthi, Sathish and Zaidi, Mohd Abbas and Lakumarapu, Nikhil Kumar and Lee, Beomseok and Han, Hyojung and Ahn, Seokchan and Kim, Sangha and Kim, Chanwoo and Hwang, Inchul},
 booktitle = {Proc. of ICASSP},
 organization = {IEEE},
 pages = {7723--7727},
 title = {Task aware multi-task learning for speech to text tasks},
 year = {2021}
}

@inproceedings{schneider2019wav2vec,
 author = {Steffen Schneider and
Alexei Baevski and
Ronan Collobert and
Michael Auli},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/interspeech/SchneiderBCA19.bib},
 booktitle = {Proc. of INTERSPEECH},
 doi = {10.21437/Interspeech.2019-1873},
 editor = {Gernot Kubin and
Zdravko Kacic},
 pages = {3465--3469},
 publisher = {{ISCA}},
 timestamp = {Fri, 29 Jan 2021 00:00:00 +0100},
 title = {wav2vec: Unsupervised Pre-Training for Speech Recognition},
 url = {https://doi.org/10.21437/Interspeech.2019-1873},
 year = {2019}
}

@inproceedings{dong2018speech,
 author = {Linhao Dong and
Shuang Xu and
Bo Xu},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icassp/DongXX18.bib},
 booktitle = {2018 {IEEE} International Conference on Acoustics, Speech and Signal
Processing, {ICASSP} 2018, Calgary, AB, Canada, April 15-20, 2018},
 doi = {10.1109/ICASSP.2018.8462506},
 pages = {5884--5888},
 publisher = {{IEEE}},
 timestamp = {Tue, 25 Jun 2019 01:00:00 +0200},
 title = {Speech-Transformer: {A} No-Recurrence Sequence-to-Sequence Model for
Speech Recognition},
 url = {https://doi.org/10.1109/ICASSP.2018.8462506},
 year = {2018}
}

@inproceedings{baevski2020wav2vec,
 author = {Alexei Baevski and
Yuhao Zhou and
Abdelrahman Mohamed and
Michael Auli},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/BaevskiZMA20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {wav2vec 2.0: {A} Framework for Self-Supervised Learning of Speech
Representations},
 url = {https://proceedings.neurips.cc/paper/2020/hash/92d1e1eb1cd6f9fba3227870bb6d7f07-Abstract.html},
 year = {2020}
}

@inproceedings{van2017neural,
 author = {A{\"{a}}ron van den Oord and
Oriol Vinyals and
Koray Kavukcuoglu},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/OordVK17.bib},
 booktitle = {Advances in Neural Information Processing Systems 30: Annual Conference
on Neural Information Processing Systems 2017, December 4-9, 2017,
Long Beach, CA, {USA}},
 editor = {Isabelle Guyon and
Ulrike von Luxburg and
Samy Bengio and
Hanna M. Wallach and
Rob Fergus and
S. V. N. Vishwanathan and
Roman Garnett},
 pages = {6306--6315},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Neural Discrete Representation Learning},
 url = {https://proceedings.neurips.cc/paper/2017/hash/7a98af17e63a0ac09ce2e96d03992fbc-Abstract.html},
 year = {2017}
}

@inproceedings{dunbar2019zero,
 author = {Ewan Dunbar and
Robin Algayres and
Julien Karadayi and
Mathieu Bernard and
Juan Benjumea and
Xuan{-}Nga Cao and
Lucie Miskic and
Charlotte Dugrain and
Lucas Ondel and
Alan W. Black and
Laurent Besacier and
Sakriani Sakti and
Emmanuel Dupoux},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/interspeech/DunbarAKBBCMDOB19.bib},
 booktitle = {Proc. of INTERSPEECH},
 doi = {10.21437/Interspeech.2019-2904},
 editor = {Gernot Kubin and
Zdravko Kacic},
 pages = {1088--1092},
 publisher = {{ISCA}},
 timestamp = {Fri, 29 Jan 2021 00:00:00 +0100},
 title = {The Zero Resource Speech Challenge 2019: {TTS} Without {T}},
 url = {https://doi.org/10.21437/Interspeech.2019-2904},
 year = {2019}
}

@inproceedings{zhang2021uwspeech,
 author = {Zhang, Chen and Tan, Xu and Ren, Yi and Qin, Tao and Zhang, Kejun and Liu, Tie-Yan},
 booktitle = {Proc. of the AAAI},
 pages = {14319--14327},
 title = {Uwspeech: Speech to speech translation for unwritten languages},
 year = {2021}
}

@inproceedings{baevski2019vq,
 author = {Alexei Baevski and
Steffen Schneider and
Michael Auli},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/BaevskiSA20.bib},
 booktitle = {Proc. of ICLR},
 publisher = {OpenReview.net},
 timestamp = {Thu, 07 May 2020 01:00:00 +0200},
 title = {vq-wav2vec: Self-Supervised Learning of Discrete Speech Representations},
 url = {https://openreview.net/forum?id=rylwJxrYDS},
 year = {2020}
}

@article{meng2022cobert,
 author = {Meng, Chutong and Ao, Junyi and Ko, Tom and Wang, Mingxuan and Li, Haizhou},
 journal = {ArXiv preprint},
 title = {CoBERT: Self-Supervised Speech Representation Learning Through Code Representation Learning},
 url = {https://arxiv.org/abs/2210.04062},
 volume = {abs/2210.04062},
 year = {2022}
}

@article{lu2022unsupervised,
 author = {Lu, Zhiyun and Wang, Yongqiang and Zhang, Yu and Han, Wei and Chen, Zhehuai and Haghani, Parisa},
 journal = {ArXiv preprint},
 title = {Unsupervised Data Selection via Discrete Speech Representation for ASR},
 url = {https://arxiv.org/abs/2204.01981},
 volume = {abs/2204.01981},
 year = {2022}
}

@inproceedings{liu2019end,
 author = {Yuchen Liu and
Hao Xiong and
Jiajun Zhang and
Zhongjun He and
Hua Wu and
Haifeng Wang and
Chengqing Zong},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/interspeech/LiuXZHWWZ19.bib},
 booktitle = {Proc. of INTERSPEECH},
 doi = {10.21437/Interspeech.2019-2582},
 editor = {Gernot Kubin and
Zdravko Kacic},
 pages = {1128--1132},
 publisher = {{ISCA}},
 timestamp = {Tue, 27 Jul 2021 01:00:00 +0200},
 title = {End-to-End Speech Translation with Knowledge Distillation},
 url = {https://doi.org/10.21437/Interspeech.2019-2582},
 year = {2019}
}

@inproceedings{ye2020variational,
 author = {Rong Ye and
Wenxian Shi and
Hao Zhou and
Zhongyu Wei and
Lei Li},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/YeS0W020.bib},
 booktitle = {Proc. of ICLR},
 publisher = {OpenReview.net},
 timestamp = {Wed, 09 Sep 2020 01:00:00 +0200},
 title = {Variational Template Machine for Data-to-Text Generation},
 url = {https://openreview.net/forum?id=HkejNgBtPB},
 year = {2020}
}

@article{hsu2021hubert,
 author = {Hsu, Wei-Ning and Bolte, Benjamin and Tsai, Yao-Hung Hubert and Lakhotia, Kushal and Salakhutdinov, Ruslan and Mohamed, Abdelrahman},
 journal = {IEEE/ACM Transactions on Audio, Speech, and Language Processing},
 pages = {3451--3460},
 publisher = {IEEE},
 title = {Hubert: Self-supervised speech representation learning by masked prediction of hidden units},
 volume = {29},
 year = {2021}
}

@inproceedings{vaswani2017attention,
 author = {Ashish Vaswani and
Noam Shazeer and
Niki Parmar and
Jakob Uszkoreit and
Llion Jones and
Aidan N. Gomez and
Lukasz Kaiser and
Illia Polosukhin},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/VaswaniSPUJGKP17.bib},
 booktitle = {Advances in Neural Information Processing Systems 30: Annual Conference
on Neural Information Processing Systems 2017, December 4-9, 2017,
Long Beach, CA, {USA}},
 editor = {Isabelle Guyon and
Ulrike von Luxburg and
Samy Bengio and
Hanna M. Wallach and
Rob Fergus and
S. V. N. Vishwanathan and
Roman Garnett},
 pages = {5998--6008},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Attention is All you Need},
 url = {https://proceedings.neurips.cc/paper/2017/hash/3f5ee243547dee91fbd053c1c4a845aa-Abstract.html},
 year = {2017}
}

@article{liu2020multilingual,
 address = {Cambridge, MA},
 author = {Liu, Yinhan  and
Gu, Jiatao  and
Goyal, Naman  and
Li, Xian  and
Edunov, Sergey  and
Ghazvininejad, Marjan  and
Lewis, Mike  and
Zettlemoyer, Luke},
 doi = {10.1162/tacl_a_00343},
 journal = {Transactions of the Association for Computational Linguistics},
 pages = {726--742},
 publisher = {MIT Press},
 title = {Multilingual Denoising Pre-training for Neural Machine Translation},
 url = {https://aclanthology.org/2020.tacl-1.47},
 volume = {8},
 year = {2020}
}

@inproceedings{wang-etal-2020-fairseq,
 address = {Suzhou, China},
 author = {Wang, Changhan  and
Tang, Yun  and
Ma, Xutai  and
Wu, Anne  and
Okhonko, Dmytro  and
Pino, Juan},
 booktitle = {Proceedings of the 1st Conference of the Asia-Pacific Chapter of the Association for Computational Linguistics and the 10th International Joint Conference on Natural Language Processing: System Demonstrations},
 pages = {33--39},
 publisher = {Association for Computational Linguistics},
 title = {Fairseq {S}2{T}: Fast Speech-to-Text Modeling with Fairseq},
 url = {https://aclanthology.org/2020.aacl-demo.6},
 year = {2020}
}

@inproceedings{edunov-etal-2018-understanding,
 address = {Brussels, Belgium},
 author = {Edunov, Sergey  and
Ott, Myle  and
Auli, Michael  and
Grangier, David},
 booktitle = {Proc. of EMNLP},
 doi = {10.18653/v1/D18-1045},
 pages = {489--500},
 publisher = {Association for Computational Linguistics},
 title = {Understanding Back-Translation at Scale},
 url = {https://aclanthology.org/D18-1045},
 year = {2018}
}

@inproceedings{ao2022speecht5,
 address = {Dublin, Ireland},
 author = {Ao, Junyi  and
Wang, Rui  and
Zhou, Long  and
Wang, Chengyi  and
Ren, Shuo  and
Wu, Yu  and
Liu, Shujie  and
Ko, Tom  and
Li, Qing  and
Zhang, Yu  and
Wei, Zhihua  and
Qian, Yao  and
Li, Jinyu  and
Wei, Furu},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2022.acl-long.393},
 pages = {5723--5738},
 publisher = {Association for Computational Linguistics},
 title = {{S}peech{T}5: Unified-Modal Encoder-Decoder Pre-Training for Spoken Language Processing},
 url = {https://aclanthology.org/2022.acl-long.393},
 year = {2022}
}

@inproceedings{caswell2019tagged,
 address = {Florence, Italy},
 author = {Caswell, Isaac  and
Chelba, Ciprian  and
Grangier, David},
 booktitle = {Proceedings of the Fourth Conference on Machine Translation (Volume 1: Research Papers)},
 doi = {10.18653/v1/W19-5206},
 pages = {53--63},
 publisher = {Association for Computational Linguistics},
 title = {Tagged Back-Translation},
 url = {https://aclanthology.org/W19-5206},
 year = {2019}
}

@inproceedings{kudo-richardson-2018-sentencepiece,
 address = {Brussels, Belgium},
 author = {Kudo, Taku  and
Richardson, John},
 booktitle = {Proc. of EMNLP},
 doi = {10.18653/v1/D18-2012},
 pages = {66--71},
 publisher = {Association for Computational Linguistics},
 title = {{S}entence{P}iece: A simple and language independent subword tokenizer and detokenizer for Neural Text Processing},
 url = {https://aclanthology.org/D18-2012},
 year = {2018}
}

@inproceedings{panayotov2015librispeech,
 author = {Vassil Panayotov and
Guoguo Chen and
Daniel Povey and
Sanjeev Khudanpur},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icassp/PanayotovCPK15.bib},
 booktitle = {2015 {IEEE} International Conference on Acoustics, Speech and Signal
Processing, {ICASSP} 2015, South Brisbane, Queensland, Australia,
April 19-24, 2015},
 doi = {10.1109/ICASSP.2015.7178964},
 pages = {5206--5210},
 publisher = {{IEEE}},
 timestamp = {Fri, 25 Dec 2020 00:00:00 +0100},
 title = {Librispeech: An {ASR} corpus based on public domain audio books},
 url = {https://doi.org/10.1109/ICASSP.2015.7178964},
 year = {2015}
}

@inproceedings{lee-etal-2022-textless,
 address = {Seattle, United States},
 author = {Lee, Ann  and
Gong, Hongyu  and
Duquenne, Paul-Ambroise  and
Schwenk, Holger  and
Chen, Peng-Jen  and
Wang, Changhan  and
Popuri, Sravya  and
Adi, Yossi  and
Pino, Juan  and
Gu, Jiatao  and
Hsu, Wei-Ning},
 booktitle = {Proceedings of the 2022 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies},
 doi = {10.18653/v1/2022.naacl-main.63},
 pages = {860--872},
 publisher = {Association for Computational Linguistics},
 title = {Textless Speech-to-Speech Translation on Real Data},
 url = {https://aclanthology.org/2022.naacl-main.63},
 year = {2022}
}

@inproceedings{zhang2022speechut,
 author = {Zhang, Ziqiang and Zhou, Long and Ao, Junyi and Liu, Shujie and Dai, Lirong and Li, Jinyu and Wei, Furu},
 booktitle = {Proc. of EMNLP},
 title = {Speechut: Bridging speech and text with hidden-unit for encoder-decoder based speech-text pre-training},
 year = {2022}
}

@inproceedings{post2018call,
 address = {Brussels, Belgium},
 author = {Post, Matt},
 booktitle = {Proceedings of the Third Conference on Machine Translation: Research Papers},
 doi = {10.18653/v1/W18-6319},
 pages = {186--191},
 publisher = {Association for Computational Linguistics},
 title = {A Call for Clarity in Reporting {BLEU} Scores},
 url = {https://aclanthology.org/W18-6319},
 year = {2018}
}

@misc{duh18multitarget,
 author = {Kevin Duh},
 howpublished = {\url{http://www.cs.jhu.edu/~kevinduh/a/multitarget-tedtalks/}},
 title = {The Multitarget TED Talks Task},
 year = {2018}
}

@inproceedings{sung2019towards,
 author = {Tzu{-}Wei Sung and
Jun{-}You Liu and
Hung{-}yi Lee and
Lin{-}Shan Lee},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icassp/SungLLL19.bib},
 booktitle = {{IEEE} International Conference on Acoustics, Speech and Signal Processing,
{ICASSP} 2019, Brighton, United Kingdom, May 12-17, 2019},
 doi = {10.1109/ICASSP.2019.8682801},
 pages = {7175--7179},
 publisher = {{IEEE}},
 timestamp = {Sun, 30 Jun 2019 01:00:00 +0200},
 title = {Towards End-to-end Speech-to-text Translation with Two-pass Decoding},
 url = {https://doi.org/10.1109/ICASSP.2019.8682801},
 year = {2019}
}

@inproceedings{salesky-etal-2019-exploring,
 address = {Florence, Italy},
 author = {Salesky, Elizabeth  and
Sperber, Matthias  and
Black, Alan W},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/P19-1179},
 pages = {1835--1841},
 publisher = {Association for Computational Linguistics},
 title = {Exploring Phoneme-Level Speech Representations for End-to-End Speech Translation},
 url = {https://aclanthology.org/P19-1179},
 year = {2019}
}

@article{chen2020mam,
 author = {Chen, Junkun and Ma, Mingbo and Zheng, Renjie and Huang, Liang},
 journal = {ArXiv preprint},
 title = {Mam: Masked acoustic modeling for end-to-end speech-to-text translation},
 url = {https://arxiv.org/abs/2010.11445},
 volume = {abs/2010.11445},
 year = {2020}
}

@inproceedings{han-etal-2021-learning,
 address = {Online},
 author = {Han, Chi  and
Wang, Mingxuan  and
Ji, Heng  and
Li, Lei},
 booktitle = {Findings of ACL-IJCNLP 2021},
 doi = {10.18653/v1/2021.findings-acl.195},
 pages = {2214--2225},
 publisher = {Association for Computational Linguistics},
 title = {Learning Shared Semantic Space for Speech-to-Text Translation},
 url = {https://aclanthology.org/2021.findings-acl.195},
 year = {2021}
}

@inproceedings{sennrich-etal-2016-improving,
 address = {Berlin, Germany},
 author = {Sennrich, Rico  and
Haddow, Barry  and
Birch, Alexandra},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/P16-1009},
 pages = {86--96},
 publisher = {Association for Computational Linguistics},
 title = {Improving Neural Machine Translation Models with Monolingual Data},
 url = {https://aclanthology.org/P16-1009},
 year = {2016}
}

@article{wu2022wav2seq,
 author = {Wu, Felix and Kim, Kwangyoun and Watanabe, Shinji and Han, Kyu and McDonald, Ryan and Weinberger, Kilian Q and Artzi, Yoav},
 journal = {ArXiv preprint},
 title = {Wav2Seq: Pre-training Speech-to-Text Encoder-Decoder Models Using Pseudo Languages},
 url = {https://arxiv.org/abs/2205.01086},
 volume = {abs/2205.01086},
 year = {2022}
}

@inproceedings{ren2020fastspeech,
 author = {Yi Ren and
Chenxu Hu and
Xu Tan and
Tao Qin and
Sheng Zhao and
Zhou Zhao and
Tie{-}Yan Liu},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/0006H0QZZL21.bib},
 booktitle = {Proc. of ICLR},
 publisher = {OpenReview.net},
 timestamp = {Wed, 23 Jun 2021 01:00:00 +0200},
 title = {FastSpeech 2: Fast and High-Quality End-to-End Text to Speech},
 url = {https://openreview.net/forum?id=piLPYqxtWuA},
 year = {2021}
}

@inproceedings{kong2020hifi,
 author = {Jungil Kong and
Jaehyeon Kim and
Jaekyoung Bae},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/KongKB20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {HiFi-GAN: Generative Adversarial Networks for Efficient and High Fidelity
Speech Synthesis},
 url = {https://proceedings.neurips.cc/paper/2020/hash/c5d736809766d46260d816d8dbc9eb44-Abstract.html},
 year = {2020}
}

@inproceedings{chen2021gigaspeech,
 author = {Guoguo Chen and
Shuzhou Chai and
Guan{-}Bo Wang and
Jiayu Du and
Wei{-}Qiang Zhang and
Chao Weng and
Dan Su and
Daniel Povey and
Jan Trmal and
Junbo Zhang and
Mingjie Jin and
Sanjeev Khudanpur and
Shinji Watanabe and
Shuaijiang Zhao and
Wei Zou and
Xiangang Li and
Xuchen Yao and
Yongqing Wang and
Zhao You and
Zhiyong Yan},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/interspeech/ChenCWDZWSPTZJK21.bib},
 booktitle = {Proc. of INTERSPEECH},
 doi = {10.21437/Interspeech.2021-1965},
 editor = {Hynek Hermansky and
Honza Cernock{\'{y}} and
Luk{\'{a}}s Burget and
Lori Lamel and
Odette Scharenborg and
Petr Motl{\'{\i}}cek},
 pages = {3670--3674},
 publisher = {{ISCA}},
 timestamp = {Mon, 14 Mar 2022 00:00:00 +0100},
 title = {GigaSpeech: An Evolving, Multi-Domain {ASR} Corpus with 10, 000 Hours
of Transcribed Audio},
 url = {https://doi.org/10.21437/Interspeech.2021-1965},
 year = {2021}
}

@article{kreuk2021textless,
 author = {Kreuk, Felix and Polyak, Adam and Copet, Jade and Kharitonov, Eugene and Nguyen, Tu-Anh and Rivi{\`e}re, Morgane and Hsu, Wei-Ning and Mohamed, Abdelrahman and Dupoux, Emmanuel and Adi, Yossi},
 journal = {ArXiv preprint},
 title = {Textless speech emotion conversion using decomposed and discrete representations},
 url = {https://arxiv.org/abs/2111.07402},
 volume = {abs/2111.07402},
 year = {2021}
}

@inproceedings{polyak2021speech,
 author = {Adam Polyak and
Yossi Adi and
Jade Copet and
Eugene Kharitonov and
Kushal Lakhotia and
Wei{-}Ning Hsu and
Abdelrahman Mohamed and
Emmanuel Dupoux},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/interspeech/PolyakACKLHMD21.bib},
 booktitle = {Proc. of INTERSPEECH},
 doi = {10.21437/Interspeech.2021-475},
 editor = {Hynek Hermansky and
Honza Cernock{\'{y}} and
Luk{\'{a}}s Burget and
Lori Lamel and
Odette Scharenborg and
Petr Motl{\'{\i}}cek},
 pages = {3615--3619},
 publisher = {{ISCA}},
 timestamp = {Mon, 14 Mar 2022 00:00:00 +0100},
 title = {Speech Resynthesis from Discrete Disentangled Self-Supervised Representations},
 url = {https://doi.org/10.21437/Interspeech.2021-475},
 year = {2021}
}

@inproceedings{xia2019generalized,
 address = {Florence, Italy},
 author = {Xia, Mengzhou  and
Kong, Xiang  and
Anastasopoulos, Antonios  and
Neubig, Graham},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/P19-1579},
 pages = {5786--5796},
 publisher = {Association for Computational Linguistics},
 title = {Generalized Data Augmentation for Low-Resource Translation},
 url = {https://aclanthology.org/P19-1579},
 year = {2019}
}

@article{tang2020multilingual,
 author = {Tang, Yuqing and Tran, Chau and Li, Xian and Chen, Peng-Jen and Goyal, Naman and Chaudhary, Vishrav and Gu, Jiatao and Fan, Angela},
 journal = {ArXiv preprint},
 title = {Multilingual translation with extensible multilingual pretraining and finetuning},
 url = {https://arxiv.org/abs/2008.00401},
 volume = {abs/2008.00401},
 year = {2020}
}

@inproceedings{chen2020facebook,
 address = {Online},
 author = {Chen, Peng-Jen  and
Lee, Ann  and
Wang, Changhan  and
Goyal, Naman  and
Fan, Angela  and
Williamson, Mary  and
Gu, Jiatao},
 booktitle = {Proceedings of the Fifth Conference on Machine Translation},
 pages = {113--125},
 publisher = {Association for Computational Linguistics},
 title = {{F}acebook {AI}{'}s {WMT}20 News Translation Task Submission},
 url = {https://aclanthology.org/2020.wmt-1.8},
 year = {2020}
}

@inproceedings{bojar2011improving,
 address = {Edinburgh, Scotland},
 author = {Bojar, Ond{\v{r}}ej  and
Tamchyna, Ale{\v{s}}},
 booktitle = {Proceedings of the Sixth Workshop on Statistical Machine Translation},
 pages = {330--336},
 publisher = {Association for Computational Linguistics},
 title = {Improving Translation Model by Monolingual Data},
 url = {https://aclanthology.org/W11-2138},
 year = {2011}
}

@inproceedings{bertoldi2009domain,
 address = {Athens, Greece},
 author = {Bertoldi, Nicola  and
Federico, Marcello},
 booktitle = {Proceedings of the Fourth Workshop on Statistical Machine Translation},
 pages = {182--189},
 publisher = {Association for Computational Linguistics},
 title = {Domain Adaptation for Statistical Machine Translation with Monolingual Resources},
 url = {https://aclanthology.org/W09-0432},
 year = {2009}
}

@inproceedings{sennrich2016improving,
 address = {Berlin, Germany},
 author = {Sennrich, Rico  and
Haddow, Barry  and
Birch, Alexandra},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/P16-1009},
 pages = {86--96},
 publisher = {Association for Computational Linguistics},
 title = {Improving Neural Machine Translation Models with Monolingual Data},
 url = {https://aclanthology.org/P16-1009},
 year = {2016}
}

@inproceedings{hoang2018iterative,
 address = {Melbourne, Australia},
 author = {Hoang, Vu Cong Duy  and
Koehn, Philipp  and
Haffari, Gholamreza  and
Cohn, Trevor},
 booktitle = {Proceedings of the 2nd Workshop on Neural Machine Translation and Generation},
 doi = {10.18653/v1/W18-2703},
 pages = {18--24},
 publisher = {Association for Computational Linguistics},
 title = {Iterative Back-Translation for Neural Machine Translation},
 url = {https://aclanthology.org/W18-2703},
 year = {2018}
}

@inproceedings{imamura2018enhancement,
 address = {Melbourne, Australia},
 author = {Imamura, Kenji  and
Fujita, Atsushi  and
Sumita, Eiichiro},
 booktitle = {Proceedings of the 2nd Workshop on Neural Machine Translation and Generation},
 doi = {10.18653/v1/W18-2707},
 pages = {55--63},
 publisher = {Association for Computational Linguistics},
 title = {Enhancement of Encoder and Attention Using Target Monolingual Corpora in Neural Machine Translation},
 url = {https://aclanthology.org/W18-2707},
 year = {2018}
}

@inproceedings{adelani2022findings,
 author = {Adelani, David Ifeoluwa and Alam, Md Mahfuz Ibn and Anastasopoulos, Antonios and Bhagia, Akshita and Costa-Juss{\'a}, Marta and Dodge, Jesse and Faisal, Fahim and Federmann, Christian and Fedorova, Natalia and Guzm{\'a}n, Francisco and others},
 booktitle = {Proceedings of the Seventh Conference on Machine Translation, Online. Association for Computational Linguistics},
 title = {Findings of the WMT 2022 shared task on large-scale machine translation evaluation for african languages},
 year = {2022}
}

@inproceedings{wenzek2021findings,
 address = {Online},
 author = {Wenzek, Guillaume  and
Chaudhary, Vishrav  and
Fan, Angela  and
Gomez, Sahir  and
Goyal, Naman  and
Jain, Somya  and
Kiela, Douwe  and
Thrush, Tristan  and
Guzm{\'a}n, Francisco},
 booktitle = {Proceedings of the Sixth Conference on Machine Translation},
 pages = {89--99},
 publisher = {Association for Computational Linguistics},
 title = {Findings of the {WMT} 2021 Shared Task on Large-Scale Multilingual Machine Translation},
 url = {https://aclanthology.org/2021.wmt-1.2},
 year = {2021}
}

@inproceedings{farhad2021findings,
 address = {Copenhagen, Denmark},
 author = {Bojar, Ond{\v{r}}ej  and
Chatterjee, Rajen  and
Federmann, Christian  and
Graham, Yvette  and
Haddow, Barry  and
Huang, Shujian  and
Huck, Matthias  and
Koehn, Philipp  and
Liu, Qun  and
Logacheva, Varvara  and
Monz, Christof  and
Negri, Matteo  and
Post, Matt  and
Rubino, Raphael  and
Specia, Lucia  and
Turchi, Marco},
 booktitle = {Proceedings of the Second Conference on Machine Translation},
 doi = {10.18653/v1/W17-4717},
 pages = {169--214},
 publisher = {Association for Computational Linguistics},
 title = {Findings of the 2017 Conference on Machine Translation ({WMT}17)},
 url = {https://aclanthology.org/W17-4717},
 year = {2017}
}

@inproceedings{hayashi2018back,
 author = {Hayashi, Tomoki and Watanabe, Shinji and Zhang, Yu and Toda, Tomoki and Hori, Takaaki and Astudillo, Ramon and Takeda, Kazuya},
 booktitle = {2018 IEEE Spoken Language Technology Workshop (SLT)},
 organization = {IEEE},
 pages = {426--433},
 title = {Back-translation-style data augmentation for end-to-end ASR},
 year = {2018}
}

@inproceedings{ueno2021data,
 author = {Ueno, Sei and Mimura, Masato and Sakai, Shinsuke and Kawahara, Tatsuya},
 booktitle = {2021 IEEE Automatic Speech Recognition and Understanding Workshop (ASRU)},
 organization = {IEEE},
 pages = {68--75},
 title = {Data Augmentation for ASR Using TTS Via a Discrete Representation},
 year = {2021}
}

@inproceedings{tjandra2017listening,
 author = {Tjandra, Andros and Sakti, Sakriani and Nakamura, Satoshi},
 booktitle = {2017 IEEE Automatic Speech Recognition and Understanding Workshop (ASRU)},
 organization = {IEEE},
 pages = {301--308},
 title = {Listening while speaking: Speech chain by deep learning},
 year = {2017}
}

@inproceedings{zhang2022ustc,
 address = {Dublin, Ireland (in-person and online)},
 author = {Zhang, Weitai  and
Ye, Zhongyi  and
Tang, Haitao  and
Li, Xiaoxi  and
Zhou, Xinyuan  and
Yang, Jing  and
Cui, Jianwei  and
Deng, Pan  and
Shi, Mohan  and
Song, Yifan  and
Liu, Dan  and
Liu, Junhua  and
Dai, Lirong},
 booktitle = {Proceedings of the 19th International Conference on Spoken Language Translation (IWSLT 2022)},
 doi = {10.18653/v1/2022.iwslt-1.15},
 pages = {198--207},
 publisher = {Association for Computational Linguistics},
 title = {The {USTC}-{NELSLIP} Offline Speech Translation Systems for {IWSLT} 2022},
 url = {https://aclanthology.org/2022.iwslt-1.15},
 year = {2022}
}

@article{bapna2022mslam,
 author = {Bapna, Ankur and Cherry, Colin and Zhang, Yu and Jia, Ye and Johnson, Melvin and Cheng, Yong and Khanuja, Simran and Riesa, Jason and Conneau, Alexis},
 journal = {ArXiv preprint},
 title = {mSLAM: Massively multilingual joint pre-training for speech and text},
 url = {https://arxiv.org/abs/2202.01374},
 volume = {abs/2202.01374},
 year = {2022}
}

@article{babu2021xls,
 author = {Babu, Arun and Wang, Changhan and Tjandra, Andros and Lakhotia, Kushal and Xu, Qiantong and Goyal, Naman and Singh, Kritika and von Platen, Patrick and Saraf, Yatharth and Pino, Juan and others},
 journal = {ArXiv preprint},
 title = {XLS-R: Self-supervised cross-lingual speech representation learning at scale},
 url = {https://arxiv.org/abs/2111.09296},
 volume = {abs/2111.09296},
 year = {2021}
}

@inproceedings{li2021multilingual,
 address = {Online},
 author = {Li, Xian  and
Wang, Changhan  and
Tang, Yun  and
Tran, Chau  and
Tang, Yuqing  and
Pino, Juan  and
Baevski, Alexei  and
Conneau, Alexis  and
Auli, Michael},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2021.acl-long.68},
 pages = {827--838},
 publisher = {Association for Computational Linguistics},
 title = {Multilingual Speech Translation from Efficient Finetuning of Pretrained Models},
 url = {https://aclanthology.org/2021.acl-long.68},
 year = {2021}
}

@inproceedings{ardila-etal-2020-common,
 address = {Marseille, France},
 author = {Ardila, Rosana  and
Branson, Megan  and
Davis, Kelly  and
Kohler, Michael  and
Meyer, Josh  and
Henretty, Michael  and
Morais, Reuben  and
Saunders, Lindsay  and
Tyers, Francis  and
Weber, Gregor},
 booktitle = {Proceedings of the Twelfth Language Resources and Evaluation Conference},
 isbn = {979-10-95546-34-4},
 language = {English},
 pages = {4218--4222},
 publisher = {European Language Resources Association},
 title = {Common Voice: A Massively-Multilingual Speech Corpus},
 url = {https://aclanthology.org/2020.lrec-1.520},
 year = {2020}
}

@inproceedings{ott2019fairseq,
 address = {Minneapolis, Minnesota},
 author = {Ott, Myle  and
Edunov, Sergey  and
Baevski, Alexei  and
Fan, Angela  and
Gross, Sam  and
Ng, Nathan  and
Grangier, David  and
Auli, Michael},
 booktitle = {Proceedings of the 2019 Conference of the North {A}merican Chapter of the Association for Computational Linguistics (Demonstrations)},
 doi = {10.18653/v1/N19-4009},
 pages = {48--53},
 publisher = {Association for Computational Linguistics},
 title = {fairseq: A Fast, Extensible Toolkit for Sequence Modeling},
 url = {https://aclanthology.org/N19-4009},
 year = {2019}
}

@inproceedings{bojar-EtAl:2016:WMT1,
 address = {Berlin, Germany},
 author = {Bojar, Ond{\v{r}}ej  and
Chatterjee, Rajen  and
Federmann, Christian  and
Graham, Yvette  and
Haddow, Barry  and
Huck, Matthias  and
Jimeno Yepes, Antonio  and
Koehn, Philipp  and
Logacheva, Varvara  and
Monz, Christof  and
Negri, Matteo  and
N{\'e}v{\'e}ol, Aur{\'e}lie  and
Neves, Mariana  and
Popel, Martin  and
Post, Matt  and
Rubino, Raphael  and
Scarton, Carolina  and
Specia, Lucia  and
Turchi, Marco  and
Verspoor, Karin  and
Zampieri, Marcos},
 booktitle = {Proceedings of the First Conference on Machine Translation: Volume 2, Shared Task Papers},
 doi = {10.18653/v1/W16-2301},
 pages = {131--198},
 publisher = {Association for Computational Linguistics},
 title = {Findings of the 2016 Conference on Machine Translation},
 url = {https://aclanthology.org/W16-2301},
 year = {2016}
}

@inproceedings{schwenk2019ccmatrix,
 address = {Online},
 author = {Schwenk, Holger  and
Wenzek, Guillaume  and
Edunov, Sergey  and
Grave, Edouard  and
Joulin, Armand  and
Fan, Angela},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2021.acl-long.507},
 pages = {6490--6500},
 publisher = {Association for Computational Linguistics},
 title = {{CCM}atrix: Mining Billions of High-Quality Parallel Sentences on the Web},
 url = {https://aclanthology.org/2021.acl-long.507},
 year = {2021}
}


==> rebib_custom.tex <==
@inproceedings{lee2022textless,
 address = {Seattle, United States},
 author = {Lee, Ann  and
Gong, Hongyu  and
Duquenne, Paul-Ambroise  and
Schwenk, Holger  and
Chen, Peng-Jen  and
Wang, Changhan  and
Popuri, Sravya  and
Adi, Yossi  and
Pino, Juan  and
Gu, Jiatao  and
Hsu, Wei-Ning},
 booktitle = {Proceedings of the 2022 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies},
 doi = {10.18653/v1/2022.naacl-main.63},
 pages = {860--872},
 publisher = {Association for Computational Linguistics},
 title = {Textless Speech-to-Speech Translation on Real Data},
 url = {https://aclanthology.org/2022.naacl-main.63},
 year = {2022}
}

@article{lakhotia2021generative,
 address = {Cambridge, MA},
 author = {Lakhotia, Kushal  and
Kharitonov, Eugene  and
Hsu, Wei-Ning  and
Adi, Yossi  and
Polyak, Adam  and
Bolte, Benjamin  and
Nguyen, Tu-Anh  and
Copet, Jade  and
Baevski, Alexei  and
Mohamed, Abdelrahman  and
Dupoux, Emmanuel},
 doi = {10.1162/tacl_a_00430},
 journal = {Transactions of the Association for Computational Linguistics},
 pages = {1336--1354},
 publisher = {MIT Press},
 title = {On Generative Spoken Language Modeling from Raw Audio},
 url = {https://aclanthology.org/2021.tacl-1.79},
 volume = {9},
 year = {2021}
}

@article{inaguma2022unity,
 author = {Inaguma, Hirofumi and Popuri, Sravya and Kulikov, Ilia and Chen, Peng-Jen and Wang, Changhan and Chung, Yu-An and Tang, Yun and Lee, Ann and Watanabe, Shinji and Pino, Juan},
 journal = {ArXiv preprint},
 title = {UnitY: Two-pass Direct Speech-to-speech Translation with Discrete Units},
 url = {https://arxiv.org/abs/2212.08055},
 volume = {abs/2212.08055},
 year = {2022}
}

@article{popuri2022enhanced,
 author = {Popuri, Sravya and Chen, Peng-Jen and Wang, Changhan and Pino, Juan and Adi, Yossi and Gu, Jiatao and Hsu, Wei-Ning and Lee, Ann},
 journal = {ArXiv preprint},
 title = {Enhanced Direct Speech-to-Speech Translation Using Self-supervised Pre-training and Data Augmentation},
 url = {https://arxiv.org/abs/2204.02967},
 volume = {abs/2204.02967},
 year = {2022}
}

@article{huang2022transpeech,
 author = {Huang, Rongjie and Zhao, Zhou and Liu, Jinglin and Liu, Huadai and Ren, Yi and Zhang, Lichao and He, Jinzheng},
 journal = {ArXiv preprint},
 title = {TranSpeech: Speech-to-Speech Translation With Bilateral Perturbation},
 url = {https://arxiv.org/abs/2205.12523},
 volume = {abs/2205.12523},
 year = {2022}
}

@inproceedings{kharitonov2022text,
 address = {Dublin, Ireland},
 author = {Kharitonov, Eugene  and
Lee, Ann  and
Polyak, Adam  and
Adi, Yossi  and
Copet, Jade  and
Lakhotia, Kushal  and
Nguyen, Tu Anh  and
Riviere, Morgane  and
Mohamed, Abdelrahman  and
Dupoux, Emmanuel  and
Hsu, Wei-Ning},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2022.acl-long.593},
 pages = {8666--8681},
 publisher = {Association for Computational Linguistics},
 title = {Text-Free Prosody-Aware Generative Spoken Language Modeling},
 url = {https://aclanthology.org/2022.acl-long.593},
 year = {2022}
}

@article{chen2022wavlm,
 author = {Chen, Sanyuan and Wang, Chengyi and Chen, Zhengyang and Wu, Yu and Liu, Shujie and Chen, Zhuo and Li, Jinyu and Kanda, Naoyuki and Yoshioka, Takuya and Xiao, Xiong and others},
 journal = {IEEE Journal of Selected Topics in Signal Processing},
 number = {6},
 pages = {1505--1518},
 publisher = {IEEE},
 title = {Wavlm: Large-scale self-supervised pre-training for full stack speech processing},
 volume = {16},
 year = {2022}
}

@inproceedings{chung2021w2v,
 author = {Chung, Yu-An and Zhang, Yu and Han, Wei and Chiu, Chung-Cheng and Qin, James and Pang, Ruoming and Wu, Yonghui},
 booktitle = {2021 IEEE Automatic Speech Recognition and Understanding Workshop (ASRU)},
 organization = {IEEE},
 pages = {244--250},
 title = {W2v-bert: Combining contrastive learning and masked language modeling for self-supervised speech pre-training},
 year = {2021}
}

@article{zhang2022speechlm,
 author = {Zhang, Ziqiang and Chen, Sanyuan and Zhou, Long and Wu, Yu and Ren, Shuo and Liu, Shujie and Yao, Zhuoyuan and Gong, Xun and Dai, Lirong and Li, Jinyu and others},
 journal = {ArXiv preprint},
 title = {Speechlm: Enhanced speech pre-training with unpaired textual data},
 url = {https://arxiv.org/abs/2209.15329},
 volume = {abs/2209.15329},
 year = {2022}
}

@inproceedings{berard2016listen,
 author = {B{\'e}rard, Alexandre and Pietquin, Olivier and Besacier, Laurent and Servan, Christophe},
 booktitle = {NIPS Workshop on end-to-end learning for speech and audio processing},
 title = {Listen and Translate: A Proof of Concept for End-to-End Speech-to-Text Translation},
 year = {2016}
}

@inproceedings{di2019adapting,
 author = {Mattia Antonino Di Gangi and
Matteo Negri and
Marco Turchi},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/interspeech/GangiNT19.bib},
 booktitle = {Proc. of INTERSPEECH},
 doi = {10.21437/Interspeech.2019-3045},
 editor = {Gernot Kubin and
Zdravko Kacic},
 pages = {1133--1137},
 publisher = {{ISCA}},
 timestamp = {Fri, 29 Jan 2021 00:00:00 +0100},
 title = {Adapting Transformer to End-to-End Spoken Language Translation},
 url = {https://doi.org/10.21437/Interspeech.2019-3045},
 year = {2019}
}

@inproceedings{gaido2021ctc,
 address = {Online},
 author = {Gaido, Marco  and
Cettolo, Mauro  and
Negri, Matteo  and
Turchi, Marco},
 booktitle = {Proceedings of the 16th Conference of the European Chapter of the Association for Computational Linguistics: Main Volume},
 doi = {10.18653/v1/2021.eacl-main.57},
 pages = {690--696},
 publisher = {Association for Computational Linguistics},
 title = {{CTC}-based Compression for Direct Speech Translation},
 url = {https://aclanthology.org/2021.eacl-main.57},
 year = {2021}
}

@inproceedings{dong2021listen,
 author = {Dong, Qianqian and Ye, Rong and Wang, Mingxuan and Zhou, Hao and Xu, Shuang and Xu, Bo and Li, Lei},
 booktitle = {Proc. of AAAI},
 pages = {12749--12759},
 title = {Listen, understand and translate: Triple supervision decouples end-to-end speech-to-text translation},
 year = {2021}
}

@inproceedings{dong2021consecutive,
 author = {Dong, Qianqian and Wang, Mingxuan and Zhou, Hao and Xu, Shuang and Xu, Bo and Li, Lei},
 booktitle = {Proc. of AAAI},
 pages = {12738--12748},
 title = {Consecutive decoding for speech-to-text translation},
 year = {2021}
}

@inproceedings{xu2021stacked,
 address = {Online},
 author = {Xu, Chen  and
Hu, Bojie  and
Li, Yanyang  and
Zhang, Yuhao  and
Huang, Shen  and
Ju, Qi  and
Xiao, Tong  and
Zhu, Jingbo},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2021.acl-long.204},
 pages = {2619--2630},
 publisher = {Association for Computational Linguistics},
 title = {Stacked Acoustic-and-Textual Encoding: Integrating the Pre-trained Models into Speech Translation Encoders},
 url = {https://aclanthology.org/2021.acl-long.204},
 year = {2021}
}

@inproceedings{zhang2020adaptive,
 address = {Online},
 author = {Zhang, Biao  and
Titov, Ivan  and
Haddow, Barry  and
Sennrich, Rico},
 booktitle = {Findings of the Association for Computational Linguistics: EMNLP 2020},
 doi = {10.18653/v1/2020.findings-emnlp.230},
 pages = {2533--2544},
 publisher = {Association for Computational Linguistics},
 title = {Adaptive Feature Selection for End-to-End Speech Translation},
 url = {https://aclanthology.org/2020.findings-emnlp.230},
 year = {2020}
}

@inproceedings{wang2021voxpopuli,
 address = {Online},
 author = {Wang, Changhan  and
Riviere, Morgane  and
Lee, Ann  and
Wu, Anne  and
Talnikar, Chaitanya  and
Haziza, Daniel  and
Williamson, Mary  and
Pino, Juan  and
Dupoux, Emmanuel},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2021.acl-long.80},
 pages = {993--1003},
 publisher = {Association for Computational Linguistics},
 title = {{V}ox{P}opuli: A Large-Scale Multilingual Speech Corpus for Representation Learning, Semi-Supervised Learning and Interpretation},
 url = {https://aclanthology.org/2021.acl-long.80},
 year = {2021}
}

@inproceedings{di2019must,
 address = {Minneapolis, Minnesota},
 author = {Di Gangi, Mattia A.  and
Cattoni, Roldano  and
Bentivogli, Luisa  and
Negri, Matteo  and
Turchi, Marco},
 booktitle = {Proc. of NAACL-HLT},
 doi = {10.18653/v1/N19-1202},
 pages = {2012--2017},
 publisher = {Association for Computational Linguistics},
 title = {{M}u{ST}-{C}: a {M}ultilingual {S}peech {T}ranslation {C}orpus},
 url = {https://aclanthology.org/N19-1202},
 year = {2019}
}

@inproceedings{wang2021covost,
 author = {Changhan Wang and
Anne Wu and
Jiatao Gu and
Juan Pino},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/interspeech/WangWGP21.bib},
 booktitle = {Proc. of INTERSPEECH},
 doi = {10.21437/Interspeech.2021-2027},
 editor = {Hynek Hermansky and
Honza Cernock{\'{y}} and
Luk{\'{a}}s Burget and
Lori Lamel and
Odette Scharenborg and
Petr Motl{\'{\i}}cek},
 pages = {2247--2251},
 publisher = {{ISCA}},
 timestamp = {Mon, 14 Mar 2022 00:00:00 +0100},
 title = {CoVoST 2 and Massively Multilingual Speech Translation},
 url = {https://doi.org/10.21437/Interspeech.2021-2027},
 year = {2021}
}

@inproceedings{zhao2021neurst,
 address = {Online},
 author = {Zhao, Chengqi  and
Wang, Mingxuan  and
Dong, Qianqian  and
Ye, Rong  and
Li, Lei},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2021.acl-demo.7},
 pages = {55--62},
 publisher = {Association for Computational Linguistics},
 title = {{N}eur{ST}: Neural Speech Translation Toolkit},
 url = {https://aclanthology.org/2021.acl-demo.7},
 year = {2021}
}

@inproceedings{du2022regularizing,
 author = {Du, Yichao and Zhang, Zhirui and Wang, Weizhi and Chen, Boxing and Xie, Jun and Xu, Tong},
 booktitle = {Proc. of AAAI},
 pages = {10590--10598},
 title = {Regularizing end-to-end speech translation with triangular decomposition agreement},
 year = {2022}
}

@inproceedings{pino2020selfa,
 author = {Juan Miguel Pino and
Qiantong Xu and
Xutai Ma and
Mohammad Javad Dousti and
Yun Tang},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/interspeech/PinoXMDT20.bib},
 booktitle = {Proc. of INTERSPEECH},
 doi = {10.21437/Interspeech.2020-2938},
 editor = {Helen Meng and
Bo Xu and
Thomas Fang Zheng},
 pages = {1476--1480},
 publisher = {{ISCA}},
 timestamp = {Thu, 12 Aug 2021 01:00:00 +0200},
 title = {Self-Training for End-to-End Speech Translation},
 url = {https://doi.org/10.21437/Interspeech.2020-2938},
 year = {2020}
}

@inproceedings{inaguma2020espnet,
 address = {Online},
 author = {Inaguma, Hirofumi  and
Kiyono, Shun  and
Duh, Kevin  and
Karita, Shigeki  and
Yalta, Nelson  and
Hayashi, Tomoki  and
Watanabe, Shinji},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2020.acl-demos.34},
 pages = {302--311},
 publisher = {Association for Computational Linguistics},
 title = {{ESP}net-{ST}: All-in-One Speech Translation Toolkit},
 url = {https://aclanthology.org/2020.acl-demos.34},
 year = {2020}
}

@inproceedings{papi2021speechformer,
 address = {Online and Punta Cana, Dominican Republic},
 author = {Papi, Sara  and
Gaido, Marco  and
Negri, Matteo  and
Turchi, Marco},
 booktitle = {Proc. of EMNLP},
 doi = {10.18653/v1/2021.emnlp-main.127},
 pages = {1698--1706},
 publisher = {Association for Computational Linguistics},
 title = {Speechformer: Reducing Information Loss in Direct Speech Translation},
 url = {https://aclanthology.org/2021.emnlp-main.127},
 year = {2021}
}

@inproceedings{ye2021end,
 author = {Rong Ye and
Mingxuan Wang and
Lei Li},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/interspeech/YeW021.bib},
 booktitle = {Proc. of INTERSPEECH},
 doi = {10.21437/Interspeech.2021-1065},
 editor = {Hynek Hermansky and
Honza Cernock{\'{y}} and
Luk{\'{a}}s Burget and
Lori Lamel and
Odette Scharenborg and
Petr Motl{\'{\i}}cek},
 pages = {2267--2271},
 publisher = {{ISCA}},
 timestamp = {Mon, 14 Mar 2022 00:00:00 +0100},
 title = {End-to-End Speech Translation via Cross-Modal Progressive Training},
 url = {https://doi.org/10.21437/Interspeech.2021-1065},
 year = {2021}
}

@inproceedings{ye2022cross,
 address = {Seattle, United States},
 author = {Ye, Rong  and
Wang, Mingxuan  and
Li, Lei},
 booktitle = {Proceedings of the 2022 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies},
 doi = {10.18653/v1/2022.naacl-main.376},
 pages = {5099--5113},
 publisher = {Association for Computational Linguistics},
 title = {Cross-modal Contrastive Learning for Speech Translation},
 url = {https://aclanthology.org/2022.naacl-main.376},
 year = {2022}
}

@inproceedings{tang2021improving,
 address = {Online},
 author = {Tang, Yun  and
Pino, Juan  and
Li, Xian  and
Wang, Changhan  and
Genzel, Dmitriy},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2021.acl-long.328},
 pages = {4252--4261},
 publisher = {Association for Computational Linguistics},
 title = {Improving Speech Translation by Understanding and Learning from the Auxiliary Text Translation Task},
 url = {https://aclanthology.org/2021.acl-long.328},
 year = {2021}
}

@inproceedings{zhang2022revisiting,
 author = {Zhang, Biao and Haddow, Barry and Sennrich, Rico},
 booktitle = {Proc. of ICML},
 title = {Revisiting End-to-End Speech-to-Text Translation From Scratch},
 year = {2022}
}

@inproceedings{tang2022unified,
 address = {Dublin, Ireland},
 author = {Tang, Yun  and
Gong, Hongyu  and
Dong, Ning  and
Wang, Changhan  and
Hsu, Wei-Ning  and
Gu, Jiatao  and
Baevski, Alexei  and
Li, Xian  and
Mohamed, Abdelrahman  and
Auli, Michael  and
Pino, Juan},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2022.acl-long.105},
 pages = {1488--1499},
 publisher = {Association for Computational Linguistics},
 title = {Unified Speech-Text Pre-training for Speech Translation and Recognition},
 url = {https://aclanthology.org/2022.acl-long.105},
 year = {2022}
}

@inproceedings{fang2022stemm,
 address = {Dublin, Ireland},
 author = {Fang, Qingkai  and
Ye, Rong  and
Li, Lei  and
Feng, Yang  and
Wang, Mingxuan},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2022.acl-long.486},
 pages = {7050--7062},
 publisher = {Association for Computational Linguistics},
 title = {{STEMM}: Self-learning with Speech-text Manifold Mixup for Speech Translation},
 url = {https://aclanthology.org/2022.acl-long.486},
 year = {2022}
}

@inproceedings{zheng2021fused,
 author = {Renjie Zheng and
Junkun Chen and
Mingbo Ma and
Liang Huang},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/ZhengCM021.bib},
 booktitle = {Proc. of ICML},
 editor = {Marina Meila and
Tong Zhang},
 pages = {12736--12746},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Wed, 25 Aug 2021 01:00:00 +0200},
 title = {Fused Acoustic and Text Encoding for Multimodal Bilingual Pretraining
and Speech Translation},
 url = {http://proceedings.mlr.press/v139/zheng21a.html},
 volume = {139},
 year = {2021}
}

@article{karakanta2018neural,
 author = {Karakanta, Alina and Dehdari, Jon and van Genabith, Josef},
 journal = {Machine Translation},
 number = {1},
 pages = {167--189},
 publisher = {Springer},
 title = {Neural machine translation for low-resource languages without parallel corpora},
 volume = {32},
 year = {2018}
}

@inproceedings{anastasopoulos2018tied,
 address = {New Orleans, Louisiana},
 author = {Anastasopoulos, Antonios  and
Chiang, David},
 booktitle = {Proc. of NAACL-HLT},
 doi = {10.18653/v1/N18-1008},
 pages = {82--91},
 publisher = {Association for Computational Linguistics},
 title = {Tied Multitask Learning for Neural Speech Translation},
 url = {https://aclanthology.org/N18-1008},
 year = {2018}
}

@inproceedings{indurthi2021task,
 author = {Indurthi, Sathish and Zaidi, Mohd Abbas and Lakumarapu, Nikhil Kumar and Lee, Beomseok and Han, Hyojung and Ahn, Seokchan and Kim, Sangha and Kim, Chanwoo and Hwang, Inchul},
 booktitle = {Proc. of ICASSP},
 organization = {IEEE},
 pages = {7723--7727},
 title = {Task aware multi-task learning for speech to text tasks},
 year = {2021}
}

@inproceedings{schneider2019wav2vec,
 author = {Steffen Schneider and
Alexei Baevski and
Ronan Collobert and
Michael Auli},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/interspeech/SchneiderBCA19.bib},
 booktitle = {Proc. of INTERSPEECH},
 doi = {10.21437/Interspeech.2019-1873},
 editor = {Gernot Kubin and
Zdravko Kacic},
 pages = {3465--3469},
 publisher = {{ISCA}},
 timestamp = {Fri, 29 Jan 2021 00:00:00 +0100},
 title = {wav2vec: Unsupervised Pre-Training for Speech Recognition},
 url = {https://doi.org/10.21437/Interspeech.2019-1873},
 year = {2019}
}

@inproceedings{dong2018speech,
 author = {Linhao Dong and
Shuang Xu and
Bo Xu},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icassp/DongXX18.bib},
 booktitle = {2018 {IEEE} International Conference on Acoustics, Speech and Signal
Processing, {ICASSP} 2018, Calgary, AB, Canada, April 15-20, 2018},
 doi = {10.1109/ICASSP.2018.8462506},
 pages = {5884--5888},
 publisher = {{IEEE}},
 timestamp = {Tue, 25 Jun 2019 01:00:00 +0200},
 title = {Speech-Transformer: {A} No-Recurrence Sequence-to-Sequence Model for
Speech Recognition},
 url = {https://doi.org/10.1109/ICASSP.2018.8462506},
 year = {2018}
}

@inproceedings{baevski2020wav2vec,
 author = {Alexei Baevski and
Yuhao Zhou and
Abdelrahman Mohamed and
Michael Auli},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/BaevskiZMA20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {wav2vec 2.0: {A} Framework for Self-Supervised Learning of Speech
Representations},
 url = {https://proceedings.neurips.cc/paper/2020/hash/92d1e1eb1cd6f9fba3227870bb6d7f07-Abstract.html},
 year = {2020}
}

@inproceedings{van2017neural,
 author = {A{\"{a}}ron van den Oord and
Oriol Vinyals and
Koray Kavukcuoglu},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/OordVK17.bib},
 booktitle = {Advances in Neural Information Processing Systems 30: Annual Conference
on Neural Information Processing Systems 2017, December 4-9, 2017,
Long Beach, CA, {USA}},
 editor = {Isabelle Guyon and
Ulrike von Luxburg and
Samy Bengio and
Hanna M. Wallach and
Rob Fergus and
S. V. N. Vishwanathan and
Roman Garnett},
 pages = {6306--6315},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Neural Discrete Representation Learning},
 url = {https://proceedings.neurips.cc/paper/2017/hash/7a98af17e63a0ac09ce2e96d03992fbc-Abstract.html},
 year = {2017}
}

@inproceedings{dunbar2019zero,
 author = {Ewan Dunbar and
Robin Algayres and
Julien Karadayi and
Mathieu Bernard and
Juan Benjumea and
Xuan{-}Nga Cao and
Lucie Miskic and
Charlotte Dugrain and
Lucas Ondel and
Alan W. Black and
Laurent Besacier and
Sakriani Sakti and
Emmanuel Dupoux},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/interspeech/DunbarAKBBCMDOB19.bib},
 booktitle = {Proc. of INTERSPEECH},
 doi = {10.21437/Interspeech.2019-2904},
 editor = {Gernot Kubin and
Zdravko Kacic},
 pages = {1088--1092},
 publisher = {{ISCA}},
 timestamp = {Fri, 29 Jan 2021 00:00:00 +0100},
 title = {The Zero Resource Speech Challenge 2019: {TTS} Without {T}},
 url = {https://doi.org/10.21437/Interspeech.2019-2904},
 year = {2019}
}

@inproceedings{zhang2021uwspeech,
 author = {Zhang, Chen and Tan, Xu and Ren, Yi and Qin, Tao and Zhang, Kejun and Liu, Tie-Yan},
 booktitle = {Proc. of the AAAI},
 pages = {14319--14327},
 title = {Uwspeech: Speech to speech translation for unwritten languages},
 year = {2021}
}

@inproceedings{baevski2019vq,
 author = {Alexei Baevski and
Steffen Schneider and
Michael Auli},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/BaevskiSA20.bib},
 booktitle = {Proc. of ICLR},
 publisher = {OpenReview.net},
 timestamp = {Thu, 07 May 2020 01:00:00 +0200},
 title = {vq-wav2vec: Self-Supervised Learning of Discrete Speech Representations},
 url = {https://openreview.net/forum?id=rylwJxrYDS},
 year = {2020}
}

@article{meng2022cobert,
 author = {Meng, Chutong and Ao, Junyi and Ko, Tom and Wang, Mingxuan and Li, Haizhou},
 journal = {ArXiv preprint},
 title = {CoBERT: Self-Supervised Speech Representation Learning Through Code Representation Learning},
 url = {https://arxiv.org/abs/2210.04062},
 volume = {abs/2210.04062},
 year = {2022}
}

@article{lu2022unsupervised,
 author = {Lu, Zhiyun and Wang, Yongqiang and Zhang, Yu and Han, Wei and Chen, Zhehuai and Haghani, Parisa},
 journal = {ArXiv preprint},
 title = {Unsupervised Data Selection via Discrete Speech Representation for ASR},
 url = {https://arxiv.org/abs/2204.01981},
 volume = {abs/2204.01981},
 year = {2022}
}

@inproceedings{liu2019end,
 author = {Yuchen Liu and
Hao Xiong and
Jiajun Zhang and
Zhongjun He and
Hua Wu and
Haifeng Wang and
Chengqing Zong},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/interspeech/LiuXZHWWZ19.bib},
 booktitle = {Proc. of INTERSPEECH},
 doi = {10.21437/Interspeech.2019-2582},
 editor = {Gernot Kubin and
Zdravko Kacic},
 pages = {1128--1132},
 publisher = {{ISCA}},
 timestamp = {Tue, 27 Jul 2021 01:00:00 +0200},
 title = {End-to-End Speech Translation with Knowledge Distillation},
 url = {https://doi.org/10.21437/Interspeech.2019-2582},
 year = {2019}
}

@inproceedings{ye2020variational,
 author = {Rong Ye and
Wenxian Shi and
Hao Zhou and
Zhongyu Wei and
Lei Li},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/YeS0W020.bib},
 booktitle = {Proc. of ICLR},
 publisher = {OpenReview.net},
 timestamp = {Wed, 09 Sep 2020 01:00:00 +0200},
 title = {Variational Template Machine for Data-to-Text Generation},
 url = {https://openreview.net/forum?id=HkejNgBtPB},
 year = {2020}
}

@article{hsu2021hubert,
 author = {Hsu, Wei-Ning and Bolte, Benjamin and Tsai, Yao-Hung Hubert and Lakhotia, Kushal and Salakhutdinov, Ruslan and Mohamed, Abdelrahman},
 journal = {IEEE/ACM Transactions on Audio, Speech, and Language Processing},
 pages = {3451--3460},
 publisher = {IEEE},
 title = {Hubert: Self-supervised speech representation learning by masked prediction of hidden units},
 volume = {29},
 year = {2021}
}

@inproceedings{vaswani2017attention,
 author = {Ashish Vaswani and
Noam Shazeer and
Niki Parmar and
Jakob Uszkoreit and
Llion Jones and
Aidan N. Gomez and
Lukasz Kaiser and
Illia Polosukhin},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/VaswaniSPUJGKP17.bib},
 booktitle = {Advances in Neural Information Processing Systems 30: Annual Conference
on Neural Information Processing Systems 2017, December 4-9, 2017,
Long Beach, CA, {USA}},
 editor = {Isabelle Guyon and
Ulrike von Luxburg and
Samy Bengio and
Hanna M. Wallach and
Rob Fergus and
S. V. N. Vishwanathan and
Roman Garnett},
 pages = {5998--6008},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Attention is All you Need},
 url = {https://proceedings.neurips.cc/paper/2017/hash/3f5ee243547dee91fbd053c1c4a845aa-Abstract.html},
 year = {2017}
}

@article{liu2020multilingual,
 address = {Cambridge, MA},
 author = {Liu, Yinhan  and
Gu, Jiatao  and
Goyal, Naman  and
Li, Xian  and
Edunov, Sergey  and
Ghazvininejad, Marjan  and
Lewis, Mike  and
Zettlemoyer, Luke},
 doi = {10.1162/tacl_a_00343},
 journal = {Transactions of the Association for Computational Linguistics},
 pages = {726--742},
 publisher = {MIT Press},
 title = {Multilingual Denoising Pre-training for Neural Machine Translation},
 url = {https://aclanthology.org/2020.tacl-1.47},
 volume = {8},
 year = {2020}
}

@inproceedings{wang-etal-2020-fairseq,
 address = {Suzhou, China},
 author = {Wang, Changhan  and
Tang, Yun  and
Ma, Xutai  and
Wu, Anne  and
Okhonko, Dmytro  and
Pino, Juan},
 booktitle = {Proceedings of the 1st Conference of the Asia-Pacific Chapter of the Association for Computational Linguistics and the 10th International Joint Conference on Natural Language Processing: System Demonstrations},
 pages = {33--39},
 publisher = {Association for Computational Linguistics},
 title = {Fairseq {S}2{T}: Fast Speech-to-Text Modeling with Fairseq},
 url = {https://aclanthology.org/2020.aacl-demo.6},
 year = {2020}
}

@inproceedings{edunov-etal-2018-understanding,
 address = {Brussels, Belgium},
 author = {Edunov, Sergey  and
Ott, Myle  and
Auli, Michael  and
Grangier, David},
 booktitle = {Proc. of EMNLP},
 doi = {10.18653/v1/D18-1045},
 pages = {489--500},
 publisher = {Association for Computational Linguistics},
 title = {Understanding Back-Translation at Scale},
 url = {https://aclanthology.org/D18-1045},
 year = {2018}
}

@inproceedings{ao2022speecht5,
 address = {Dublin, Ireland},
 author = {Ao, Junyi  and
Wang, Rui  and
Zhou, Long  and
Wang, Chengyi  and
Ren, Shuo  and
Wu, Yu  and
Liu, Shujie  and
Ko, Tom  and
Li, Qing  and
Zhang, Yu  and
Wei, Zhihua  and
Qian, Yao  and
Li, Jinyu  and
Wei, Furu},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2022.acl-long.393},
 pages = {5723--5738},
 publisher = {Association for Computational Linguistics},
 title = {{S}peech{T}5: Unified-Modal Encoder-Decoder Pre-Training for Spoken Language Processing},
 url = {https://aclanthology.org/2022.acl-long.393},
 year = {2022}
}

@inproceedings{caswell2019tagged,
 address = {Florence, Italy},
 author = {Caswell, Isaac  and
Chelba, Ciprian  and
Grangier, David},
 booktitle = {Proceedings of the Fourth Conference on Machine Translation (Volume 1: Research Papers)},
 doi = {10.18653/v1/W19-5206},
 pages = {53--63},
 publisher = {Association for Computational Linguistics},
 title = {Tagged Back-Translation},
 url = {https://aclanthology.org/W19-5206},
 year = {2019}
}

@inproceedings{kudo-richardson-2018-sentencepiece,
 address = {Brussels, Belgium},
 author = {Kudo, Taku  and
Richardson, John},
 booktitle = {Proc. of EMNLP},
 doi = {10.18653/v1/D18-2012},
 pages = {66--71},
 publisher = {Association for Computational Linguistics},
 title = {{S}entence{P}iece: A simple and language independent subword tokenizer and detokenizer for Neural Text Processing},
 url = {https://aclanthology.org/D18-2012},
 year = {2018}
}

@inproceedings{panayotov2015librispeech,
 author = {Vassil Panayotov and
Guoguo Chen and
Daniel Povey and
Sanjeev Khudanpur},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icassp/PanayotovCPK15.bib},
 booktitle = {2015 {IEEE} International Conference on Acoustics, Speech and Signal
Processing, {ICASSP} 2015, South Brisbane, Queensland, Australia,
April 19-24, 2015},
 doi = {10.1109/ICASSP.2015.7178964},
 pages = {5206--5210},
 publisher = {{IEEE}},
 timestamp = {Fri, 25 Dec 2020 00:00:00 +0100},
 title = {Librispeech: An {ASR} corpus based on public domain audio books},
 url = {https://doi.org/10.1109/ICASSP.2015.7178964},
 year = {2015}
}

@inproceedings{lee-etal-2022-textless,
 address = {Seattle, United States},
 author = {Lee, Ann  and
Gong, Hongyu  and
Duquenne, Paul-Ambroise  and
Schwenk, Holger  and
Chen, Peng-Jen  and
Wang, Changhan  and
Popuri, Sravya  and
Adi, Yossi  and
Pino, Juan  and
Gu, Jiatao  and
Hsu, Wei-Ning},
 booktitle = {Proceedings of the 2022 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies},
 doi = {10.18653/v1/2022.naacl-main.63},
 pages = {860--872},
 publisher = {Association for Computational Linguistics},
 title = {Textless Speech-to-Speech Translation on Real Data},
 url = {https://aclanthology.org/2022.naacl-main.63},
 year = {2022}
}

@inproceedings{zhang2022speechut,
 author = {Zhang, Ziqiang and Zhou, Long and Ao, Junyi and Liu, Shujie and Dai, Lirong and Li, Jinyu and Wei, Furu},
 booktitle = {Proc. of EMNLP},
 title = {Speechut: Bridging speech and text with hidden-unit for encoder-decoder based speech-text pre-training},
 year = {2022}
}

@inproceedings{post2018call,
 address = {Brussels, Belgium},
 author = {Post, Matt},
 booktitle = {Proceedings of the Third Conference on Machine Translation: Research Papers},
 doi = {10.18653/v1/W18-6319},
 pages = {186--191},
 publisher = {Association for Computational Linguistics},
 title = {A Call for Clarity in Reporting {BLEU} Scores},
 url = {https://aclanthology.org/W18-6319},
 year = {2018}
}

@misc{duh18multitarget,
 author = {Kevin Duh},
 howpublished = {\url{http://www.cs.jhu.edu/~kevinduh/a/multitarget-tedtalks/}},
 title = {The Multitarget TED Talks Task},
 year = {2018}
}

@inproceedings{sung2019towards,
 author = {Tzu{-}Wei Sung and
Jun{-}You Liu and
Hung{-}yi Lee and
Lin{-}Shan Lee},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icassp/SungLLL19.bib},
 booktitle = {{IEEE} International Conference on Acoustics, Speech and Signal Processing,
{ICASSP} 2019, Brighton, United Kingdom, May 12-17, 2019},
 doi = {10.1109/ICASSP.2019.8682801},
 pages = {7175--7179},
 publisher = {{IEEE}},
 timestamp = {Sun, 30 Jun 2019 01:00:00 +0200},
 title = {Towards End-to-end Speech-to-text Translation with Two-pass Decoding},
 url = {https://doi.org/10.1109/ICASSP.2019.8682801},
 year = {2019}
}

@inproceedings{salesky-etal-2019-exploring,
 address = {Florence, Italy},
 author = {Salesky, Elizabeth  and
Sperber, Matthias  and
Black, Alan W},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/P19-1179},
 pages = {1835--1841},
 publisher = {Association for Computational Linguistics},
 title = {Exploring Phoneme-Level Speech Representations for End-to-End Speech Translation},
 url = {https://aclanthology.org/P19-1179},
 year = {2019}
}

@article{chen2020mam,
 author = {Chen, Junkun and Ma, Mingbo and Zheng, Renjie and Huang, Liang},
 journal = {ArXiv preprint},
 title = {Mam: Masked acoustic modeling for end-to-end speech-to-text translation},
 url = {https://arxiv.org/abs/2010.11445},
 volume = {abs/2010.11445},
 year = {2020}
}

@inproceedings{han-etal-2021-learning,
 address = {Online},
 author = {Han, Chi  and
Wang, Mingxuan  and
Ji, Heng  and
Li, Lei},
 booktitle = {Findings of ACL-IJCNLP 2021},
 doi = {10.18653/v1/2021.findings-acl.195},
 pages = {2214--2225},
 publisher = {Association for Computational Linguistics},
 title = {Learning Shared Semantic Space for Speech-to-Text Translation},
 url = {https://aclanthology.org/2021.findings-acl.195},
 year = {2021}
}

@inproceedings{sennrich-etal-2016-improving,
 address = {Berlin, Germany},
 author = {Sennrich, Rico  and
Haddow, Barry  and
Birch, Alexandra},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/P16-1009},
 pages = {86--96},
 publisher = {Association for Computational Linguistics},
 title = {Improving Neural Machine Translation Models with Monolingual Data},
 url = {https://aclanthology.org/P16-1009},
 year = {2016}
}

@article{wu2022wav2seq,
 author = {Wu, Felix and Kim, Kwangyoun and Watanabe, Shinji and Han, Kyu and McDonald, Ryan and Weinberger, Kilian Q and Artzi, Yoav},
 journal = {ArXiv preprint},
 title = {Wav2Seq: Pre-training Speech-to-Text Encoder-Decoder Models Using Pseudo Languages},
 url = {https://arxiv.org/abs/2205.01086},
 volume = {abs/2205.01086},
 year = {2022}
}

@inproceedings{ren2020fastspeech,
 author = {Yi Ren and
Chenxu Hu and
Xu Tan and
Tao Qin and
Sheng Zhao and
Zhou Zhao and
Tie{-}Yan Liu},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/0006H0QZZL21.bib},
 booktitle = {Proc. of ICLR},
 publisher = {OpenReview.net},
 timestamp = {Wed, 23 Jun 2021 01:00:00 +0200},
 title = {FastSpeech 2: Fast and High-Quality End-to-End Text to Speech},
 url = {https://openreview.net/forum?id=piLPYqxtWuA},
 year = {2021}
}

@inproceedings{kong2020hifi,
 author = {Jungil Kong and
Jaehyeon Kim and
Jaekyoung Bae},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/KongKB20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {HiFi-GAN: Generative Adversarial Networks for Efficient and High Fidelity
Speech Synthesis},
 url = {https://proceedings.neurips.cc/paper/2020/hash/c5d736809766d46260d816d8dbc9eb44-Abstract.html},
 year = {2020}
}

@inproceedings{chen2021gigaspeech,
 author = {Guoguo Chen and
Shuzhou Chai and
Guan{-}Bo Wang and
Jiayu Du and
Wei{-}Qiang Zhang and
Chao Weng and
Dan Su and
Daniel Povey and
Jan Trmal and
Junbo Zhang and
Mingjie Jin and
Sanjeev Khudanpur and
Shinji Watanabe and
Shuaijiang Zhao and
Wei Zou and
Xiangang Li and
Xuchen Yao and
Yongqing Wang and
Zhao You and
Zhiyong Yan},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/interspeech/ChenCWDZWSPTZJK21.bib},
 booktitle = {Proc. of INTERSPEECH},
 doi = {10.21437/Interspeech.2021-1965},
 editor = {Hynek Hermansky and
Honza Cernock{\'{y}} and
Luk{\'{a}}s Burget and
Lori Lamel and
Odette Scharenborg and
Petr Motl{\'{\i}}cek},
 pages = {3670--3674},
 publisher = {{ISCA}},
 timestamp = {Mon, 14 Mar 2022 00:00:00 +0100},
 title = {GigaSpeech: An Evolving, Multi-Domain {ASR} Corpus with 10, 000 Hours
of Transcribed Audio},
 url = {https://doi.org/10.21437/Interspeech.2021-1965},
 year = {2021}
}

@article{kreuk2021textless,
 author = {Kreuk, Felix and Polyak, Adam and Copet, Jade and Kharitonov, Eugene and Nguyen, Tu-Anh and Rivi{\`e}re, Morgane and Hsu, Wei-Ning and Mohamed, Abdelrahman and Dupoux, Emmanuel and Adi, Yossi},
 journal = {ArXiv preprint},
 title = {Textless speech emotion conversion using decomposed and discrete representations},
 url = {https://arxiv.org/abs/2111.07402},
 volume = {abs/2111.07402},
 year = {2021}
}

@inproceedings{polyak2021speech,
 author = {Adam Polyak and
Yossi Adi and
Jade Copet and
Eugene Kharitonov and
Kushal Lakhotia and
Wei{-}Ning Hsu and
Abdelrahman Mohamed and
Emmanuel Dupoux},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/interspeech/PolyakACKLHMD21.bib},
 booktitle = {Proc. of INTERSPEECH},
 doi = {10.21437/Interspeech.2021-475},
 editor = {Hynek Hermansky and
Honza Cernock{\'{y}} and
Luk{\'{a}}s Burget and
Lori Lamel and
Odette Scharenborg and
Petr Motl{\'{\i}}cek},
 pages = {3615--3619},
 publisher = {{ISCA}},
 timestamp = {Mon, 14 Mar 2022 00:00:00 +0100},
 title = {Speech Resynthesis from Discrete Disentangled Self-Supervised Representations},
 url = {https://doi.org/10.21437/Interspeech.2021-475},
 year = {2021}
}

@inproceedings{xia2019generalized,
 address = {Florence, Italy},
 author = {Xia, Mengzhou  and
Kong, Xiang  and
Anastasopoulos, Antonios  and
Neubig, Graham},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/P19-1579},
 pages = {5786--5796},
 publisher = {Association for Computational Linguistics},
 title = {Generalized Data Augmentation for Low-Resource Translation},
 url = {https://aclanthology.org/P19-1579},
 year = {2019}
}

@article{tang2020multilingual,
 author = {Tang, Yuqing and Tran, Chau and Li, Xian and Chen, Peng-Jen and Goyal, Naman and Chaudhary, Vishrav and Gu, Jiatao and Fan, Angela},
 journal = {ArXiv preprint},
 title = {Multilingual translation with extensible multilingual pretraining and finetuning},
 url = {https://arxiv.org/abs/2008.00401},
 volume = {abs/2008.00401},
 year = {2020}
}

@inproceedings{chen2020facebook,
 address = {Online},
 author = {Chen, Peng-Jen  and
Lee, Ann  and
Wang, Changhan  and
Goyal, Naman  and
Fan, Angela  and
Williamson, Mary  and
Gu, Jiatao},
 booktitle = {Proceedings of the Fifth Conference on Machine Translation},
 pages = {113--125},
 publisher = {Association for Computational Linguistics},
 title = {{F}acebook {AI}{'}s {WMT}20 News Translation Task Submission},
 url = {https://aclanthology.org/2020.wmt-1.8},
 year = {2020}
}

@inproceedings{bojar2011improving,
 address = {Edinburgh, Scotland},
 author = {Bojar, Ond{\v{r}}ej  and
Tamchyna, Ale{\v{s}}},
 booktitle = {Proceedings of the Sixth Workshop on Statistical Machine Translation},
 pages = {330--336},
 publisher = {Association for Computational Linguistics},
 title = {Improving Translation Model by Monolingual Data},
 url = {https://aclanthology.org/W11-2138},
 year = {2011}
}

@inproceedings{bertoldi2009domain,
 address = {Athens, Greece},
 author = {Bertoldi, Nicola  and
Federico, Marcello},
 booktitle = {Proceedings of the Fourth Workshop on Statistical Machine Translation},
 pages = {182--189},
 publisher = {Association for Computational Linguistics},
 title = {Domain Adaptation for Statistical Machine Translation with Monolingual Resources},
 url = {https://aclanthology.org/W09-0432},
 year = {2009}
}

@inproceedings{sennrich2016improving,
 address = {Berlin, Germany},
 author = {Sennrich, Rico  and
Haddow, Barry  and
Birch, Alexandra},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/P16-1009},
 pages = {86--96},
 publisher = {Association for Computational Linguistics},
 title = {Improving Neural Machine Translation Models with Monolingual Data},
 url = {https://aclanthology.org/P16-1009},
 year = {2016}
}

@inproceedings{hoang2018iterative,
 address = {Melbourne, Australia},
 author = {Hoang, Vu Cong Duy  and
Koehn, Philipp  and
Haffari, Gholamreza  and
Cohn, Trevor},
 booktitle = {Proceedings of the 2nd Workshop on Neural Machine Translation and Generation},
 doi = {10.18653/v1/W18-2703},
 pages = {18--24},
 publisher = {Association for Computational Linguistics},
 title = {Iterative Back-Translation for Neural Machine Translation},
 url = {https://aclanthology.org/W18-2703},
 year = {2018}
}

@inproceedings{imamura2018enhancement,
 address = {Melbourne, Australia},
 author = {Imamura, Kenji  and
Fujita, Atsushi  and
Sumita, Eiichiro},
 booktitle = {Proceedings of the 2nd Workshop on Neural Machine Translation and Generation},
 doi = {10.18653/v1/W18-2707},
 pages = {55--63},
 publisher = {Association for Computational Linguistics},
 title = {Enhancement of Encoder and Attention Using Target Monolingual Corpora in Neural Machine Translation},
 url = {https://aclanthology.org/W18-2707},
 year = {2018}
}

@inproceedings{adelani2022findings,
 author = {Adelani, David Ifeoluwa and Alam, Md Mahfuz Ibn and Anastasopoulos, Antonios and Bhagia, Akshita and Costa-Juss{\'a}, Marta and Dodge, Jesse and Faisal, Fahim and Federmann, Christian and Fedorova, Natalia and Guzm{\'a}n, Francisco and others},
 booktitle = {Proceedings of the Seventh Conference on Machine Translation, Online. Association for Computational Linguistics},
 title = {Findings of the WMT 2022 shared task on large-scale machine translation evaluation for african languages},
 year = {2022}
}

@inproceedings{wenzek2021findings,
 address = {Online},
 author = {Wenzek, Guillaume  and
Chaudhary, Vishrav  and
Fan, Angela  and
Gomez, Sahir  and
Goyal, Naman  and
Jain, Somya  and
Kiela, Douwe  and
Thrush, Tristan  and
Guzm{\'a}n, Francisco},
 booktitle = {Proceedings of the Sixth Conference on Machine Translation},
 pages = {89--99},
 publisher = {Association for Computational Linguistics},
 title = {Findings of the {WMT} 2021 Shared Task on Large-Scale Multilingual Machine Translation},
 url = {https://aclanthology.org/2021.wmt-1.2},
 year = {2021}
}

@inproceedings{farhad2021findings,
 address = {Copenhagen, Denmark},
 author = {Bojar, Ond{\v{r}}ej  and
Chatterjee, Rajen  and
Federmann, Christian  and
Graham, Yvette  and
Haddow, Barry  and
Huang, Shujian  and
Huck, Matthias  and
Koehn, Philipp  and
Liu, Qun  and
Logacheva, Varvara  and
Monz, Christof  and
Negri, Matteo  and
Post, Matt  and
Rubino, Raphael  and
Specia, Lucia  and
Turchi, Marco},
 booktitle = {Proceedings of the Second Conference on Machine Translation},
 doi = {10.18653/v1/W17-4717},
 pages = {169--214},
 publisher = {Association for Computational Linguistics},
 title = {Findings of the 2017 Conference on Machine Translation ({WMT}17)},
 url = {https://aclanthology.org/W17-4717},
 year = {2017}
}

@inproceedings{hayashi2018back,
 author = {Hayashi, Tomoki and Watanabe, Shinji and Zhang, Yu and Toda, Tomoki and Hori, Takaaki and Astudillo, Ramon and Takeda, Kazuya},
 booktitle = {2018 IEEE Spoken Language Technology Workshop (SLT)},
 organization = {IEEE},
 pages = {426--433},
 title = {Back-translation-style data augmentation for end-to-end ASR},
 year = {2018}
}

@inproceedings{ueno2021data,
 author = {Ueno, Sei and Mimura, Masato and Sakai, Shinsuke and Kawahara, Tatsuya},
 booktitle = {2021 IEEE Automatic Speech Recognition and Understanding Workshop (ASRU)},
 organization = {IEEE},
 pages = {68--75},
 title = {Data Augmentation for ASR Using TTS Via a Discrete Representation},
 year = {2021}
}

@inproceedings{tjandra2017listening,
 author = {Tjandra, Andros and Sakti, Sakriani and Nakamura, Satoshi},
 booktitle = {2017 IEEE Automatic Speech Recognition and Understanding Workshop (ASRU)},
 organization = {IEEE},
 pages = {301--308},
 title = {Listening while speaking: Speech chain by deep learning},
 year = {2017}
}

@inproceedings{zhang2022ustc,
 address = {Dublin, Ireland (in-person and online)},
 author = {Zhang, Weitai  and
Ye, Zhongyi  and
Tang, Haitao  and
Li, Xiaoxi  and
Zhou, Xinyuan  and
Yang, Jing  and
Cui, Jianwei  and
Deng, Pan  and
Shi, Mohan  and
Song, Yifan  and
Liu, Dan  and
Liu, Junhua  and
Dai, Lirong},
 booktitle = {Proceedings of the 19th International Conference on Spoken Language Translation (IWSLT 2022)},
 doi = {10.18653/v1/2022.iwslt-1.15},
 pages = {198--207},
 publisher = {Association for Computational Linguistics},
 title = {The {USTC}-{NELSLIP} Offline Speech Translation Systems for {IWSLT} 2022},
 url = {https://aclanthology.org/2022.iwslt-1.15},
 year = {2022}
}

@article{bapna2022mslam,
 author = {Bapna, Ankur and Cherry, Colin and Zhang, Yu and Jia, Ye and Johnson, Melvin and Cheng, Yong and Khanuja, Simran and Riesa, Jason and Conneau, Alexis},
 journal = {ArXiv preprint},
 title = {mSLAM: Massively multilingual joint pre-training for speech and text},
 url = {https://arxiv.org/abs/2202.01374},
 volume = {abs/2202.01374},
 year = {2022}
}

@article{babu2021xls,
 author = {Babu, Arun and Wang, Changhan and Tjandra, Andros and Lakhotia, Kushal and Xu, Qiantong and Goyal, Naman and Singh, Kritika and von Platen, Patrick and Saraf, Yatharth and Pino, Juan and others},
 journal = {ArXiv preprint},
 title = {XLS-R: Self-supervised cross-lingual speech representation learning at scale},
 url = {https://arxiv.org/abs/2111.09296},
 volume = {abs/2111.09296},
 year = {2021}
}

@inproceedings{li2021multilingual,
 address = {Online},
 author = {Li, Xian  and
Wang, Changhan  and
Tang, Yun  and
Tran, Chau  and
Tang, Yuqing  and
Pino, Juan  and
Baevski, Alexei  and
Conneau, Alexis  and
Auli, Michael},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2021.acl-long.68},
 pages = {827--838},
 publisher = {Association for Computational Linguistics},
 title = {Multilingual Speech Translation from Efficient Finetuning of Pretrained Models},
 url = {https://aclanthology.org/2021.acl-long.68},
 year = {2021}
}

@inproceedings{ardila-etal-2020-common,
 address = {Marseille, France},
 author = {Ardila, Rosana  and
Branson, Megan  and
Davis, Kelly  and
Kohler, Michael  and
Meyer, Josh  and
Henretty, Michael  and
Morais, Reuben  and
Saunders, Lindsay  and
Tyers, Francis  and
Weber, Gregor},
 booktitle = {Proceedings of the Twelfth Language Resources and Evaluation Conference},
 isbn = {979-10-95546-34-4},
 language = {English},
 pages = {4218--4222},
 publisher = {European Language Resources Association},
 title = {Common Voice: A Massively-Multilingual Speech Corpus},
 url = {https://aclanthology.org/2020.lrec-1.520},
 year = {2020}
}

@inproceedings{ott2019fairseq,
 address = {Minneapolis, Minnesota},
 author = {Ott, Myle  and
Edunov, Sergey  and
Baevski, Alexei  and
Fan, Angela  and
Gross, Sam  and
Ng, Nathan  and
Grangier, David  and
Auli, Michael},
 booktitle = {Proceedings of the 2019 Conference of the North {A}merican Chapter of the Association for Computational Linguistics (Demonstrations)},
 doi = {10.18653/v1/N19-4009},
 pages = {48--53},
 publisher = {Association for Computational Linguistics},
 title = {fairseq: A Fast, Extensible Toolkit for Sequence Modeling},
 url = {https://aclanthology.org/N19-4009},
 year = {2019}
}

@inproceedings{bojar-EtAl:2016:WMT1,
 address = {Berlin, Germany},
 author = {Bojar, Ond{\v{r}}ej  and
Chatterjee, Rajen  and
Federmann, Christian  and
Graham, Yvette  and
Haddow, Barry  and
Huck, Matthias  and
Jimeno Yepes, Antonio  and
Koehn, Philipp  and
Logacheva, Varvara  and
Monz, Christof  and
Negri, Matteo  and
N{\'e}v{\'e}ol, Aur{\'e}lie  and
Neves, Mariana  and
Popel, Martin  and
Post, Matt  and
Rubino, Raphael  and
Scarton, Carolina  and
Specia, Lucia  and
Turchi, Marco  and
Verspoor, Karin  and
Zampieri, Marcos},
 booktitle = {Proceedings of the First Conference on Machine Translation: Volume 2, Shared Task Papers},
 doi = {10.18653/v1/W16-2301},
 pages = {131--198},
 publisher = {Association for Computational Linguistics},
 title = {Findings of the 2016 Conference on Machine Translation},
 url = {https://aclanthology.org/W16-2301},
 year = {2016}
}

@inproceedings{schwenk2019ccmatrix,
 address = {Online},
 author = {Schwenk, Holger  and
Wenzek, Guillaume  and
Edunov, Sergey  and
Grave, Edouard  and
Joulin, Armand  and
Fan, Angela},
 booktitle = {Proc. of ACL},
 doi = {10.18653/v1/2021.acl-long.507},
 pages = {6490--6500},
 publisher = {Association for Computational Linguistics},
 title = {{CCM}atrix: Mining Billions of High-Quality Parallel Sentences on the Web},
 url = {https://aclanthology.org/2021.acl-long.507},
 year = {2021}
}

